Coordinating drones with mothership vehicles: The mothership and multiple drones routing problem with Graphs

This paper considers the optimization problems that arise to coordinate a tandem between a mothership vehicle and a fleet of drones. %more than one drone. Each drone can be launched from the mothership to perform an operation. After completing the operations the drones return to the mothership to recharge batteries and to be ready for a new operation. Operations consist on (partially) visiting graphs with given lengths to deliver some service or to perform some surveillance/inspection activity. The goal is to minimize the overall weighted distance traveled by the mothership while satisfying some requirements in terms of percentages of visits to the target graphs. In all cases, we develop exact formulations resorting to mixed integer second order cone programs that are compared on a testbed of instances to assess their performance. We also develop a matheuristic algorithm that provides reasonable solutions. Computational experiments show the usefulness of our methods in different scenarios.

==> Mothership Drone/bounds.tex <==
\section{Strengthening the formulation of \AMD}\label{bounds}
\noindent
In this section we present some valid inequalities for \AMD\xspace that reinforce the formulation given in Section \ref{Form}. Moreover, the \eqref{DCW} constraint has products of binary and continuous variables that, when they are linearized, produce big-M constants that have to be tightened. This section also provides some bounds for these constants whenever it is possible. 

%\CV{*** This last sentence is not done yet -JUSTO dixit- ***}

%Notation here is not very good: we use C for clusters, centroids and the drone capacity. This must be improved.

\subsection{Valid inequalities for the \AMD}
\noindent
In this problem, we assume that the fleet has more than one drone since otherwise the problem reduces to (AMDRPG) that was already studied in \cite{art:Amorosi2021}. Therefore, if there exists a stage in which more than one drone is launched, the mothership does not need to perform $|\mathcal G|$ different stages. Hence, most likely the model does not need to deal with those stages that are numbered at the end. By exploiting this idea, it is possible to concentrate all drone operations on the first stages, avoiding empty tasks in $\mathcal T$.
\noindent
Let $\beta^t$ be a binary variable that assumes the value one if all the target graphs are visited when the operation $t$ begins, and  zero, otherwise. Note that, if all the operations are completed before the stage $t$ then they are also completed before the stage $t+1$. Hence, $\beta$ variables must satisfy the following constraints:

\begin{equation}\tag{Monotonicity}\label{eq:Monotonicity}
\beta^t \leq \beta^{t+1}, \mbox{ for all } t=1,\ldots, |\mathcal{G}|-1.
\end{equation}

\noindent
Let $k^t$ denote the number of graphs that are visited in the stage $t$. This number can be computed using the $u$ variables since $u^{e_gtd}$ takes the value 1 if the graph $g$ is visited in stage $t$ by the drone $d$. Thus:

$$k^t=\sum_{e_g\in g:g\in\mathcal G}\sum_{d\in\mathcal D} u^{e_gtd}.$$

\noindent
Hence, if $\beta^t$ equals one, the entire set of graphs in $\mathcal G$ must have been visited before the stage $t$:

\begin{equation}\tag{VI-1}\label{eq:VI-1}
\sum_{t'=1}^{t-1} k^{t'} \geq |\mathcal G|\beta^t,
\end{equation}
where $|\mathcal G|$ denotes the number of graphs of $\mathcal G$.

\noindent
To reduce the space of feasible solutions, we can assume without loss of generality that it is not permitted to have a stage $t$ without any operation if some graphs are still to be visited. This can be enforced by the following constraints:

\begin{equation}\tag{VI-2}\label{eq:VI-2}
k^t \geq 1 - \beta^t.
\end{equation}

\noindent
In addition, it is also possible to reduce the symmetry. Since we are assuming that drones are indistinguishable, we can assume that given an arbitrary order on them, we always assign drones to operations in that given order. This assumption allows us to assign for an operation at the stage $t$ the first drone that is available, avoiding to consider the last ones, if they are not necessary. This consideration can be implemented by means of the following set of inequalities. For all $t\in\mathcal T$:
\medskip

% \noindent **** OJO :  Mas fuertes ************
\begin{equation}\tag{VI-3}\label{eq:VI-3}
\sum_{e_g\in \mathcal G} u^{e_gtd} \leq \sum_{e_g:g\in\mathcal G}u^{e_gtd-1}, \; \forall d=2,\ldots |\mathcal D|,      
\end{equation}
\begin{equation}\tag{VI-4}\label{eq:VI-4}
\sum_{e_g\in \mathcal G} v^{e_gtd} \leq \sum_{e_g:g\in\mathcal G}v^{e_gtd-1}, \; \forall d=2,\ldots |\mathcal D|.      
\end{equation}
% ****************************
% \CV{\begin{equation}\tag{VI-3}\label{eq:VI-3}
% u^{e_gtd_1} \leq \sum_{e_g:g\in\mathcal G}\sum_{t\in\mathcal T} u^{e_gtd_2},\quad d_1>d_2
% \end{equation}
% \begin{equation}\tag{VI-4}\label{eq:VI-4}
% v^{e_gtd_1} \leq \sum_{e_g:g\in\mathcal G}\sum_{t\in\mathcal T} v^{e_gtd_2},\quad d_1>d_2.
% \end{equation}

\noindent
Hence, if the drone $d_1$ is assigned to the task $t$, every drone $d_2$ that is, for the launching order in $\mathcal D$, before than $d_1$, must have been also assigned to perform the task $t$.
\medskip
% }

\noindent
The model that we have proposed includes big-M constants. We have defined different big-M constants along this work. In order to strengthen the formulations we provide tight upper and lower bounds for those constants. In this section we present some results that adjust them for each one of the models.

\subsubsection*{Big $M$ constants bounding the distance from the launching / rendezvous point on the path followed by the mothership to the rendezvous / launching point on the target graph $g\in \mathcal{G}$}

%\CV{Maybe BigM can be more adjusted taking into account the endurance of the drone\ldots}
% \begin{itemize}
% \item \underline{\AMD}. 
\noindent
To linearize the first term of the objective function in \AMD, we define the auxiliar non-negative continuous variables $p_L^{e_gtd}$ (resp. $p_R^{e_gtd}$) and we model the product by including the following constraints:
\begin{align*}
p_L^{e_gtd} & \geq m_L^{e_g} u^{e_gtd}, \\
p_L^{e_gtd} & \leq d_L^{e_g} - M_L^{e_gtd}(1-u^{e_gt}).
\end{align*}
The best upper bound $M_L^{e_gtd}$ or $M_R^{e_gtd}$ that we can consider is the full diameter of the data, that is the maximum distance between every pair of vertices of the graphs $g\in \mathcal{G}$, in the input data, i.e., every launching or rendezvous point is inside the circle whose diametrically opposite points are described below. 
$$
M_R^{e_gtd} = \max_{\{v\in V_g, v'\in V_{g'} : g, g'\in\mathcal G\}} \|v - v'\| = M_L^{e_gtd}.
$$
\noindent
On the other hand, the minimum distance in this case can be zero. This bound is attainable whenever the launching or the rendezvous points of the mothership is the same that the rendezvous or launching point on the target graph $g\in \mathcal{G}$.

% \item \underline{\NMD}. In this case, the best upper bounds for $M_R^{e_gt}$ or $M_L^{e_gt}$ is the maximum distance between the polygonal chain $\mathcal{P}$ or the graph $\mathcal{N}$ and any of the target graphs $g\in \mathcal{G}$:
% $$
% M_R^{e_gt} = \max_{\{v\in V_g, w\in \mathcal N\}}\|v - w\| = M_L^{i_gt}.
% $$
% On the other hand, the minimum distance can be computed by taking the closest points between the graph $g$ and the network $\mathcal{N}$:
% $$
% m_R^{e_gt} = \min_{\{v\in V_g, w\in \mathcal N\}}\|v - w\| = m_L^{e_gt}.
% $$
% \end{itemize}

% \subsubsection*{Bounds on the big $M$ constants for the distance from the launching point to the rendezvous points for the MTZ/SEC formulations in \AMD}

% We can compute a tighter upper bound for the distance $d_{RL}^{gg'}$ between each pair of graphs $g,g'$ for the constraints obtained by the linearization of its product:
% \begin{align*}
% p^{gg'} & \geq m_{RL}^{gg'} d_{RL}^{gg'}, \\
% p^{gg'} & \leq d_{RL}^{gg'} - M_{RL}^{gg'}(1-w^{gg'}).
% \end{align*}
% This upper bound $M_{RL}^{gg'}$ is given by the diameter of $g\cup g'$:
% $$
% M_{RL}^{gg'} = \max_{\{v\in V_g, v'\in V_{g'}\}}\|v - v'\|.
% $$


\subsubsection*{Bounds on the big $M$ constants for the distance from the launching to the rendezvous points on the target graph $g\in \mathcal{G}$.} 
\noindent
When the drone visits a graph $g$, it has to go from one edge $e_g$ to another edge $e'_g$ depending on the order given by $z^{e_ge_g'}$. This fact produces a product of variables linearized by the following constraints:
\begin{align*}
p^{e_ge'_g} & \geq m^{e_ge_g'} d_{RL}^{gg'}, \\
p^{e_ge_g'} & \leq d^{e_ge_g'} - M^{e_ge_g'}(1-z^{e_ge_g'}).
\end{align*}

\noindent
Since we are taking into account the distance between two edges $e=(B^{e_g},C^{e_g}), \, e'=(B^{e^\prime_g},C^{e^\prime_g})\in E_g$, the maximum and minimum distances between their vertices give us the upper and lower bounds:
\begin{align*}
M^{e_g e^\prime_g} = & \max\{\|B^{e_g} - C^{e^\prime_g}\|, \|B^{e_g} - B^{e^\prime_g}\|, \|C^{e_g} - B^{e^\prime_g}\|, \|C^{e_g} - C^{j_g}\|\}, \\
m^{e_g e^\prime_g} = & \min\{\|B^{e_g} - C^{e^\prime_g}\|, \|B^{e_g} - B^{e^\prime_g}\|, \|C^{e_g} - B^{e^\prime_g}\|, \|C^{e_g} - C^{e^\prime_g}\|\}.
\end{align*}

% \subsubsection*{Bounds on the big $M$ constants for the distance covered by the mothership on the polygonal for the \PMD \ model during one drone operation.}
% In the case of \PMD, we can also set tighter upper bounds for the distance covered by the drone inside the polygonal during an operation that starts in $e$ and finishes at $e'$ (or vice versa) (see \eqref{pol:dLRt} and \eqref{pol:dRLt}). This is clearly bounded from above by the total length of the line segments where the mothership is located. 
% \begin{equation*}
% M_{LR}^{ee't} = M_{RL}^{ee't} = \left\{\begin{matrix}
% \mathcal L(e), & \text{if } e = e',\\ 
% \displaystyle \sum_{e<e''<e'}\mathcal L(e'') & \text{if } e < e', \\
% \displaystyle \sum_{e'<e''<e}\mathcal L(e'') & \text{if } e > e'.
% \end{matrix}\right.
% \end{equation*}


\subsubsection*{Bounds on the big $M$ constants for the distance covered by the drone during an operation for all the models by stages}
\noindent
To link the drone operation with the trip followed by the mothership, we have defined the constraint $\eqref{DCW}$ that includes another big-M constant:
\begin{equation*}
\left(\sum_{e_g\in E_g} u^{e_gtd}d_L^{e_gtd} + \sum_{e_g, e^\prime_g\in E_g}z^{e_ge^\prime_g}d^{e_ge^\prime_g} + \sum_{e_g\in E_g} \mu^{e_g}d^{e_g} + \sum_{e_g\in E_g} v^{e_gtd}d_R^{e_gtd}\right)/v_D \leq d_{RL}^t/v_M + M(1 - \sum_{e_g\in E_g} u^{e_gtd}).
\end{equation*}
\noindent
To obtain an upper bound on $M$ we add to the length of the graph $\mathcal L(g)$ the big-Ms computed for $u^{e_gtd}$ and $v^{e_gtd}$, namely $M_{L}^{e_gtd}$ and $M_R^{e_gtd}$, respectively, and the maximum distance that can be traveled by the drone to move from one edge to another one. This results in a valid value for this $M$ constant:

$$M = \mathcal{L}(g) + M_L^{e_gtd} + M_R^{e_gtd} + \sum_{e_g, e_g'\in E_g}M^{e_ge_g'}.$$



==> Mothership Drone/case_study.tex <==
\section{Case Study}

\noindent
In this section we describe a realistic application of the system studied in this paper to perform surveillance operations. Considering the current COVID-19 restrictions, we focus on the problem of preventing and identifying possible concentrations of people during events such as popular or religious festivals. In particular we consider the Courtyards Festival of Cordoba (\url{https://patios.cordoba.es/es/}). This is a social event that takes place every year in the city of Cordoba, Spain, during the first two weeks of May. Courtyard’s owners decorate their houses with many flowers trying to win the award that is offered by the Town Hall. During this competition a festival runs in parallel with a number of artistic performances along six different paths located in different areas in the city as shown in Figure \ref{fig:mapPF}.
In the pandemic context, to monitor the situation to avoid concentration of people, we propose to apply a system consisting of one helicopter and a fleet of three drones.
This kind of system has been proved successfully and has been already applied in the military field by the US Army in order to leave the helicopter to the edge of dangerous airspace and release drones, which will then penetrate enemy territory and send back intelligence, surveillance and reconnaissance information (see \cite{FG}).
In our application the reason to adopt a similar system is the possibility to inspect simultaneously and in real time different paths also reducing the risk of flying the helicopter over populated areas and the cost for moving the helicopter by minimizing the total length of its tour.

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figures/first.png}
\caption{Map of the Courtyards Festival in Cordoba. \label{fig:mapPF}}
\end{figure}

\noindent
We run the model presented in Section \ref{Form} on this scenario starting from the initial solution provided by the matheuristic, where the 6 coloured paths reported in the map of Figure \ref{fig:mapPF} represent the 6 target graphs to be visited, in this case inspected, by the fleet of drones. In addition, we suppose that the drones' speed is 100 km/h while that of the helicopter is  50 km/h aiming to minimize costs.
Moreover, we assume that the fleet is composed by three drones with an endurance equal to 2 hours, and we impose that each target graph must be fully visited (inspected).  As we can see from Figure \ref{fig:Mtour}, the origin of the mothership tour coincides with the destination and it is located in an area of the city where it is possible to assume the take-off and landing of an helicopter. Figure \ref{fig:Mtour} reports the tour followed by the helicopter in the solution obtained within the time limit of 2 hours sets to solve the model and with a percentage gap equal to 83\%. We can observe that the helicopter, starting from the origin, flies to the point $x_L^1$ that is the first launching point and then flies along the edge connecting $x_L^1$ with $x_R^1$, that is the first rendezvous point. Next, the helicopter flies to $x_L^2$ for launching the second drones' mission that are retrieved at point $x_R^2$. The third and last mission starts from $x_L^3$ and ends at point $x_R^3$ from where the helicopter goes back to the final destination.\\
Figure \ref{fig:tourD} shows the tour followed by the three drones for inspecting the six paths. In particular, one drone, in red, starts from $x_L^1$ for visiting the path of "Alcazar Viejo". From the same point a second drone, in green, starts for visiting the path of "Santa Maria-San Agustin". Both drones end their first mission at point $x_R^1$, where they are retrieved by the helicopter. Then, the helicopter flies to point $x_L^2$ where only one drone, the red one, starts its second mission to visit the path of "Juderia-San Francisco". In the meanwhile the helicopter, containing the other two drones, flies to point $x_R^2$ where it retrieves the previously launched drone. The last mission involves all the three drones that are launched from point $x_L^3$. The first drone, the red one, visits the path of "San Lorenzo", the second, the green one, visits the path of "Regina-Realejo" and the third, the blue one, visits the path of "Santiago-San Pedro".
All the three drones are retrieved by the helicopter at point $x_R^3$ and after that the helicopter goes back to the destination. 
The total distance travelled by the helicopter is equal to 11.27 km.

All details of this case study, including maps coordinates, .lp models and solutions can be found in \cite{Puerto2021}.


\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figures/second.png}
\caption{Mothership tour. \label{fig:Mtour}}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figures/third.png}
\caption{The complete solution. \label{fig:tourD}}
\end{figure}

==> Mothership Drone/conclusion.tex <==
\section{Concluding remarks}
\noindent
This papers has analyzed the coordination problem that arises between a mothership vehicle and a fleet of drones that must coordinate their routes to minimize the total distance travelled by the mothership while visiting a set of targets modeled by graphs. We have presented exact formulations of the problem, for its synchronized and not synchronized versions. They are mixed integer non-linear programming models. Moreover, we presented valid inequalities for them. \\
Our computational results show that the considered problem is very challenging to solve even on small to medium size instances. For that reason, additionally, we have proposed a matheuristic algorithm that provides acceptable feasible solutions in very short computing time; so that it is a good alternative to the exact method. We report extensive computational experiments on randomly generated instances. Moreover, we present a case study related to inspection activities in the context of COVID-19 restrictions. We show the application of the system described in this paper in the framework of the Courtyard Festival in the city of Cordoba, by illustrating the solution obtained by adopting the problem formulation, in its synchronized version, and its solution by means of the initialization provided by the proposed matheuristic.\\
\noindent
The formulation and algorithms proposed in this paper can be seen a first building block to handle coordination of systems given by a base vehicle and drones. Further research in this topic must focus on finding faster and more accurate algorithms able to solve larger instances. Moreover, it is also challenging to model more complex operations  allowing that drones can visit more than one target per trip. These problems being very interesting are beyond the scope of the present paper and will be the focus of a follow up research line.

==> Mothership Drone/description.tex <==
\section{Problem description and valid formulation}\label{section:desc}
% Datos iniciales del problema

\subsection{Problem description}
In the All terrain Mothership and Multiple Drones Routing Problem with Graphs (\AMD), there is one mothership (the base vehicle) and a fleet of homogeneous drones $\mathcal D$ that have to coordinate among them and with the mothership to perform a number of operations consisting in visiting given percentages of the length of a set of graphs $\mathcal G$. The mothership and the drones travel at constant velocities $v_M$ and $v_D$, respectively. Moreover, it is assumed that each  drone has a limited flying autonomy (endurance) $N^d$, so that once it is launched it must complete the operation and return back to the base vehicle to recharge batteries before the time limit. The base vehicle can move freely on a continuous space and starts at a known location, denoted $orig$ where the mothership and the fleet of drones are ready to depart. Once all the operations are finished the mothership and the drones must return together to a final location, called $dest$. 
%Finally, the mothership is allowed to move freely in a continuous space: $\mathbb R^2$ or $\mathbb R^3$.
\noindent
The set of target graphs $\mathcal G$ to be visited  permits to model real situations like monitoring and inspection activities on portions of networks (roads or wires) where traditional vehicles cannot arrive, due to, for example,  the presence of narrow streets, or because of a natural disaster or a terrorist attack that caused damages on the network. In all these cases, the inspection or monitoring of the drone consists in traversing edges of the network to perform a reconnaissance activity. For this reason we model the targets, to be visited by the drone, as graphs. The operation of visiting a graph can be of two different types: 1) traversing a given percentage of the length of each one of its edges or 2) visiting a percentage of the total length of the network. 

% In this case, for the sake of simplicity, it is assumed that there exist no obstacles to prevent drone travelling in straight line. Nevertheless, that extension is interesting to be further considered although is beyond the scope of this paper.\\

\noindent
In this problem, it is assumed that each graph must be visited by one drone: once the drone assigned to the operation enters the graph, it has to complete the entire operation of traversing this target before to be able to leave the graph to return to the base. Moreover, at each stage the drones must be launched from the mothership at the same point (the launching points have to be determined) and they also must be retrieved at the same point (the rendezvous points also have to be determined). However, this does not mean that the mothership and all drones must arrive at a rendezvous location at the same time: the fastest arriving vehicle may wait for the others at the rendezvous location. Note also that every drone of the fleet does not have to be launched from the current base vehicle location in all the stages because of the capacity constraint. In addition, it is supposed that the cost induced by the drones' trips are negligible as compared to those incurred by the base vehicle. Therefore, the goal is to minimize the overall distance traveled by the mothership. In spite of that, the reader may note that from a theoretical point of view the extension to include in the objective function also the distances traveled by the drones is straightforward and does not increase the complexity of the models and formulations.
\noindent
The goal of the \AMD \ is to find the launching and rendezvous points of the fleet of drones $\mathcal D$ satisfying the visit requirements for the graphs in $\mathcal G$ and minimizing the length of the path traveled by the mothership.\\

\noindent



% The mothership and the drone begin at a starting location, denoted $orig$ and a set $\mathcal G$ of target locations modeled by graphs, that must be visited by the drone, are located in the plane. These assumptions permit to model several real situations like roads or wired networks inspection.
% %The natural application for this situation comes from road or wired network inspection. 
% For each stage $t \in \{1, \ldots, |\mathcal G|\}$, we require that the drone is launched from the current mothership location, that at stage $t$ is a decision variable denoted by $x_L^t$, flies to one of the graphs $g$ that has to be visited , traverses the required portion of $g$ and then returns to the current position of the mothership, that most likely is different from the launching point $x_L^t$, and  that is another decision variable denoted by $x_R^t$. Once all targets graphs have been visited, the mothership and drone return to a final location (depot), denoted by $dest$.\\
% \noindent
% Let $g = (V_g, E_g)$ be a graph in $\mathcal G$ whose total length is denoted by $\mathcal L(g)$ and $e_g$ that denotes the edge $e$ of this graph $g$. This edge is parametrized by its endpoints $B^{e_g}, C^{e_g}$ and its length $\|\overline{B^{e_g}C^{e_g}}\|$ is denoted by $\mathcal L(e_g)$. For each line segment, we assign a binary variable $\mu^{e_g}$ that indicates whether or not the drone visits the segment $e_g$ and define entry and exit points $(R^{e_g}, \rho^{e_g})$ and $(L^{e_g}, \lambda^{e_g})$, respectively, that determine the portion of the edge visited by the drone. \\
% \noindent
% We have considered two modes of visit to the targets graphs $g\in \mathcal{G}$:
% \begin{itemize}
%     \item Visiting a percentage $\alpha^{e_g}$ of each edge $e_g$ which can be modeled by using the following constraints:
%     \begin{equation}\label{eq:alphaE}\tag{$\alpha$-E}
%     |\lambda^{e_g} - \rho^{e_g}|\mu^{e_g}\geq \alpha^{e_g}, \quad \forall e_g\in E_g.
%     \end{equation}
%     \item Visiting a percentage $\alpha_g$ of the total length of the graph:
%     \begin{equation}\label{eq:alphaG}\tag{$\alpha$-G}
%     \sum_{e_g\in E_g} \mu^{e_g}|\lambda^{e_g} - \rho^{e_g}|\mathcal L(e_g) \geq \alpha^g\mathcal L(g),
%     \end{equation}
%     where $\mathcal L(g)$ denotes the total length of the graph.
% \end{itemize}

% \bigskip
% \noindent
% In both cases, we need to introduce a binary variable $\text{entry}^{e_g}$ that determines the traveling direction on the edge $e_g$ as well as the definition of the parameter values $\nu_\text{min}^{e_g}$ and $\nu_\text{max}^{e_g}$ of the access and exit points to that segment. Then, for each edge $e_g$, the absolute value constraint \eqref{eq:alphaE} can be represented by:

% \begin{equation}\label{eq:alpha-E}\tag{$\alpha$-E}
%  \mu^{e_g}|\rho^{e_g}-\lambda^{e_g}|\geq \alpha^{e_g} \Longleftrightarrow
%  \left\{
%  \begin{array}{ccl}
%   \rho^{e_g} - \lambda^{e_g}                       & =    & \nu_\text{max}^{e_g} - \nu_\text{min}^{e_g}                                     \\
%   \nu_\text{max}^{e_g}                         & \leq & 1-{\text{entry}^{e_g}}                                    \\
%   \nu_\text{min}^{e_g}                      & \leq & {  \text{entry}^{e_g}},                                        \\
%   \mu^{e_g}(\nu_\text{max}^{e_g} + \nu_\text{min}^{e_g} ) & \geq & \alpha^{e_g}
%   \\
%  \end{array}
%  \right.
% \end{equation}

% \noindent
% The linearization of \eqref{eq:alphaG} is similar to \eqref{eq:alphaE} by changing the last inequality in \eqref{eq:alpha-E} for

% \begin{equation}\label{eq:alpha-G}\tag{$\alpha$-G}
% \sum_{e_g\in E_g} \mu^{e_g}(\nu_\text{max}^{e_g} + \nu_\text{min}^{e_g})\mathcal L(e_g)\geq \alpha_g\mathcal L(g).
% \end{equation}

% \noindent
% In our model wlog, we assume  that the mothership and drone do not need to arrive at a rendezvous location at the same time: the
% faster arriving vehicle may wait for the other at the rendezvous location. In addition, we also assume that vehicles move at constant speeds, although this hypothesis could be relaxed. . The mothership and the drone must travel together from $orig$ to the first launching point. Similarly, after the drone visits the last target location, the mothership and the drone must meet at the final rendezvous location before traveling together back to $dest$. The first launching location and final rendezvous location are allowed to be $orig$ and $dest$, respectively, but it is not mandatory. For the ease of presentation, in this paper we will assume that $orig$ and $dest$ are the same location. However, all results extend easily to the case that $orig$ and $dest$ are different locations.\\
% \noindent
% The goal is to find a minimum time path that begins at $orig$, ends at $dest$, and where
% every $g \in \mathcal G$ is visited by the drone.\\
% \noindent
% Depending on the assumptions made on the movements of the mothership vehicle this problem gives rise to two different versions: a) the mothership vehicle can move freely on the continuous space (all terrain ground vehicle, boat on the water or aircraft vehicle); and b) the mothership vehicle must move on a road network (that is, it is a normal truck or van). In the former case, that we will call All terrain Mothership-Drone Routing Problem with Graphs (\AMD), each launch and rendezvous location may be chosen from a continuous space (the Euclidean 2-or-3 dimension space). In the latter case, that we will call Network Mothership-Drone Routing Problem with Graphs (\NMD) from now on, each launch and rendezvouz location must be chosen on a given graph embedded in the considered space. For the sake of presentation and length  of the paper, we will focus in this paper, mainly, on the first model \AMD. The second model, namely \NMD, is addressed using similar techniques but providing slightly less details.




==> Mothership Drone/description_old.tex <==
\section{Description of the Problem}
\JP{In the Mothership and Drone Routing Problem with Graphs (MDRPG), there is one mothership (the base vehicle) and one drone and the problem consists on the coordination between the drone and the base vehicle to minimize the total distance travelled by both vehicles. \JP{In this case, for the sake of simplicity, we assume that there exist no obstacles to prevent drone travel from moving in straight line segments. Nevertheless, that extension is interesting to be further considered although is beyond the scope of this paper.}

The mothership and the drone begin at a starting location, denoted $orig$. There exists a set $\mathcal G$ of target locations modeled by graphs that must be visited by the drone. The natural application for this situation comes from road or wired network inspection. For each stage $t \in \{1, \ldots, |\mathcal G|\}$, we require that the drone is launched from the current mothership location, that at stage $t$ is a decision variable denoted by $x_L^t$, flies to one of the graphs that has to be visited $g$, traverses the required portion of $g$ and then returns to the current position of the mothership, that most likely is different from the launching point $x_L^t$, and  that is another decision variable denoted by $x_R^t$. Once all targets graphs have been visited, the mothership and drone return to a final location (depot), denoted by $dest$.

Let $g = (V_G, E_G)$ be a graph in $\mathcal G$ whose total length is denoted by $\mathcal L(g)$ and $i_g$ that denotes the edge $e$ of this graph $g$. This edge is parametrized by its endpoints $B^{i_g}, C^{i_g}$ and its length $\|\overline{B^{i_g}C^{i_g}}\|$ is denoted by $\mathcal L(i_g)$. For each line segment, we assign a binary variable $\mu^{i_g}$ that indicates whether or not the drone visits the segment $i_g$ and define entry and exit points $(R^{i_g}, \rho^{i_g})$ and $(L^{i_g}, \lambda^{i_g})$, respectively, that determine the portion of the edge visited by the drone. }

We have considered two modes of visit to the targets graphs $g\in \mathcal{G}$:
\begin{itemize}
    \item Visiting a percentage $\alpha^{i_g}$ of each edge $i_g$ which can be modeled by using the following constraints:
    \begin{equation}\label{eq:alphaE}\tag{$\alpha$-E}
    |\lambda^{i_g} - \rho^{i_g}|\mu^{i_g}\geq \alpha^{i_g}, \quad \forall i_g, \forall g.
    \end{equation}
    \item Visiting a percentage $\alpha_g$ of the total length of the graph:
    \begin{equation}\label{eq:alphaG}\tag{$\alpha$-G}
    \sum_{i_g} \mu^{i_g}|\lambda^{i_g} - \rho^{i_g}|\mathcal L(i_g) \geq \alpha_g\mathcal L(g), \quad \forall g
    \end{equation}
    where $\mathcal L(g)$ denotes the total length of the graph.
\end{itemize}

\bigskip

In both cases, we need to introduce a binary variable that determines the traveling direction on the edge $i_g$ as well as the definition of the parameter values $\nu_\text{min}^{i_g}$ and $\nu_\text{max}^{i_g}$ of the access and exit points to that segment. Then, for each edge $i_g$, the absolute value constraint \eqref{eq:alphaE} can be represented by:

\begin{equation}\label{eq:alpha-E}\tag{$\alpha$-E}
 \mu^{i_g}|\rho^{i_g}-\lambda^{i_g}|\geq \alpha^{i_g} \Longleftrightarrow
 \left\{
 \begin{array}{ccl}
  \rho^{i_g} - \lambda^{i_g}                       & =    & \nu_\text{max}^{i_g} - \nu_\text{min}^{i_g}                                     \\
  \nu_\text{max}^{i_g}                         & \leq & 1-\text{entry}^{i_g}                                    \\
  \nu_\text{min}^{i_g}                      & \leq & \text{entry}^{i_g},                                        \\
  \mu^{i_g}(\nu_\text{max}^{i_g} + \nu_\text{min}^{i_g} ) & \geq & \alpha^{i_g}
  \\
 \end{array}
 \right.
\end{equation}

The linearization of \eqref{eq:alphaG} is similar to \eqref{eq:alphaE} by changing the last inequality in \eqref{eq:alpha-E} for

\begin{equation}\label{eq:alpha-G}\tag{$\alpha$-G}
\sum_{i_g} \mu^{i_g}(\nu_\text{max}^{i_g} + \nu_\text{min}^{i_g})\mathcal L(i_g)\geq \alpha_g\mathcal L(g).
\end{equation}

\JP{In our model wlog, we assume  that the mothership and drone do not need to arrive at a rendezvous location at the same time: the
faster arriving vehicle may wait for the other at the rendezvous location. In addition, we also assume that vehicles move at constant speeds, although this hypothesis could be relaxed. The mothership travels at $v_M$ speed whereas the drone has a speed of $v_D$ > $v_M$. The mothership and the drone must travel together from $orig$ to the first launch location. Similarly, after the drone visits the last target location, the mothership and the drone must meet at the final rendezvous location before traveling together back to $dest$. The first launch location and final rendezvous location are allowed to be $orig$ and $dest$, respectively, but it is not mandatory. For the ease of presentation, in this paper we will assume that $orig$ and $dest$ are the same location. However, all results extend easily to the case that $orig$ and $dest$ are different locations.

The goal is to find a minimum time path that begins at $orig$, ends at $dest$, and where
every $g \in \mathcal G$ is visited by the drone.

Depending on the assumptions made on the movements of the mothership vehicle this problem gives rise to two different versions: a) the mothership vehicle can move freely on the continuous space (all terrain ground vehicle, boat on the water or flying vehicle); and b) the mothership vehicle must move on a travel network (that is, it is a normal truck or van). In the former case, that we will call All terrain Mothership-Drone Routing Problem with Graphs (\AMD), each launch and rendezvous location may be chosen from a continuous space (the Euclidean 2-or-3 dimension space). In the latter case, that we will call Network Mothership-Drone Routing Problem with Graphs (\NMD) from now on, each launch and rendezvouz location must be chosen on a given graph embedded in the considered space. For the sake of presentation and length  of the paper, we will focus in this paper, mainly, on the first model \AMD. The second model, namely \NMD, is addressed using similar techniques but providing slightly less details.}




==> Mothership Drone/experiments.tex <==
\newpage
\section{Experimental results}


% \begin{figure}[h!]
% \begin{center}
%  \includegraphics[width=1\linewidth]{Grid_generation.png}
% \end{center}
% \end{figure}
\noindent
In this section we discuss the experimental results obtained testing the formulations presented in Section \ref{Form} and the matheuristic procedure proposed in Section \ref{Math} on a testbed of instances. In particular, we consider instances like the ones used in \cite{art:Amorosi2021} where the targets, to be visited by the drones, are represented by grid graphs.
This set consists of 5 instances of respectively 5 and 10 target graphs, with different cardinality of the set of nodes. More precisely, each instance is composed of 20$\%$ graphs with 4 nodes, 20$\%$ graphs of 6 nodes, 20$\%$ graphs of 8 nodes and 20$\%$ graphs of 10 nodes. Moreover, we assume that the velocity of the drones is twice that of the mothership and that a random percentage of each target graph, or of each of its edges, must be visited by the fleet of drones.\\
We consider in our experiments that the number of drones varies between 1 and 3 and that the drones
endurance (expressed as maximum time that the drone can operate when it is fully recharged) ranges between 20 and 60.
Table \ref{table:tab1} reports a summary of the characteristics of our instances.

\renewcommand{\arraystretch}{0.7}
\begin{table}[!h]
\caption{Instances parameter values}
\centering
\footnotesize
\begin{tabular}{l | c }
\hline
\# Targets & (5,10)\\
\hline
\# Drones &	(1,2,3)\\
\hline
\# Vertices & (4,6,8,10,12)\\
\hline
Drone endurance & (20,30,40,50,60)\\
\hline
$\%$ target (edge) & random variable
\end{tabular}
\label{table:tab1}
\end{table}

\noindent
Table \ref{table:tab2} reports the results obtained solving the \AMD model on the instances previously described, by adopting the commercial solver Gurobi. We consider the exact solution both providing and not providing an initial solution computed by the matheuristic described in Section \ref{Math}. More precisely, the first column of Table \ref{table:tab2} indicates the number of target graphs to be visited by the fleet of drones, the second column reports the capacity of the drones, the third column distinguishes between the visit of a percentage of each edge (e) and the percentage of each target graph (g). The fourth column reports the size of the fleet of drones. Thus, for each combination of the listed parameters, we summarize the average percentage gap of the solution obtained within the time limit set equal to 2 hours. We report respectively average percentage gap with initialization by the solution provided by the matheuristic, solution time, in seconds, of the matheuristic and average gap without initialization by the solution obtained by the matheuristic.\\
We can observe that the value of the average percentage gap ranges between a minimum of 66.9\% and a maximum of 97.43\%. This shows that the model is hard to be solved even on small size instances. Moreover, we can see that in most of the cases, the average percentage gap associated with the variant of the model consisting in visiting a given percentage of each edge, is higher than the one associated with the variant imposing to visit a given percentage of each target graph. Another thing that we can observe is that the average percentage gap increases with the number of drones and decreases with the drone endurance.\\
As regards the number of target graphs, we can see that by increasing it from 5 to 10, the exact method, without initialization by the solution obtained with the matheursitic, becomes even harder. Indeed, the red entries of the table mean that some instances could not find a feasible solution within the time limit (note that in the brackets we indicate the number of these instances). The number of not solvable instances increases with the number of drones. Moreover, for the minimum level of endurance, the exact solution of the model without initialization provided by the matheuristic, does not provide any solution, within the time limit, for instances with 10 graphs and 2 or 3 drones.\\
Considering the comparison with the exact method starting from the solution provided by the matheuristic, we can note that the values of average percentage gap are very close to the ones related to the exact solution method without initialization. Thus the initialization does not speed up the convergence of the solver. However, we can see that the matheuristic is always able to find a feasible solution of the problem, even for the cases in which the solver is not.\\
Moreover, the average solution times of the matheuristic range between a minimum of 37 seconds to a maximum of 3 minutes. They increase with the drone capacity for the variant of the model in which a given percentage of each edge must be visited, while they decrease by increasing the number of drones for the variant of the model in which a given percentage of each target graph must visited. By increasing the number of target graphs from 5 to 10, the average solution times of the matheuristics become more than double for both model variants.
Summing up, the results obtained show that the exact solution method given by solving the formulation is very challenging even for small size instances. However, exploiting it, the matheuristic is able to provide  solutions for all instances rather quickly.


%\begin{table}[!h]
%\caption{Comparison between exact solution with and without initialization by the matheuristic solution}
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c c c c c c c c c|}
%\hline
%\multirow{3}{*}{$\bm{|\mathcal{G}|}$} & \multirow{3}{*}{$\bm{N^d}$}  & \multirow{3}{*}{\textbf{v.t.}} & \multicolumn{9}{|c|}{\textbf{$\#$ drones}} \\
%\cline{4-12}
%& & & \multicolumn{3}{c|}{1} & \multicolumn{3}{c|}{2} & \multicolumn{3}{c|}{3}\\
%\cline{4-12}
%& & &  $\%$Gap (i) & TimeH & $\%$Gap (wi) & $\%$Gap (i) & TimeH & $\%$Gap (wi)& $\%$Gap (i) & TimeH & $\%$Gap (wi)\\
%\hline
%\multirow{5}{*}{\midrule 5} & \multirow{2}{*}{20} & e & 82,63 & 61,56 & 81,70 & 91,57 &	63,80 &	90,61 &	93,06 &	60,87 &	90,93\\
%&  & g & 79,09 & 44,97 & 79,63 & 89,03 & 37,32 & 91,85 & 94,00 & 39,05 & 95,80\\
%\cline{2-12}
%& \multirow{2}{*}{30} & e & 82,70 &	65,21 &	80,17 &	85,14 &	64,41 &	82,21 &	91,90 &	63,34 &	90,12\\
%& & g & 75,80 &	55,77 &	71,19 &	84,36 &	44,36 &	88,27 &	91,02 &	44,59 &	91,39\\
%\cline{2-12}
%& \multirow{2}{*}{40} & e & 80,94 &	68,81 &	77,98 &	83,44 &	64,80 &	82,16 &	91,24 &	63,19 &	86,25\\
%& & g & 74,47 &	43,92 &	73,46 &	81,21 &	38,27 &	84,35 &	85,34 &	37,51 &	89,63\\
%\cline{2-12}
%& \multirow{2}{*}{50} & e & 76,87 &	66,67 &	74,41 &	81,12 &	63,86 &	79,57 &	85,11 &	63,51 &	86,16\\
%& & g & 70,58 &	43,42 &	66,90 &	80,96 &	43,98 &	88,84 &	80,49 &	44,35 &	82,81\\
%\cline{2-12}
%& \multirow{2}{*}{60} & e & 76,39 &	67,78 &	71,61 &	81,63 &	66,08 &	79,84 &	83,82 &	64,40 &	82,06\\
%& & g & 78,17 &	44,69 &	72,79 &	79,35 &	40,63 &	86,55 &	81,74 &	50,01 &	84,66\\
%\hline
%\multirow{5}{*}{10} & \multirow{2}{*}{20} & e & 82,56 &	137,93 &	84,91 &	92,30 &	128,53 & - & 94,73 & 124,44 & -\\
%&  & g & 81,00 & 119,20 & \textcolor{red}{84,08 (2)} & 89,88 & 83,50 & \textcolor{red}{96,64 (2)} & 96,44 & 70,00 & \textcolor{red}{97,43 (3)}\\
%\cline{2-12}
%& \multirow{2}{*}{30} & e & 80,60 &	159,00 & 80,93 & 87,11 & 132,15 & \textcolor{red}{87,58 (3)} &	94,56 &	127,35 & \textcolor{red}{92,85 (2)}\\
%& & g & 79,93 &	132,67 & \textcolor{red}{82,70 (1)} & 86,32 & 80,29 & \textcolor{red}{86,13 (3)} & 91,12 &	76,72 &	\textcolor{red}{89,74 (1)}\\
%\cline{2-12}
%& \multirow{2}{*}{40} & e & 79,05 &	191,37 & 78,07 & 85,11 & 131,26 &	84,33 &	91,88 &	132,10 & \textcolor{red}{88,61 (1)}\\
%& & g & 80,23 &	115,00 & 79,64 & 87,31 & 68,39 & \textcolor{red}{84,57 (3)} & 96,09 &	69,40 &	\textcolor{red}{91,86 (1)}\\
%\cline{2-12}
%& \multirow{2}{*}{50} & e & 81,49 &	188,32 & 77,81 & 87,72 & 134,01 &	\textcolor{red}{85,51 (1)} &	92,68 &	132,82 & \textcolor{red}{90,79 (3)}\\
%& & g & 79,92 &	87,23 &	80,38 &	82,80 &	66,14 &	\textcolor{red}{84,00 (3)} &	92,48 &	64,94 &	\textcolor{red}{91,96 (2)}\\
%\cline{2-12}
%& \multirow{2}{*}{60} & e & 83,79 &	155,27 & 81,57 & 85,91 & 131,94 &	\textcolor{red}{82,96 (2)} &	92,24 &	130,11 & \textcolor{red}{86,58 (3)}\\
%& & g & 77,57 &	97,89 &	78,46 &	86,94 &	76,53 &	\textcolor{red}{88,29 (2)} &	94,31 &	69,53 &	\textcolor{red}{92,23 (3)}\\
%\hline
%\end{tabular}
%\label{table:tab2}
%\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h!]
\centering
\caption{Comparison between exact solution with and without initialization by the matheuristic solution}
\label{table:tab2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|ccc|ccc|ccc|}
\hline
 &  &  & \multicolumn{9}{c|}{\textbf{\# drones}} \\ \cline{4-12} 
 &  &  & \multicolumn{3}{c|}{1} & \multicolumn{3}{c|}{2} & \multicolumn{3}{c|}{3} \\ \cline{4-12} 
\multirow{-3}{*}{$\bm{|\mathcal G|}$} & \multirow{-3}{*}{$\bm{N^d}$} & \multirow{-3}{*}{\textbf{v.t.}} & \% Gap (i) & TimeH & \% Gap (wi) & \% Gap (i) & TimeH & \% Gap (wi) & \% Gap (i) & TimeH & \% Gap (wi) \\ \hline
 &  & e & 82,63 & 61,56 & 81,70 & 91,57 & 63,80 & 90,61 & 93,06 & 60,87 & 90,93 \\ \cline{3-3}
 & \multirow{-2}{*}{20} & g & 79,09 & 44,97 & 79,63 & {\color[HTML]{333333} 89,03} & 37,32 & 91,85 & 94,00 & 39,05 & 95,80 \\ \cline{2-12} 
 &  & e & 82,70 & 65,21 & 80,17 & 85,14 & 64,41 & 82,21 & 91,9 & 63,34 & 90,12 \\ \cline{3-3}
 & \multirow{-2}{*}{30} & g & 75,80 & 55,77 & 71,19 & 84,36 & 44,36 & 88,27 & 91,02 & 44,59 & 91,39 \\ \cline{2-12} 
 &  & e & 80,94 & 68,81 & 77,98 & 83,44 & 64,80 & 82,16 & 91,24 & 63,19 & 86,25 \\ \cline{3-3}
 & \multirow{-2}{*}{40} & g & 74,47 & 43,92 & 73,46 & 81,21 & 38,27 & 84,35 & 85,34 & 37,51 & 89,63 \\ \cline{2-12} 
 &  & e & 76,87 & 66,67 & 74,41 & 81,12 & 63,86 & 79,57 & 85,11 & 63,51 & 86,16 \\ \cline{3-3}
 & \multirow{-2}{*}{50} & g & 70,58 & 43,42 & 66,90 & 80,96 & 43,98 & 88,84 & 80,49 & 44,35 & 82,81 \\ \cline{2-12} 
 &  & e & 76,39 & 67,78 & 71,61 & 81,63 & 66,08 & 79,84 & 83,82 & 64,40 & 82,06 \\ \cline{3-3}
\multirow{-10}{*}{5} & \multirow{-2}{*}{60} & g & 78,17 & 44,69 & 72,79 & 79,35 & 40,63 & 86,55 & 81,74 & 50,01 & 84,66 \\ \hline
 &  & e & 82,56 & 137,93 & 84,91 & 92,30 & 128,53 & - & 94,73 & 124,44 & - \\ \cline{3-3}
 & \multirow{-2}{*}{20} & g & 81,00 & 119,20 & {\color[HTML]{FE0000} 84,08 (2)} & 89,88 & 83,50 & {\color[HTML]{FE0000} 96,64 (2)} & 96,44 & 70,00 & {\color[HTML]{FE0000} 97,43 (3)} \\ \cline{2-12} 
 &  & e & 80,60 & 159,00 & 80,93 & 87,11 & 132,15 & {\color[HTML]{FE0000} 87,58 (3)} & 94,56 & 127,35 & {\color[HTML]{FE0000} 92,85 (2)} \\ \cline{3-3}
 & \multirow{-2}{*}{30} & g & 79,93 & 132,67 & {\color[HTML]{FE0000} 82,70 (1)} & 86,32 & 80,29 & {\color[HTML]{FE0000} 86,13 (3)} & 91,12 & 76,72 & {\color[HTML]{FE0000} 89,74 (1)} \\ \cline{2-12} 
 &  & e & 79,05 & 191,37 & 78,07 & 85,11 & 131,26 & 84,33 & 91,88 & 132,10 & {\color[HTML]{FE0000} 88,61 (1)} \\ \cline{3-3}
 & \multirow{-2}{*}{40} & g & 80,23 & 115,00 & 79,64 & 87,31 & 68,39 & {\color[HTML]{FE0000} 84,57 (3)} & 96,09 & 69,40 & {\color[HTML]{FE0000} 91,86 (1)} \\ \cline{2-12} 
 &  & e & 81,49 & 188,32 & 77,81 & 87,72 & 134,01 & {\color[HTML]{FE0000} 85,51 (1)} & 92,68 & 132,82 & {\color[HTML]{FE0000} 90,79 (3)} \\ \cline{3-3}
 & \multirow{-2}{*}{50} & g & 79,92 & 87,23 & 80,38 & 82,80 & 66,14 & {\color[HTML]{FE0000} 84,00 (3)} & 92,48 & 64,94 & {\color[HTML]{FE0000} 91,96 (2)} \\ \cline{2-12} 
 &  & e & 83,79 & 155,27 & 81,57 & 85,91 & 131,94 & {\color[HTML]{FE0000} 82,96 (2)} & 92,24 & 130,11 & {\color[HTML]{FE0000} 86,58 (3)} \\ \cline{3-3}
\multirow{-10}{*}{10} & \multirow{-2}{*}{60} & g & 77,57 & 97,89 & 78,46 & 86,94 & 76,53 & {\color[HTML]{FE0000} 88,29 (2)} & 94,31 & 69,53 & {\color[HTML]{FE0000} 92,23 (3)} \\ \hline
\end{tabular}%
}
\end{table}

\noindent
We show in Figure \ref{fig:heatmap} the relationship between the objective function values of the problem and the number of available drones and their capacity. This figure reports the average objective values of all the instances with three target graphs varying the number of drones in $\{1,2,3\}$ and their endurance (capacity) in $\{10,20,30,40,50,60\}$. The darker the color intensity the smaller the objective value. As expected, our experiment confirms that both, a greater number of drones and larger endurance reduce total length of the mothership route.

\begin{figure}[h!]
\includegraphics[width=\linewidth]{heatmap.png}
\caption{Heatmap of objective function values depending on number of drones and drone capacities. The darker the color intensity the smaller the objective value. \label{fig:heatmap}}
\end{figure}
\noindent
%In order to test the performances of the matheuristic proposed in Section \ref{Math}, we coded it in Python and we run it on the same sets of instances (Grid and Delaunay) on which the three formulations have been solved. Table \ref{table:tab3} reports for each instance, numbered from 0 to 4, distinguishing between Grid and Delauney, respectively, the best objective function provided by the best formulation, the objective function provided by the matheuristic and the associated CPU time. As already noticed from Table \ref{table:tab2}, for grid graph instances, SEC formulation has the best behaviour, with the exception of the instance number 3 for which the MTZ provides a smaller value of the objective function. As for the Delaunay graph instances, MTZ is the best formulation, but also in this case there is an exception on the instance number 2 for which SEC formulation returns a smaller value of the objective function.\\
%The results show that the matheuristic returns a solution with value of the objective function that is higher than the one provided by the SEC formulation on grid instances. However, these values are smaller than the ones provided by the Stages and the MTZ formulations. Moreover, the saving in terms of resolution time is very significant as the maximum CPU time is less than 1 minute.  As regards the Delaunay instances, the matheuristic performances are even better, as it finds a solution that is better than the best one provided by the MTZ formulation and in a resolution time that is at most 28 minutes. 



%\renewcommand{\arraystretch}{0.7}
%\begin{table}[!h]
%\caption{Heuristic performances}
%\centering
%\footnotesize
%\begin{tabular}{c | c c c | c c c}
%\hline
%\textbf{\#}  & \multicolumn{3}{c}{\textbf{Grid}} &  \multicolumn{3}{c}{\textbf{Delauney}} \\
 % \hline
% &Best Obj & Obj Heuristic &CPU Time &Best Obj & Obj Heuristic & CPU Time \\
%\hline
%0 &	1087,87	& 1117,83 &	50,99 &	947,01 &	934,46 &	52,49\\
%1 &	1100,38	& 1319,64 &	24,64 &	986,22 &	 938,68	& 72,73\\
%2 &	1350,67	& 1126,35 &	46,06 &	888,48 &	865,66 &	1073,80\\
%3 &	1218,66	& 1476,36 &	27,18 &	1249,69 &	1154,62 &	1703,33\\
%4 &	1297,77	& 1424,37 &	40,91 &	1239,93	 & 1184,67 &	81,15\\
%    \hline
%\end{tabular}
%\label{table:tab3}
%\end{table}


\noindent
%We performed a second set of experiments by observing that, even if there are small differences between the SEC and the MTZ formulations depending on the type of instances, their performances are comparable.
%Thus, in the rest of the tests we focused on the MTZ formulation. We compared its performances, with or without providing the initial solution found by the matheuristic, on a set of larger instances. More precisely, we generated 20 instances with targets represented by grid graphs and 20 instances with targets represented by Delauney graphs. The instances of each typology are split in 4 groups of 5 instances each, consisting respectively of 5, 10, 15 and 20 targets to be visited.
%In each instance the same percentage of graphs ($20\%$) has respectively 4, 6, 8, 10 and 12 nodes. 
%Moreover, we assumed that the origin coincides with the destination in all instances and we randomly generated with uniform distribution between 0 and 1, two values representing the percentage of each edge and of each graph to be visited.
%As regards the speeds, we set the speed of the drone three times the one of the mothership.
%We run the MTZ formulation by adopting Gurobi, setting a time limit of 7200 sec. for each instance.
%On the same instances also the matheuristic has been applied. Note that, in order to define a stopping rule for the exact resolution of the AMDRPG model within the matheuristic procedure (STEP 3 and STEP 4), we set the maximum number of solutions generated by the solver equal to five.
%For each instance, the solution provided by the matheuristic has been then used to initialize the exact resolution of the MTZ formulation in order to try to speed up the resolution process.
%Table \ref{table:tab4} shows the results of the comparison between the exact resolution of the formulation with and without initialization. In the first column, named List, we report the size of the instances in terms of number of targets to be visited (0, 1, 2 and 3 identifies instances respectively with 5, 10, 15 and 20 graphs).The second column refers to the two variants of the model, that is, a given percentage of each edge of the targets (e) or a given percentage of each target (g) must be visited by the drone. The other columns report respectively the average percentage gap of the solutions found within the time limit starting from the initial solution provided by the matheuristic, the average running time of the matheuristic and the average percentage gap of the solutions found within the time limit without initialization. These information are reported for both Grid and Delauney instances.

%\renewcommand{\arraystretch}{0.7}
%\begin{table}[!h]
%\caption{Comparison between exact resolution with and without initialization}
%\centering
%\footnotesize
%\begin{tabular}{c c | c c c | c c c}
%\hline
% &  & \multicolumn{3}{c}{\textbf{Grid}} &  \multicolumn{3}{c}{\textbf{Delauney}} \\
%\hline
% List &  $\%$  & $\%$ Gap (i) & Time$\_$h & $\%$ Gap (ni)  & $\%$ Gap (i) & Time$\_$h &  $\%$ Gap (ni)\\
%\hline
%\multirow{}{}{0} & e & 0.72 & 105.12 & 0.73 & 0.78 & 154.92 & 0.74\\
%& g & 0.55 & 58.92 & 0.54 & 0.62 & 92.64 & 0.67\\
%\hline
%\multirow{}{}{1} & e & 0.76 & 241.99 & 0.76 & 0.80 & 314.69 & 0.79\\
%& g & 0.71 & 182.61 & 0.70 & 0.74 & 353.04 & 0.75\\
%\hline
%\multirow{}{}{2} & e & 0.76 & 367.69 & 0.76 & 0.80 & 447.61 & 0.80 \\
%& g & 0.71 & 326.49 & 0.72 & 0.76 & 429.16 & 0.76\\
%\hline
%\multirow{}{}{3} & e & 0.75 & 481.68 & 0.74 & 0.80 & 514.98 & 0.76^*\\
%& g & 0.71 & 492.27 & 0.70 & 0.77 & 582.90 & 0.77\\
%    \hline
%\end{tabular}
%\label{table:tab4}
%\end{table}

\noindent
%From Table \ref{table:tab4} we can notice that in most of the cases the average gaps associated with the solution found within the time limit, with and without initialization by the solution found by the matheuristic, are the same or very close (note that in the last column the $*$ indicates that only one instance has been solved within the time limit).
%As regards the running time of the matheuristic, we can see also from the boxplots in Figure \ref{fig:1}, that it increases with the number of targets to be visited both for Grid and Delaunay instances. Considering the model variants based on the minimum percentage of each edge or each graph to visit, we can observe that for Grid instances the average running time of the model imposing a minimum percentage of each edge to be visited, is greater than the one associated with the other variant, with the exception of the instances of biggest size (List=3). \\
\noindent
%The boxplots in Figure \ref{fig:2} represent the percentage gap of the solution provided by the matheuristic with respect to the one provided by the exact resolution of the MTZ model within the time limit, with initialization by the solution found by the matheuristic. From them we can notice that the gap increases with the size both for Grid and Delaunay instances but it is always less than 0.5$\%$.  
%Figure \ref{fig:3} shows the percentage gap of the solution provided by the exact resolution of the MTZ formulation within the time limit without the initialization, with respect to the one found with the initialization. This gap is very close to 0 both for Grid and Delaunay instances. Only for the biggest size we observe values ranging between 0.1$\%$ and 0.6$\%$. These observations suggest that, even if the initialization of the model by the solution provided by the matheuristic does not speed up the convergence to the optimal solution, the matheuristic provides solutions of very good quality. Indeed, it generates in less than 10 minutes solutions that are very close to the ones provided by the model within 2 hours.\\


%\begin{figure}[htp]% [H] is so declass\'e!
%\centering
%\begin{minipage}{0.45\textwidth}
%\includegraphics[width=\textwidth]{time_h.png}
%\caption{Matheuristic running time}
%\label{fig:1}
%\end{minipage}\hfill
%\begin{minipage}{0.45\textwidth}
%\includegraphics[width=\textwidth]{improved_gap.png}
%\caption{Matheuristic improved gap}
%\label{fig:2}
%\end{minipage}\par
%\vskip\floatsep% normal separation between figures
%\includegraphics[width=0.45\textwidth]{differencewithwithout.png}
%\caption{Improved gap of MTZ formulation with and without initialization}
%\label{fig:3}
%\end{figure}



%\noindent
%As regards the \NMD \xspace problem, we generated three sets of instances with targets represented by grid graphs considering different structures of the polygonal network where the mothership can move.
%In particular, we defined a first set of instances where the mothership network is represented by a graph of 6 nodes with a tree structure with origin of the path of the base vehicle different from the destination.
%A second set of instances involving a mothership network consisting in a complete graph of 4 vertices with origin of the path of the base vehicle different from the destination.  
%A third set of instances characterized by star graphs of 7 nodes representing the mothership network, where the origin coincides with the destination and it is located at the centre of the star. We generated 10 instances for each of these three classes, 5 of them with 5 targets and 5 with 10 targets to be visited. 
%Moreover, as for the AMDRPG, for each of these 10 instances we randomly generated two values representing the percentage of each edge and of each graph that must be visited by the drone.
%We run on these sets of instances both Stages and MTZ formulations. Table \ref{table:tab5} summarizes the results obtained comparing them. The first column identifies the size of the instances, similarly to Table \ref{table:tab4}, (0 for instances with 5 targets and 1 for instances with 10 targets).
%The second column distinguishes between minimum percentage of each edge (e) or of each graph (g) to be visited by the drone.
%The remaining columns refer to the three different class  of instances described above (1 for the networks with a tree structure, 2 for complete networks and 3 for start networks).
%For each of these sets of instances the average percentage gap of the solutions found within the time limit of 7200 sec. by the two formulations (Stages and MTZ) is reported.


%\renewcommand{\arraystretch}{0.7}
%\begin{table}[!h]
%\caption{Comparison between formulations of \NMD}
%\centering
%\footnotesize
%\begin{tabular}{c c | c c | c c | c c}
%\hline
% & Net Struct  & \multicolumn{2}{c}{1} &  \multicolumn{2}{c}{2}  & \multicolumn{2}{c}{3}\\
%\hline
%List & $\%$ &  Stages  & MTZ & Stages & MTZ  & Stages & MTZ\\
%\hline
%\multirow{}{}{0} & e & 0.89 & 0.33 & 0.88 & 0.24 & 0.87 & 0.39\\
%& g & 0.86 & 0.29 & 0.89 & 0.18 & 0.90 & 0.42\\
%\hline
%\multirow{}{}{1} & e & 0.92 & 0.43 & 0.92 & 0.33 & 0.92 & 0.46\\
%& g & 0.91 & 0.36 & 0.92 & 0.23 & 0.92 & 0.39\\
%\hline
%\end{tabular}
%\label{table:tab5}
%\end{table}

\noindent
%We can observe that for each class of instances and model variants, based on the percentage of each edge or each graph to be visited, the MTZ formulation performs better than the Stages one. In all the cases the percentage average gap associated with the MTZ formulation is one third or half of that associated with the Stages formulation. For this reason, in the following tests, related to the comparison between the exact resolution of the \NMD\xspace  model with and without the initialization by the solution found by the matheuristic, we focused only on the MTZ formulation.\\
%Table \ref{table:tab6} summarizes the results of this comparison distinguishing again between the different network structures (columns labelled 1, 2 and 3), the different size (rows labelled 0 and 1) characterizing the instances and model variants (minimum percentage of each edge (e) or each graph (g) to be visited). For each combination of network structure, size and model variant we reported the average percentage gap with initialization ($\%$ Gap (i)), the solution time of the matheuristic (T$\_$h) and the average percentage gap without initialization by the solution found by the matheuristic ($\%$ Gap (ni))

%\renewcommand{\arraystretch}{0.8}
%\begin{table}[!h]
%\caption{Comparison between exact resolution with and without initialization of \NMD}
%\centering
%\scriptsize
%\begin{tabular}{c c | c c c | c c c | c c c}
%\hline
% & Net Struct  & \multicolumn{3}{c}{1} &  \multicolumn{3}{c}{2}  & \multicolumn{3}{c}{3}\\
%\hline
%List &  $\%$  & $\%$ Gap (i) & T$\_$h & $\%$ Gap (ni)  & $\%$ Gap (i) & T$\_$h &  $\%$ Gap (ni) & $\%$ Gap (i) & T$\_$h &  $\%$ Gap (ni)\\
%\hline
%\multirow{}{}{0} & e & 0.32 & 109.96 & 0.33 & 0.24 & 207 & 0.24 & 0.39 & 177.57 & 0.39\\
%& g & 0.30 & 110.92 & 0.29 & 0.18 & 163.36 & 0.18 & 0.45 & 149.68 & 0.42\\
%\hline
%\multirow{}{}{1} & e & 0.48 & 1030.64 & 0.43 & 0.39 & 802.3 & 0.33 & 0.53 & 770.05 & 0.46\\
%& g & 0.33 & 479.36 & 0.36 & 0.35 & 639.09 & 0.23 & 0.42 & 689.51 & 0.39\\
%\hline
%\end{tabular}
%\label{table:tab6}
%\end{table}

\noindent
%We can observe that, similarly to the AMDRPG problem, the average gaps associated with the solution found within the time limit, with and without initialization by the solution found by the matheuristic, are very close. Considering the average running time we can notice that the \NMD\xspace  problem is more challanging to be solved with respect to the AMDRPG. It increases very fast with the size of the instances especially for the case in which the network where the mothership moves has a tree structure. Moreover, as for the Grid instances in the continuous case, the model variant imposing a minimum percentage of each edge to be visited takes more time to be solved.

%\begin{figure}
%\centering
%\includegraphics[width=5cm]{improved_gap_ND.png}
%\caption{Matheuristic improved gap for \NMD}
%\label{fig:4}
%\end{figure}
\noindent
%The boxplots showed in Figure \ref{fig:4} report the percentage gap of the solution provided by the matheuristic with respect to the one provided by the exact resolution of the MTZ model within the time limit, with initialization by the solution found by the matheuristic.
%We can notice that, excluding the outliers, this gap ranges between 0$\%$ and 0.7$\%$ and its lowest values are observed for the instances in which the network where the mothership moves has a star structure (green boxplots). 
%From the previous observations, similarly to the AMDRPG, we can conclude that the behaviour of the matheuristic is very good in terms of quality of the solutions provided, even if the initialization of the MTZ model does not help in speeding up the convergence to the optimal solution. 













==> Mothership Drone/formulations.tex <==
\subsection{Mixed Integer Non Linear Programming Formulations}\label{Form}
% \JP{In this section we present a MINLP formulation for the (\AMD). Let us denote by $\mathcal T$ the set of stages/tasks that the mothership and the fleet of drones have to carry out. These stages are visits to the different graphs in $\mathcal G$ with the required constraints. A stage $t\in\mathcal T$ is referred to as the operation in which the mothership launches some drones from a taking-off location, denoted by $x_L^t$ and later it takes them back on a rendezvous location $x_R^t$. Here, it is important to realize that both locations $x^L_t$ and $x^R_t$ must be determined in the continuous space where the mothership is assumed to move. Note that $|\mathcal T|\leq|\mathcal G|$, since it is assumed that, for each stage, at least one drone must be launched. Clearly, the distance $d_{LR}^t$ traveled by the base vehicle for the stage $t$, i.e., to go from $x_L^t$ to $x_R^t$ is
% $$d_{LR}^t=\|x_L^t - x_R^t\|,$$
% where $\|\cdot\|_2$ denoted the Euclidean distance,  although this assumption can be extended to any $l_p$ norm, $1\leq p\leq \infty$.} 
\noindent
In this section we present a MINLP mathematical programming formulation for the \AMD %\;\hspace{-2}%  
that can be used to solve medium size instances of this problem.
\noindent
As mentioned in Section \ref{section:desc}, we assume that the mothership is allowed to move freely in a continuous space that for the sake of presentation we  assume to be $\mathbb R^2$. Here, distances are measured by the Euclidean norm, $\|\cdot\|_2$, although this assumption can be extended to any $l_p$ norm, $1\leq p\leq \infty$ (see \cite{Blanco2017}).
\noindent
In the following, we introduce the parameters or input data that formally describe the problem and that are summarized in Table \ref{table:t1}.

 \begin{table}[!h]
\scriptsize
\centering
%\color{blue}
\begin{tabular}{ | l | }
\hline
\textbf{Problem Parameters}\\
\hline
$orig$: coordinates of the point defining the origin of the mothership path (or tour).\\
$dest$: coordinates of the point defining the destination of the mothership path (or tour).\\
$\mathcal{G}$: set of the target graphs.\\
$g = (V_g, E_g)$: set of nodes and edges of each target graph $g \in \mathcal{G}$.\\
$\mathcal{L}(e_g)$: length of edge $e$ of graph $g \in \mathcal{G}$.\\
$\mathcal{L}(g)=\sum_{e_g\in E_g} \mathcal L(e_g)$: total length of the graph $g\in\mathcal G$.\\
$B^{e_g}, C^{e_g}$: coordinates of the endpoints of edge $e$ of graph $g \in \mathcal{G}$.\\
$\alpha^{e_g}$: percentage of edge $e$ of graph $g \in \mathcal{G}$ that must be visited.\\
$\alpha^{g}$: percentage of graph $g \in \mathcal{G}$ that must be visited.\\
$v_D$: drone speed.\\
$v_M$: mothership speed.\\
$N^d$: drone endurance. \\
$M$: big-M constant.\\
\hline
\end{tabular}
\caption{Nomenclature for AMMDRPG}
\label{table:t1}
\end{table}

\begin{table}[h!]
%\tiny
\scriptsize
\centering
%\color{blue}
\begin{tabular}{|l|}
\hline 
\textbf{Binary and Integer Decision Variables}\\
\hline
$\mu^{e_g} \in \{0,1\} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$): equal to 1 if edge $e$ of graph $g$ (or a portion of it) is visited by the drone,\\ \hspace*{1cm} and  0 otherwise.\\
$\text{entry}^{e_g} \in \{0,1\} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$): auxiliary binary variable used for linearizing expressions.\\
$u^{e_{g}td} \in \{0,1\} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$) $\: \forall t \in \mathcal T \: \forall d \in \mathcal D$: equal to 1 if the drone $d$ enters in graph $g$ by the edge $e_g$ at stage $t$,\\ \hspace*{1cm} 0 otherwise.\\
$z^{e_{g}e^{'}_{g}} \in \{0,1\} \:\: \forall e_g, e_g' \in E_g$ ($g \in \mathcal{G}$): equal to 1 if the drone goes from $e_g$ to $e^{'}_{g}$, 0 otherwise.\\
$v^{e_{g}td} \in \{0,1\} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$) $\: \forall t \in\mathcal T \: \forall d \in \mathcal D$: equal to 1 if the drone $d$ exits from graph $g$ by $e_g$ at stage $t$,\\ \hspace*{1cm} 0 otherwise.\\
$s^{e_g},\; \forall e_g \in E_g$ ($g \in \mathcal{G}$): integer non negative variable representing the order of visit of the edge $e$ of graph $g$.\\
\hline
\textbf{Continuous Decision Variables}\\
\hline
$\rho^{e_g} \in [0,1]$ and $\lambda^{e_g} \in [0,1] \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$): defining the entry and exit points on $e_g$.\\
$\nu_\text{min}^{e_g}$ and $\nu_\text{max}^{e_g} \in [0,1] \forall e_g \in E_g$ ($g \in \mathcal{G}$): auxiliary variables used for linearizing expressions.\\
$x_L^t \:\: \forall t \in\mathcal T$: coordinates representing the point where the mothership launches the drone at stage $t$.\\
$x_R^t \:\: \forall t \in\mathcal T$: coordinates representing the point where the mothership retrieves the drone at stage $t$.\\
$R^{e_g} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$): coordinates representing the entry point on edge $e$ of graph $g$.\\
$L^{e_g} \:\: \forall e_g \in E_g$ ($g \in \mathcal{G})$: coordinates representing the exit point on edge $e$ of graph $g$.\\
$d_L^{e_gtd} \geq 0, \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$) $\forall t \in\mathcal T \:\forall d\in\mathcal D$: representing the distance travelled by the drone $d$ from the launching\\
\hspace*{1cm} point $x_L^t$ on the mothership at stage $t$ to the first visiting point $R^{e_g}$ on $e_g$.\\
$d^{e_ge^\prime_g} \geq 0, \:\: \forall e_g, e^\prime_g \in E_g $ ($g \in \mathcal{G}$): representing the distance travelled by the drone from the launching\\
\hspace*{1cm} point $L^{e_g}$ on $e_g$ to the rendezvous point $R^{e^\prime_g}$ on $e^\prime_g$.\\
$d^{e_g} \geq 0, \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$): representing the distance travelled by the drone from the rendezvous\\
\hspace*{1cm} point $R^{e_g}$ to the launching point $L^{e_g}$ on $e_g$. \\
$d_R^{e_gtd} \geq 0 \:\: \forall e_g \in E_g$ ($g \in \mathcal{G}$) $\forall t \in\mathcal T\:\forall d\in\mathcal D$: representing the distance travelled by the drone $d$ from the last\\
\hspace*{1cm} visiting point $L^{e_g}$ on $e_g$ to the rendezvous point $x_R^t$ on the mothership at stage $t$.\\
$d_{LR}^t \geq 0 \:\: \forall t \in\mathcal T$: representing the distance travelled by the mothership from the \\
\hspace*{1cm} launching point $x_L^t$ to the rendezvous point $x_R^t$ at stage $t$.\\
$d_{RL}^t \geq 0 \:\: \forall t \in\mathcal T$: representing the distance travelled by the mothership from the \\ 
\hspace*{1cm} rendezvous point $x_R^t$ at stage $t$ to the launching point $x_L^{(t+1)}$ at the stage $t+1$.\\
\hline
\end{tabular}
\caption{Decision Variables for AMMDRPG}
\label{table:t2}
\end{table}

\noindent
To represent the movement of the drone within a graph $g\in\mathcal G$, we proceed to introduce some notation related to $g$.
Let $g = (V_g, E_g)$ be a graph in $\mathcal G$ whose total length is denoted by $\mathcal L(g)$. Here, $V_g$ denotes the set of nodes and $E_g$ denotes the set of edges connecting pairs of nodes. Let $e_g$ be the edge $e$ of the graph $g \in G$ and let $\mathcal  L(e_g)$ be its length. Each edge $e_g$ is parameterized by its endpoints $B^{e_g}= (B^{e_g}(x_1), B^{e_g}(x_2))$ and $C^{e_g}= (C^{e_g}(x_1), C^{e_g}(x_2))$ and we can compute its length $\mathcal L(e_g) =\|C^{e_g} -  B^{e_g}\|$.

% We shall refer to $e_g$  as a generic edge $e$ of this graph $g$. The  edge $e_g$ is determined by its endpoints $B^{e_g}, C^{e_g}$ and its length $\|\overline{B^{e_g}C^{e_g}}\|$ is denoted by $\mathcal L(e_g)$. For each edge $e_g$, we assign a binary variable $\mu^{e_g}$ that indicates whether or not the drone visits $e_g$. In addition, for each edge $e_g$ we define an entry $(R^{e_g}, \rho^{e_g})$ and an exit point $(L^{e_g}, \lambda^{e_g})$, being $\rho^{e_g}$ and $\lambda^{e_g}$ the values in the parametrization of the edge $e_g$ where the drone enters and leaves the edge. \\
\noindent
As discussed in Section \ref{section:desc}, we consider two modes of visit to the target graphs $g\in \mathcal{G}$:
\begin{itemize}
    \item Visiting a percentage $\alpha^{e_g}$ of each edge $e_g$ which can be modeled by using the following constraints:
    \begin{equation}\label{eq:alphaE}\tag{$\alpha$-E}
    |\lambda^{e_g} - \rho^{e_g}|\mu^{e_g}\geq \alpha^{e_g}, \quad \forall e_g\in E_g.
    \end{equation}
    \item Visiting a percentage $\alpha^g$ of the total length of the graph:
    \begin{equation}\label{eq:alphaG}\tag{$\alpha$-G}
    \sum_{e_g\in E_g} \mu^{e_g}|\lambda^{e_g} - \rho^{e_g}|\mathcal L(e_g) \geq \alpha^g\mathcal L(g).
    \end{equation}
   % \CV{where $\mathcal L(g)$ denotes the total length of the graph., this is mentioned before}
\end{itemize}

\bigskip
\noindent
In both cases the corresponding constraints are nonlinear. In order to linearize them, we need to introduce a binary variable $\text{entry}^{e_g}$ that determines the traveling direction on the edge $e_g$ as well as the definition of the parameter values $\nu_\text{min}^{e_g}$ and $\nu_\text{max}^{e_g}$ of the access and exit points to that segment. Then, for each edge $e_g$, the absolute value constraint \eqref{eq:alphaE} can be represented by:

\begin{equation}\label{eq:alpha-E}\tag{$\alpha$-E}
 \mu^{e_g}|\rho^{e_g}-\lambda^{e_g}|\geq \alpha^{e_g} \Longleftrightarrow
 \left\{
 \begin{array}{ccl}
  \rho^{e_g} - \lambda^{e_g}                       & =    & \nu_\text{max}^{e_g} - \nu_\text{min}^{e_g},                                     \\
  \nu_\text{max}^{e_g}                         & \leq & 1-{\text{entry}^{e_g}},                                   \\
  \nu_\text{min}^{e_g}                      & \leq & {  \text{entry}^{e_g}},                                        \\
  \mu^{e_g}(\nu_\text{max}^{e_g} + \nu_\text{min}^{e_g} ) & \geq & \alpha^{e_g}.
  \\
 \end{array}
 \right.
\end{equation}

\noindent
The linearization of \eqref{eq:alphaG} is similar to \eqref{eq:alphaE} by changing the last inequality in \eqref{eq:alpha-E} by

\begin{equation}\label{eq:alpha-G}\tag{$\alpha$-G}
\sum_{e_g\in E_g} \mu^{e_g}(\nu_\text{max}^{e_g} + \nu_\text{min}^{e_g})\mathcal L(e_g)\geq \alpha^g\mathcal L(g).
\end{equation}

\noindent
To model this problem, we use stages identified with the order in which the different elements in the problem are visited. Let us denote by $\mathcal T$ the set of stages/tasks that the mothership and the fleet of drones have to carry out. These stages are visits to the different graphs in $\mathcal G$ with the required constraints. A stage $t\in\mathcal T$ is referred to as the operation in which the mothership launches some drones from a taking-off location, denoted by $x_L^t$ and later it takes them back on a rendezvous location $x_R^t$. Here, it is important to realize that both locations $x_L^t$ and $x_R^t$ must be determined in the continuous space where the mothership is assumed to move. Note that $|\mathcal T|\leq|\mathcal G|$, since it is assumed that, for each stage, at least one drone must be launched.
\noindent
For each stage $t\in\mathcal T$, each one of the drones launched from the mothership must follow a path starting from and returning to the mothership, while visiting the required edges of $g$. According to the notation introduced above, we write this generic path in the following form:

$$
x_L^t\rightarrow R^{e_g}\rightarrow L^{e_g}\rightarrow\ldots\rightarrow R^{e^\prime_g}\rightarrow L^{e^\prime_g}\rightarrow \ldots \rightarrow R^{e''_g} \rightarrow x_R^t\rightarrow x_L^{t+1}.
$$


\begin{figure}[h!]
\centering
\includegraphics[width=0.95\linewidth]{figures/figure_latex.png}
\caption{Example illustrating the meaning of the launching  (L) and retrieving (R) points.}
\label{fig:illustrative}
\end{figure}

\noindent
Figure \ref{fig:illustrative} shows an example of the notation over a configuration with four target graphs that have four nodes and four edges. Here, it is supposed that the number of available drones is two. %: one with six nodes and 7 edges and the other one with four nodes and edges%. 
The mothership begins at its starting point $orig$. Then, it moves to $x_L^1$ where two drones are launched to visit two graphs. There, each drone follows a route (represented by the orange and green paths) that ensures the coverage of $50 \%$ of each edge of the graph. The red dots on the visited graphs are the intermediate points $R^{e_g}$ and $L^{e_g}$ used by the drones in their visit to the edges of the different graphs. After finishing the visit of the first two graphs the drones return to the point $x_R^1$ from where they are launched again to visit the remaining two graphs. Once these graphs are visited, the drones return to the mothership at the rendezvous point $x_R^2$ and then the mothership ends its route at the destination point $dest$.


% \JP{ ************************ 

% TO BE INSERTED: An example showing the notation with a figure...  Please Carlos insert something similar to what we use in the previous paper (JUSTO dixit)

%      ************************}
\noindent
To include the definition of these paths in our mathematical programming formulation we need to make decisions to choose:
\begin{itemize}
    \item The optimal assignment of drones for visiting graphs in a given stage $t$.
    \item The optimal order to visit the edges of each graph in its corresponding stage.
\end{itemize}

% Binary variables
% Thus, to this end one can define the following binary variables:
\noindent
We model the route that the drone follows by using the binary variables $u^{e_gtd}$, $z^{e_ge^\prime_g}$ and $v^{e_gtd}$ defined in Table \ref{table:t2}.


% \begin{itemize}
%   \item $u^{{e_g}td} = 1$ if the visit of graph $g$ is done at stage $t$ by the drone $d$ and it starts from edge $e_g$.
%   \item $v^{{e_g}td}= 1$ if the visit of graph $g$ that is done by drone $d$ at stage $t$ finishes in the edge $e_g$.
%   \item $z^{e_ge'_g}= 1$ if the drone moves from edge $e_g$ to $e'_g$ while visiting the graph $g$.
% \end{itemize}

% By using these binary variables, we can model the route that follows the drone:
\begin{align}
    \sum_{g\in \mathcal G}\sum_{e_g\in E_g} \sum_{d\in\mathcal D} u^{e_gtd} & \leq 1, &\forall t\in \mathcal T, \label{st:DEnt}\\%\tag{DEn}\\
    \sum_{g\in\mathcal G}\sum_{e_g\in E_g} \sum_{d\in\mathcal D} v^{e_gtd} & \leq 1, &\forall t\in \mathcal T, \label{st:DExt}\\%\tag{DEx}\\
    \sum_{e_g\in E_g} \sum_{t\in \mathcal T} \sum_{d\in\mathcal D} u^{e_gtd} & = 1, &\forall g\in\mathcal G, \label{st:DEng}\\%\tag{D
    \sum_{e_g\in E_g} \sum_{t\in \mathcal T} \sum_{d\in\mathcal D} v^{e_gtd} & = 1, &\forall g\in\mathcal G, \label{st:DExg}\\%\tag{D
    \sum_{e_g\in E_g} u^{e_gtd} & = \sum_{e_g\in E_g} v^{e_gtd}, &\forall g\in\mathcal G, \forall t\in \mathcal T, \forall d\in\mathcal D, \label{st:Duv}\\%\tag{D
     \sum_{t\in \mathcal T} \sum_{d \in \mathcal D} u^{e_gtd} + \sum_{e^\prime_g\in E_g} z_g^{e^\prime_ge_g} & = \mu^{e_g}, &\forall e_g\in E_g:g\in\mathcal G, \label{st:DInu}\\
     \sum_{t\in \mathcal T} \sum_{d \in \mathcal D} v^{e_gtd} + \sum_{e^\prime_g\in E_g} z_g^{e_ge^\prime_g} & = \mu^{e_g}, &\forall e_g\in E_g:g\in\mathcal G. \label{st:DInv}
\end{align}

\noindent 
Inequalities \eqref{st:DEnt} and \eqref{st:DExt} state that for each stage at most one drone can be launched and retrieved for performing an operation.  Constraints \eqref{st:DEng} and \eqref{st:DExg} assure that each graph is visited at some stage $t$ by some drone $d$. Equations \eqref{st:Duv} ensure that the operation of entering and exiting from the graph $g$ occurs in the same stage $t$ and is done by the same drone $d$. Constraints \eqref{st:DInu} state that 
if edge $e$ of graph $g$ is visited by the drone $d$, one of two alternative situations must occur: either $e$ is the first edge of graph $g$ visited by the drone $d$ at stage $t$, or edge $e$ is visited by the drone $d$ after visiting another edge $e^\prime$ of graph $g$. Similarly, constraints \eqref{st:DInv} state that if edge $e$ of graph $g$ is visited by the drone $d$, either $e$ is the last edge of graph $g$ visited by the drone at stage $t$, or the drone $d$ must move to another edge $e^\prime$ of graph $g$ after visiting edge $e$.
% Constraints \eqref{st:DInu} (resp. \eqref{st:DInv}) state that if the edge $e_g$ is visited, $\mu^{e_g}=1$, then either the drone enters coming from (leaves to) the mothership, $\sum_{t\in \mathcal T} \sum_{d \in \mathcal D} u^{e_gtd}=1$ ($\sum_{t\in \mathcal T} \sum_{d \in \mathcal D} v^{e_gtd}=1$), or it enters from (leaves to) another edge $e^\prime_g$, $\sum_{e^\prime_g\in E_g} z_g^{e^\prime_ge_g}=1$ ($\sum_{e^\prime_g\in E_g} z_g^{e_ge^\prime_g} =1$).

% A first attempt to model this problem uses stages identified with the order in which the different elements in the problem are visited. We identify each visit to one of the target graphs with a stage of the process. Then, by using the notation below, we define the stages set associated to graphs $T:=\{1,\ldots,|\mathcal G|\}$ and those associated to the launching and rendezvous points including $orig$ and $dest$ $T'=\{0,\ldots,|\mathcal G|+1\}$. For each stage $t\in T$, the drone follows the following path starting from the mothership, visiting the required edges of $g$ and returning to the mothership:

% $$
% x_L^t\rightarrow R^{e_g}\rightarrow L^{e_g}\rightarrow\ldots\rightarrow R^{e^\prime_g}\rightarrow L^{e^\prime_g}\rightarrow \ldots \rightarrow R^{e''_g} \rightarrow x_R^t\rightarrow x_L^{t+1}.
% $$

% This path calls in a natural way for the definition of binary variables that choose:
% \begin{itemize}
%     \item The optimal order to visit each graph $g\in\mathcal G$. In other words, defining the sequence of the stages.
%     \item The optimal order to visit the edges of each graph in its corresponding stage.
% \end{itemize}

% Thus, to this end one can define the following binary variables:
% \begin{itemize}
%     \item $u^{e_gt} = 1$ if the drone enters by the segment $e_g$ at the stage $t$.
%     \item $z^{e_ge^\prime_g} = 1$ if the drone goes from the segment $e_g$ to the segment $e^\prime_g$.
%     \item $v^{e_gt} = 1$ if the drone exits the graph by the segment $e_g$ at the stage $t$.
% \end{itemize}

% By using these binary variables, we can model the route that follows the drone:
% \begin{align}
%     \sum_{g\in \mathcal G}\sum_{e_g\in E_g} u^{e_gt} & = 1, &\forall t\in T \label{st:DEnt}\\%\tag{DEn}\\
%     \sum_{g\in\mathcal G}\sum_{e_g\in E_g} v^{e_gt} & = 1, &\forall t\in T \label{st:DExt}\\%\tag{DEx}\\
%     \sum_{e_g\in E_g} \sum_{t\in T} u^{e_gt} & = 1, &\forall g\in\mathcal G \label{st:DEng}\\%\tag{D
%     \sum_{e_g\in E_g}\sum_{t\in T} v^{e_gt} & = 1, &\forall g\in\mathcal G \label{st:DExg}\\%\tag{D
%     \sum_{e_g\in E_g} u^{e_gt} & = \sum_{e_g\in E_g} v^{e_gt}, &\forall g\in\mathcal G, \forall t\in T \label{st:Duv}\\%\tag{D
%     \sum_{e^\prime_g\in E_g} z_g^{e^\prime_ge_g} + \sum_{t\in T} u^{e_gt} & = \mu^{e_g}, &\forall e_g\in E_g:g\in\mathcal G \label{st:DInu}\\
%     \sum_{e^\prime_g\in E_g} z_g^{e_ge^\prime_g} + \sum_{t\in T} v^{e_gt} & = \mu^{e_g}, &\forall e_g\in E_g:g\in\mathcal G \label{st:DInv}
% \end{align}

% \noindent
% Equations \eqref{st:DEnt} and \eqref{st:DExt} state that in each stage the drone visits (enter and exit, respectively) only one graph. Constraints \eqref{st:DEng} and \eqref{st:DExg} assure that each graph is visited at some stage. Constraints \eqref{st:DInu} (resp. \eqref{st:DInv}) state that the number of exterior edges plus the number of interior edges that enter (resp. exit) to the edge $e_g$ is given by $\mu^{e_g}$.

\subsubsection*{Elimination of subtours}
\noindent
In order to represent actual routes of the drones over the target graphs, subtours cannot be allowed. Note that subtours would represent fake operations since they would allow free jumps of the drone between different routes at no time. To prevent the existence of subtours within each graph $g\in \mathcal G$ that the drone must visit, one can include, among others, either the compact formulation that uses the Miller-Tucker-Zemlin constraints (MTZ) or the subtour elimination  constraints (SEC).\\
\noindent
For the MTZ formulation, we use the continuous variables $s^{e_g}$, defined in Table \ref{table:t2}, that state the order to visit the edge $e_g$ and set the following constraints for each $g\in\mathcal G$:

\begin{align}
    s^{e_g} - s^{e^\prime_g} + |E_g|z^{e_ge^\prime_g} & \leq |E_g| - 1  , &\quad\forall e_g \neq e_g'\in E_g, \tag{MTZ$_1$} \label{MTZ1}\\
    0 & \leq s^{e_g} \leq |E_g| - 1, &\quad\forall e_g\in E_g.\tag{MTZ$_2$}\label{MTZ2}
\end{align}

\noindent
Alternatively, we can also use the family of subtour elimination constraints for each $g\in\mathcal G$:
\begin{equation}\tag{SEC}\label{SEC}
    \sum_{e_g, e^\prime_g \in S} z_g^{e_ge^\prime_g} \leq |S| - 1, \quad \forall S\subset E_g.
\end{equation}

\noindent
%(Copiado del XPPN)
Since there is an exponential number of SEC constraints, when we implement this formulation we need to perform a row generation procedure including constraints whenever they are required by a separation oracle. To find SEC inequalities, as usual, we search for disconnected components in the current solution. Among them, we choose the shortest subtour found in the solution to be added as a lazy constraint to the model.\\

\noindent
 The goal of the \AMD\xspace is to find a feasible solution that minimizes the total distance traveled by the mothership. To account for the different distances among the decision variables of the model we need to set the continuous variables $d_L^{e_gtd}$, $d^{e_g}$, $d^{e_ge^\prime_g}$, $d_R^{e_gtd}$, $d_{RL}^t$ and $d_{LR}^t$, defined in Table \ref{table:t2}. This can be done by means of the following constraints:
 
 %define the following instrumental variables:
% \begin{itemize}
%     \item $d_L^{e_gtd} = \|x_L^t - R^{e_g}\|$. Distance traveled by the drone $d$ from the launching point at the stage $t$ to the first visiting point in the segment $e_g$.
%     \item $d^{e_ge^\prime_g} = \|R^{e_g} - L^{e^\prime_g}\|$. Distance traveled by the drone $d$ from the launching point in $e_g$ to the next rendezvous point in the following edge $e^\prime_g$ of the graph $g$.
%     \item $d^{e_g} = \|R^{e_g} - L^{e_g}\|$. Distance traveled by the drone from the retrieving point  to the next launching point in $e_g$.
%     \item $d_R^{e_gtd} = \|L^{e_g} - x_R^t\|$. Distance traveled by the drone $d$ from the launching point in the last segment $e_g$ visited of the graph $g$ to the retrieving point on the mothership at the stage $t$.
%     \item $d_{LR}^t = \|x_L^t - x_R^t\|$. Distance traveled by the mothership from the launching point to the retrieving point at the stage $t$.
%     \item $d_{RL}^t = \|x_R^t - x_L^{t+1}\|$. Distance traveled by the mothership from the retrieving point at stage $t$ to the launching point at stage $t+1$.
% \end{itemize}

\begin{align*}
\|x_L^t- R^{e_g}\| & \leq  d_L^{e_gtd},  &\quad \forall e_g:g\in \mathcal{G}, \forall t\in \mathcal T, \forall d\in\mathcal D, \tag{DIST$_{1}$-t} \label{eq:d1}\\
\|R^{e_g}- L^{e_g}\| & \leq  d^{e_g},  &\quad \forall e_g:g\in \mathcal{G}, \tag{DIST$_{2}$-t} \label{eq:d2}\\
\|R^{e_g}- L^{e^\prime_g}\| & \leq  d^{e_ge^\prime_g}, &\quad \forall e_g\neq e_g'\in E_g:g\in \mathcal{G}, \tag{DIST$_{3}$-t} \label{eq:d3}\\
\|L^{e_g}- x_R^t\| & \leq  d_R^{e_gtd}, &\quad \forall e_g:g\in \mathcal{G},\forall t\in T, \forall d\in\mathcal D, \tag{DIST$_{4}$-t} \label{eq:d4}\\
\|x_R^t- x_L^{t+1}\| & \leq  d_{RL}^t, & \quad \forall t\in \mathcal T, \tag{DIST$_{5}$-t} \label{eq:d5}\\
\|x_L^t- x_R^t\| & \leq  d_{LR}^t, & \quad \forall t\in \mathcal T. \tag{DIST$_{6}$-t} \label{eq:d6}\\
\end{align*}

\noindent
The coordination between the drones and the mothership must ensure that the time spent by the drone $d$ to visit the graph $g$ at the stage $t$ is less than or equal to the time that the mothership needs to move from the launching point to the retrieving point during the stage $t$. To this end, we need to define the following coordination constraint for each graph $g\in \mathcal G$, stage $t\in \mathcal T$ and drone $d\in\mathcal D$:

\begin{equation}\tag{DCW}\label{DCW}
\frac{1}{v_D}\left(\sum_{e_g\in E_g} u^{e_gtd}d_L^{e_gtd} + \sum_{e_g, e^\prime_g\in E_g}z^{e_ge^\prime_g}d^{e_ge^\prime_g} + \sum_{e_g\in E_g} \mu^{e_g}d^{e_g} + \sum_{e_g\in E_g} v^{e_gtd}d_R^{e_gtd}\right) \leq \frac{d_{LR}^t}{v_M} + M(1 - \sum_{e_g\in E_g} u^{e_gtd}).
\end{equation}


\noindent
Eventually, we have to impose that the tour of the mothership, together with the drones, starts from the origin $orig$ and ends at the destination $dest$. To this end, we define the following constraints:

\begin{align*}
x_L^0 & =  orig,  \tag{ORIG$_1$} \label{eq:O1} \\
x_R^0 & =  orig,  \tag{ORIG$_2$} \label{eq:O2} \\
x_L^{|\mathcal{G}|+1} & =  dest,  \tag{DEST$_1$} \label{eq:D1} \\
x_R^{|\mathcal{G}|+1} & =  dest.  \tag{DEST$_2$} \label{eq:D2} 
\end{align*}

\noindent
Note that, since the objective function of this problem minimizes the right-hand-side of \eqref{DCW}, this constraint will become an equality and we can model the time capacity constraint for a particular stage $t\in \mathcal T$ by limiting the distance traveled by the mothership for this task $t$:

\begin{equation}\tag{Capacity}\label{CAP}
    d_{LR}^t \leq N^d.
\end{equation}



% \end{itemize}


% A natural approach to model this problem is to consider stages which are identified with the targets that the drone has to visit. This way the problem needs to considers $|\mathcal{G}|$ stages that are indexed by $t=1,\ldots, |\mathcal{G}|$. To provide a valid formulation for the model under this approach, we introduce the following variables:
% \begin{itemize}

\noindent
Therefore, putting together all the constraints introduced before, the following formulation minimizes the overall distance traveled by the mothership ensuring the coordination with the fleet of drones while guaranteeing the required coverage of the target graphs.
\begin{mini*}|s|
 {}{\sum_{t\in \mathcal T} (d_{RL}^t + d_{LR}^t)}{}{} \label{AMMDRPG} \tag{AMMDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{MTZ1}-\eqref{MTZ2}} \text{ or }  \eqref{SEC}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\eqref{DCW}}{}{}
 \addConstraint{\eqref{CAP}}{}{}
 \addConstraint{\eqref{eq:d1}-\eqref{eq:d6}}{}{}
 \addConstraint{\eqref{eq:O1}-\eqref{eq:D2}.}{}{}
\end{mini*}

\noindent
The objective function accounts for the distances traveled by the mothership. Constraints \eqref{st:DEnt}-\eqref{st:DInv} models the route followed by the drone $d\in\mathcal D$, \eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} ensure that the displacement of the drone $d\in\mathcal D$ assigned to the target graph $g\in\mathcal G$ is a route, \eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G} defines what is required in each visit to a target graph. Finally, constraints (\ref{eq:d1})-(\ref{eq:d6}) set the variables $d_L^{e_gtd}$, $d^{e_g}$, $d^{e_ge^\prime_g}$, $d_R^{e_gtd}$, $d_{RL}^t$ and $d_{LR}^t$, defined in Table \ref{table:t2}, which represent Euclidean distances needed in the model. \\

% Then, the next six constraints model Euclidean distances needed in the model. \\
% \noindent
% Observe that we are assuming constant velocities for the mothership $v_M$ and the drone $v_D$.\\
\noindent
Note that, to deal with the bilinear terms of \eqref{DCW}, we use McCormick's envelopes to linearize them by adding variables $p\geq 0$  representing the products and introducing the following constraints:
\begin{align*}
    p & \leq  M z, \\
    p & \leq  d, \\
    p & \geq m z, \\
    p & \geq d - M(1 - z),
\end{align*}
where $m$ and $M$ are, respectively, the lower and upper bounds of the distance variable $d$. These bounds will be adjusted for each bilinear term in Section \ref{bounds}.

\subsection{The \AMD\xspace without synchronisation}\label{amdasyn}
\noindent
In the \eqref{AMMDRPG} formulation, we assume that every drone is launched and retrieved in the same stage. In this subsection, we show how this assumption can be relaxed.
We consider a variant of the model presented in Section \ref{Form}, in which we assume that the mothership can retrieve one drone in a stage different from the one in which it has been launched. That is, the mothership can move to another point to launch a new drone without having  retrieved the one that was launched before.

%\JP{
%{\color{atomictangerine} \bf *********************************

%TO BE INSERTED: We must include an example showing the difference with the syncronized model where the objective value is smaller and the solution pattern takes advantange of the asyncronus mode of operation.

% **********************************}
% }
\noindent
To deal with this extension, we do not need to define new variables since it is possible to use the same variables that were used in the previous model. First of all, constraint \eqref{st:Duv} must be changed to:
\begin{equation}\label{constraint:Duv-S}
    \sum_{e_g\in E_g} u^{e_gtd} -  \sum_{e_g\in E_g} \sum_{t'\geq t} v^{e_gt'd}=0, \quad\forall  g\in\mathcal G,\forall t\in\mathcal T, \forall d\in\mathcal D.
\end{equation}
This equation states that, if the graph $g$ is assigned to the drone $d$ at the stage $t$, there is another stage $t' \geq t$ in which the drone must come back to the mothership.
\noindent
In addition, if the drone $d$ is launched at $t_1$ and retrieved at $t_2$, this drone cannot be used in any intermediate stage. Hence, for each graph $g\in\mathcal G$ and drone $d\in\mathcal D$ the following constraints must be satisfied:
\begin{equation}\label{constraint:u-S}
 \sum_{e_g\in E_g}\sum_{t=t_1+1}^{t_2} u^{e_gtd}\leq M(2-\sum_{e_g\in E_g} u^{e_gt_1d} - \sum_{e_g\in E_g}v^{e_gt_2d}),\quad t_1 < t_2,
\end{equation}
\begin{equation}\label{constraint:v-S}
 \sum_{e_g\in E_g}\sum_{t=t_1}^{t_2-1} v^{e_gtd}\leq M(2-\sum_{e_g\in E_g} u^{e_gt_1d} - \sum_{e_g\in E_g}v^{e_gt_2d}),\quad t_1< t_2.
\end{equation}
\noindent
Moreover, the coordination constraint \eqref{DCW} must be modified to consider the general case in which the stages of launching and retrieving can be different. For each $t_1<t_2$ and $\forall g\in\mathcal G,\forall d\in\mathcal D$:
\begin{tiny}
\begin{align}\tag{DCW-S}\label{constraint:DCW-S}
\frac{1}{v_D}\left(\sum_{e_g\in E_g} u^{e_gt_1d}d_L^{e_gt_1d} + \sum_{e_g, e^\prime_g\in E_g}z^{e_ge^\prime_g}d^{e_ge^\prime_g} + \sum_{e_g\in E_g} \mu^{e_g}d^{e_g} + \sum_{e_g\in E_g} v^{e_gt_2d}d_R^{e_gt_2d}\right) \leq & \frac{\sum_{t=t_1}^{t_2}d_{LR}^t}{v_M} + \frac{\sum_{t=t_1}^{t_2-1}d_{RL}^t}{v_M} \nonumber
\\  &  + M(2 - \sum_{e_g\in E_g} u^{e_gt_1d} - \sum_{e_g\in E_g} v^{e_gt_2d}).  \nonumber
\end{align}
\end{tiny}

\noindent
This inequality takes into account the total time the mothership needs to go from the launching point $x_L^{t_1}$ to the rendezvous point $x_R^{t_2}$ when  the drone $d$ is chosen to visit the graph $g\in\mathcal G$ and this operation begins at stage $t_1$ and ends at $t_2$.
\noindent
Finally, we present a result that links the two models presented before. Note that the only difference that solutions can have between these models is that, for the non-synchronized case, the mothership can launch a second drone sequentially before retrieving another one that was launched before. Figure \ref{fig:proof1} shows a solution that is not possible for the model with synchronization. Indeed, we can see that a first drone is launched at $x_L^1$ to visit $P_1$ that is retrieved at $x_R^1$. However, the mothership has launched another drone at $x_L^2$ that goes visiting $P_2$ before having retrieved the first drone. Obviously, this solution does not satisfy the assumption in the synchronized model. 


\begin{figure}[h!]
    \centering
    \includegraphics[width = 0.7\linewidth]{proof1.PNG}
    \caption{The mothership launches two drones sequentially}
    \label{fig:proof1}
\end{figure}

\noindent
In order to present our next result, wlog,  we restrict ourselves to the degenerate case where graphs reduce to points. The reader may note that we could reduce the general case to this one reducing the available capacity so that is possible to traverse the required percentage of these graphs. We simplify the proof considering a generic solution between two consecutive target points.


\begin{theorem}
Let $x_L^1$, $x_L^2$ (resp. $x_R^1$, $x_R^2$) be the launching (resp. rendezvous) points associated to the visit of the target points $P_1$ and $P_2$. If there exist two points $x_L$ and $x_R$ verifying 
$$
 \left\{
 \begin{array}{ccl}
  \dfrac{\|x_L-x_R\|}{v_C} & \leq    & \dfrac{\|x_L - P_1\| + \|P_1 - x_R\|}{v_D}, \\
  \dfrac{\|x_L-x_R\|}{v_C} & \leq    & \dfrac{\|x_L - P_2\| + \|P_2 - x_R\|}{v_D}, \\
  \dfrac{\|x_L-x_R\|}{v_C} & \leq   & N^d, \\
  \|x_L-x_R\| & \leq & \|x_L^1 - x_L^2\| + \|x_L^2- x_R^1\| + \|x_R^1-x_R^2\|,
 \end{array}
 \right.
$$

\noindent then the contribution of this partial route to the optimal objective value will be the same in both models.
\end{theorem}

\begin{proof}
Note that in the considered configuration, the order of visit to the points $P_1$ and $P_2$ is fixed and then, the binary variables in the model are fixed in this case. Thus, the only difference that the two models can have are the location of the launching and rendezvous points. Hence, the only constraints that are involved are those related to these points. These are the conditions in the statement: The first two are the \eqref{DCW} inequalities. The third one is the \eqref{CAP} constraint and the last one ensures that the distance traveled by the mothership in the synchronized model is smaller than or equal to the distance assumed in the non-synchronized solution described in the statement. Therefore, the conclusion follows.

\end{proof}

% Note that this result states necessary and sufficient conditions to obtain the same solution for the two models.



%(Meto restricción de capacidad? para hacer experimentos puede complicarse)

% $$
% e=(i, j) \ni x_R^t \rightarrow V_i \vee V_j \rightarrow \ldots \rightarrow V_k \rightarrow \ldots \rightarrow V_{i'} \rightarrow x_L^{t+1} \in (i',j')=e'
% $$

% The design of these paths obeys to define binary variables that decide which vertices are selected in each stage $t$: 

==> Mothership Drone/formulations_old.tex <==
\section{Mixed Integer Non Linear Programming Formulations}
In this section we present alternative MINLP formulations for the (\MDR) depending on the nature of  the mothership  that will be compared computationally in later sections. We start analyzing first the situation where the mothership moves in a continuous space, namely the (\AMD). 
%We shall address later the second model (\NMD). As it will clear later, we will elaborate from the previous model modifying some intrinsic conditions that characterize each problem.

A first attempt to model this problem uses stages identified with the order in which the different elements in the problem are visited. We identify each visit to one of the target graphs with a stage of the process. Then, by using the notation below, in each stage $t\in \{1,\ldots,|\mathcal G|\}$, the drone follows the following path starting from the mothership, visiting the required edges of $G$ and returning to the mothership:

$$
x_L^t\rightarrow R^{i_g}\rightarrow L^{i_g}\rightarrow\ldots\rightarrow R^{j_g}\rightarrow L^{j_g}\rightarrow \ldots \rightarrow R^{u(g)} \rightarrow x_R^t\rightarrow x_L^{t+1}.
$$

This path calls in a natural way for the definition of binary variables that choose:
\begin{itemize}
    \item The optimal order to visit each graph $g\in\mathcal G$. In other words, defining the sequence of the stages.
    \item The optimal order to visit the edges of each graph in its corresponding stage.
\end{itemize}

Thus, to this end one can define the following binary variables:
\begin{itemize}
    \item $u^{i_gt} = 1$ if the drone enters by the segment $i_g$ at the stage $t$.
    \item $z^{i_gj_g} = 1$ if the drone goes from the segment $i_g$ to the segment $j_g$.
    \item $v^{i_gt} = 1$ if the drone exits the graph by the segment $i_g$ at the stage $t$.
\end{itemize}

By using these binary variables, we can model the route that follows the drone:
\begin{align}
    \sum_{i_g} u^{i_gt} & = 1, &\quad\forall t \label{st:DEnt}\\%\tag{DEn}\\
    \sum_{i_g} v^{i_gt} & = 1, &\quad\forall t \label{st:DExt}\\%\tag{DEx}\\
    \sum_{i_g, t} u^{i_gt} & = 1, &\quad\forall g \label{st:DEng}\\%\tag{D
    \sum_{i_g, t} v^{i_gt} & = 1, &\quad\forall g \label{st:DExg}\\%\tag{D
    \sum_{i_g} u^{i_gt} & = \sum_{i_g} v^{i_gt}, &\quad\forall g, t \label{st:Duv}\\%\tag{D
    \sum_{j_g} z_g^{j_gi_g} + \sum_{t} u^{i_gt} & = \mu^{i_g}, &\quad\forall i_g \label{st:DInu}\\
    \sum_{j_g} z_g^{i_gj_g} + \sum_{t} v^{i_gt} & = \mu^{i_g}, &\quad\forall i_g \label{st:DInv}
\end{align}

Equations \eqref{st:DEnt} and \eqref{st:DExt} state that in each stage the drone visits (enter and exit, respectively) only one graph. Constraints \eqref{st:DEng} and \eqref{st:DExg} assure that each graph is visited at some stage. Constraints \eqref{st:DInu} (resp. \eqref{st:DInv}) say that the number of exterior edges plus the number of interior edges that enter (resp. exit) to the edge $i_g$ is given by $\mu^{i_g}$.

\subsubsection*{Elimination of subtours}
To prevent the existence of subtours within each graph $g\in \mathcal G$ that the drone must visit, one can include, among others, either the compact formulation that uses the Miller-Tucker-Zemlin constraints or the subtour elimination  constraints (SEC).

For the MTZ formulation, we define the continuous variables $s^{i_g}$ that indicate the order to visit the edge $i_g$ and establish the following constraints for each $g\in\mathcal G$:

\begin{align}
    s^{i_g} - s^{j_g} + |E_g|z^{i_gj_g} & \leq |E_g| - 1  , &\quad\forall i_g\neq j_g \tag{MTZ$_1$} \label{MTZ1}\\
    0 & \leq s^{i_g} \leq |E_g| - 1 &\quad\forall i_g\tag{MTZ$_2$}\label{MTZ2}
\end{align}

Alternatively, we can also use the family of subtour elimination constraints:
\begin{equation}\tag{SEC}\label{SEC}
    \sum_{i_g, j_g \in S} z_g^{i_gj_g} \leq |S| - 1, \quad \forall g \in \mathcal G,\quad \forall S\subset E_g
\end{equation}

%(Copiado del XPPN)
Since there is an exponential number of SEC constraints, when we implement this formulation we need to perform a row generation procedure including constraints whenever they are required by a separation oracle. To find SEC inequalities, as usual, we search for disconnected components in the current solution. Among them, we choose the shortest subtour found in the solution to be added as a lazy constraint to the model.

 \subsection{All terrain Mothership-Drone Routing Problem with Graphs}
In this problem, we assume that the mothership  is allowed to move freely in a continuous space: $\mathbb R^2$ or $\mathbb R^3$. The goal of the \AMD is to find a feasible solution that minimizes the total distance traveled  by the drone and  the mothership. Hence, assuming that lengths are given by the Euclidean distance, $\|\cdot\|_2$, between their endpoints, to account for the different distances among the decision variables of the model we need to define the following instrumental variables:
\begin{itemize}
    \item $d_L^{i_gt} = \|x_L^t - R^{i_g}\|$. Distance traveled by the drone from the launch point at the stage $t$ to the first visiting point in the segment $i_g$.
    \item $d^{i_gj_g} = \|R^{i_g} - L^{j_g}\|$. Distance traveled by the drone from the launch point in $i_g$ to the rendezvous point in $j_g$.
    \item $d^{i_g} = \|R^{i_g} - L^{i_g}\|$. Distance traveled by the drone from the retrieve point  to the next launch point in $i_g$.
\end{itemize}

\subsubsection{A first formulation for \AMD \ based on stages}
\JP{A natural approach to model this problem is to consider stages which are identified with the targets that the drone has to visit. This way the problem needs to considers $|\mathcal{G}|$ stages that are indexed by $t=1,\ldots, |\mathcal{G}|$. To provide a valid formulation for the model under this approach, we introduce the following variables:
\begin{itemize}
    \item $d_R^{i_gt} = \|L^{i_g} - x_R^t\|$. Distance traveled by the drone from the launch point in the segment $i_g$ to the retrieve point on the mothership at the stage $t$.
    \item $d_{LR}^t = \|x_L^t - x_R^t\|$. Distance traveled by the mothership from the launch point to the retrieve point at the stage $t$.
    \item $d_{RL}^t = \|x_R^t - x_L^{t+1}\|$. Distance traveled by the mothership from the retrieve point at the stage $t$ to the launch point at the stage $t+1$.
\end{itemize}

Therefore, the following formulation minimizes the overall distance traveled by the mothership and drone coordinating their movements and ensuring the required coverage of the targets.}
\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{} \label{AMDRPG-ST} \tag{AMDRPG-ST}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^t\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|x_R^t- x_L^{t+1}\|}{\leq d_{RL}^t,\quad}{\forall i_g,t}{}
 \addConstraint{\|x_L^t- x_R^t\|}{\leq d_{LR}^t,\quad}{\forall i_g,t}{}
 \addConstraint{\left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}), \quad}{\forall g, t}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{The objective function has four terms: the first and fourth ones compute the distances to go to and return from the mothership to the target graph $g$ visited at the stage $t$, the second one accounts for the distance traveled by the drone on the edges of the target graph $g$ between two consecutive \textit{jumps} between edges, and the third one computes the distances traveled by the drone while it \textit{jumps} between two consecutive edges on the target graph $g$. Constraints \eqref{st:DEnt}-\eqref{st:DInv} models the route followed by the drone, \eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G} ensure that the displacement of the drone in each visit to a target graph is a Hamiltonian route, \eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G} defines what is required in each visit to a target graph. Then, the next six constraints models Euclidean distances needed in the model.}
Constraints \eqref{ACW} ensure that the time spent by the drone to visit the graph $g$ at the stage $t$ is less than or equal to the time that the mothership needs to move from the launch point to the retrieve point at the stage $t$. If we want to penalized the waiting time of the drone, we can add a slack variable in the restriction that has to be included in the objective function. %

Observe that we are assuming constant velocities for the mothership $v_M$ and the drone $v_D$.
%(Meto restricción de capacidad? para hacer experimentos puede complicarse)

To deal with the bilinear terms of the objective function, we use McCormick's envelopes to linearize these terms by adding variables $p\geq 0$ that represent these products and introduce these constraints:
\begin{align*}
    p & \geq  m z, \\
    p & \leq d - M(1 - z),
\end{align*}
where $m$ and $M$ are, respectively, the lower and upper bounds of the distance variable $d$. These bounds will be adjusted for each bilinear term in Section \ref{bounds}.

 \subsubsection{Alternative formulations for \AMD  based on enforcing connectivity: MTZ-constraints and subtour elimination-constraints (SEC)\label{sec:AMDMTZ}}
 
\JP{In this family of formulations we replace the variables $u^{\cdot t},\; v^{\cdot t}$ and constraints that model the tour using stages, namely (\ref{st:DEnt})-(\ref{st:DInv}), by constraints that ensure connectivity. We will distinguish two different approaches. The first one is based on the rationale of Miller-Tucker-Zemlin (MTZ) whereas the second one uses an extended formulation based on SEC.} 

We start presenting the formulation based on MTZ. It requires the definition of two families of binary variables that choose:
\begin{itemize}
    \item The optimal order to visit the  graphs $g\in\mathcal G$ in the tour of the mothership.
    \item The optimal order to visit the edges of each graph.
\end{itemize}

The above concepts can be modeled with the following binary variables:
\begin{itemize}
    \item $u^{i_g} = 1$ if the drone accesses the segment $i_g$.
    \item $z^{i_gj_g} = 1$ if the drone goes from the segment $i_g$ to the segment $j_g$.
    \item $v^{i_g} = 1$ if the drone exits the graph  $g$ by the segment $i_g$.
    \item $w^{gg'} = 1$ if the mothership goes from $x_L^g$ to $x_R^{g'}$.
\end{itemize}

By using these binary variables, we can model the route that follows the drone in each particular graph $g\in \mathcal G$:
\begin{align}
    \sum_{i_g} u^{i_g} & = 1, \label{DEnt2}\\%\tag{DEn}\\
    \sum_{i_g} v^{i_g} & = 1, \label{DExt}\\%\tag{DEx}\\
    \sum_{j_g} z^{j_gi_g} + u^{i_g} & = \mu^{i_g}, &\quad\forall i_g \label{DInu}\\
    \sum_{j_g} z^{i_gj_g} + v^{i_g} & = \mu^{i_g}, &\quad\forall i_g \label{DInv2}
\end{align}

On the other hand, to model the tour followed by the mothership, we have to include the following new constraints:
\begin{align}
    \sum_{g\in\mathcal G} w^{g0} & = 0, \label{TOrig}\\
    \sum_{g'\in\mathcal G} w^{(n_G+1) g'} & = 0, \label{TDest}\\
    \sum_{g'\in\mathcal G'\setminus\{g\}} w^{gg'} & = 1, \label{TExt} &\quad\forall g\in \mathcal G\\
    \sum_{g\in\mathcal G'\setminus\{g'\}} w^{gg'} & = 1, &\quad\forall g'\in \mathcal G\label{TEnt}\\
    s_g - s_{g'} + |\mathcal G'|w^{gg'} & \leq |\mathcal G'| - 1  , &\quad\forall g \neq g' \tag{MTZ$_3$} \label{MTZ3}\\
    0 & \leq s_g \leq |\mathcal G'| - 1 &\quad\forall g\in \mathcal G\tag{MTZ$_4$}\label{MTZ4}\\
    s_0 & = 0, \tag{MTZ$_5$}\label{MTZ5}\\
    s_{n_G+1}&=n_G+1, \tag{MTZ$_6$}\label{MTZ6}
\end{align}

\JP{The reader may note that constraints (\ref{TExt}), (\ref{TEnt}) and (\ref{MTZ3})-(\ref{MTZ6}) are of the type MTZ for the complete graph $\hat G=(\hat N,\hat E)$ induced by the graphs $g\in \mathcal G$ to be visited, where a node $\hat e_g \in \hat N$ if $g\in \mathcal G$. Thus, we enforce that the mothership route follows a Hamiltonian tour on the graphs to be visited by the drone.  Next, we have to connect the visits of the drone to the graphs with the tour followed by the mothership. To this end, we require to introduce variables defining the launching and recovery points to account for the distances traveled and to defined the inner tour of the mothership. }


In this problem, we assume that the mothership is allowed to move freely in $\mathbb R^2$. Hence, assuming that lengths are given by the Euclidean distance, $\|\cdot\|_2$, between their endpoints, we need to define the following continuous variables that account for the distances among distinguished points:
\begin{itemize}
    \item $d_L^{i_g} = \|x_L^g - R^{i_g}\|$. Distance traveled by the drone from the launching point to the first visiting point in the segment $i_g$.
    \item $d^{i_gj_g} = \|R^{i_g} - L^{j_g}\|$. Distance traveled by the drone from the launching point in $i_g$ to the next rendezvous point $j_g$.
    \item $d^{i_g} = \|R^{i_g} - L^{i_g}\|$. Distance traveled by the drone from the retrieve point  to the next launch point in $i_g$.
    \item $d_R^{i_g} = \|L^{i_g} - x_R^g\|$. Distance traveled by the drone from the launch point in the segment $i_g$ to the retrieve point on the mothership.
    \item $d_{LR}^g = \|x_L^g - x_R^g\|$. Distance traveled by the mothership from the launch point to the retrieve point while the drone is visiting $g$.
    \item $d_{RL}^{gg'} = \|x_R^g - x_L^{g'}\|$. Distance traveled by the mothership from the retrieve point for the graph $g$ to the launch point associated to the graph $g'$.
\end{itemize}

\begin{figure}[h]
\centering
\includegraphics[height=9cm,width=\textwidth]{AMDRPG2.png}
\caption{Example illustrating the meaning of the launching  (L) and retrieving (R)  points. \label{fig:illustrative}}
\end{figure}

\JP{Figure \ref{fig:illustrative} shows an example of a configuration with two target graphs with four  nodes and four edges.%: one with six nodes and 7 edges and the other one with four nodes and edges%. 
The mothership begins at its starting point $x_L^0$. Then, it moves to $x_L^1$ where the drone is launched to visit the graph 2. There, the drone follows a route that ensures the coverage of $0.66 \%$ of the entire graph and returns to the point $x_R^2$ from where it is launched again to visit the second graph. Once, this graph is visited the drone returns to the mothership at the rendezvous point $x_R^2$ and so on ... }


\JP{In this formulation of \AMD the goal of is again to find a feasible solution that minimizes the total distance traveled  by the drone and  the mothership but without using stages. Instead the model ensures the Hamiltonian nature of the routes using the rationale of connectivity by the MTZ or SEC family of constraints. Therefore, modifying the previous formulation \sf{AMDRPG-ST}, replacing constraints based on stages, one obtains the following alternative valid formulation.}
\begin{mini*}|s|
 {}{\sum_{i_g} (u^{i_g}d_L^{i_g} + v^{i_g}d_R^{i_g}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_g d_{LR}^g + \sum_{g,g'}d_{RL}^{gg'}w^{gg'}}{}{}\label{AMDRPG-MTZ}\tag{AMDRPG-MTZ}
 \addConstraint{\eqref{DEnt2}-\eqref{DInv2}}{}{}
 \addConstraint{\eqref{TOrig}-\eqref{TEnt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
%\addConstraint{\eqref{MTZ3} - \eqref{MTZ6} \text{ or } \eqref{SEC} }{}{}   
 \addConstraint{\eqref{MTZ3} - \eqref{MTZ6}}{}{}   
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^g- R^{i_g}\|}{\leq d_L^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^g\|}{\leq d_R^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|x_R^g- x_L^{g'}\|}{\leq d^{gg'}_{RL},\quad}{\forall g,g'}{}
 \addConstraint{\|x_L^g- x_R^g\|}{\leq d^g_{LR},\quad}{\forall g}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g} d^{i_g} + \sum_{i_g}v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_{RL}^{g}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}


\JP{The formulation above \eqref{AMDRPG-MTZ} can be slightly modified replacing constraints $\eqref{MTZ3} - \eqref{MTZ6}$ by 
\begin{equation}\label{SEC-graph}
\sum_{g,g'\in \mathcal G} w^{gg'} \le |S|-1, \quad \forall S\subseteq \{1,\ldots, |\mathcal G|\}.
\end{equation}
This way we obtain another formulation for \AMD using SEC rather than MTZ constraints to represent the mothership tour. We will call this formulation (AMDRPG-SEC). Later, we will compare their performance in the computational results section.


\subsubsection{Comparing the formulations\label{ss:compare}}
A straightforward analysis of the two types of formulations, namely by stages and based on connectivity, shows that \ref{AMDRPG-MTZ} has much less variables and constraints than \ref{AMDRPG-ST}. Indeed, the latter requires definition of distance variables for each $i_g$ and $t$ which is a quadratic number rather than a linear one as used by the former. In addition, to enforce coordination \ref{AMDRPG-ST} needs constraints (DCW) for each $g\in \mathcal{G},\ t=1,\ldots,T$ whereas \ref{AMDRPG-MTZ} only uses (DCW) constraints for $g\in \mathcal{G}$. This is an important decrease in the dimension of the problems to be solved. This observation is confirmed in efficiency in problem solving in the section of computational experiments.} 


\subsection{Network Mothership-Drone Routing Problem on a Polygonal with Graphs (\PMD)}
The most significant difference between \AMD and  \PMD \ is that, in the latter, the mothership cannot move freely in $\mathbb R^2$ but it has to move on a network that models a road system where the mothership (truck) is restricted to move. \JP{An intermediate situation between moving freely and moving on a general road network is to assume that the mothership moves on a closed polygonal, namely a piecewise linear, chain. Modeling this situation is a transition step to achieve the more general case of the mothership moving on general networks. We will present the results for the \PMD \  following a scheme similar to that of \AMD. First, we present a model by stages and then another one based on connectivity constraints.}

Let $\mathcal P$ denote a polygonal chain parametrized by its breakpoints $A_1, \ldots, A_p$ ordered in the direction of travel. Observe that we are assuming that there exists a pre-specified orientation that determines the direction of the mothership's displacement. Let also $\gamma_L^{et}$ and $\gamma_R^{et}$ be the parameter values that define the points $x_L^t$ and $x_R^t$ on the edge $e$ on $\mathcal P$, respectively. \JP{Figure \ref{fig:ex1} illustrates the meaning of the parameters $\gamma_L^{et}$ and $\gamma_R^{et}$ on a polygonal chain with 4 pieces.} Then, the distance measured on the polygonal can be obtained by the following expressions:
\begin{equation}\tag{$d^{t\mathcal P}_{LR}$}\label{eq:dLRPt}
d_{LR}^{ee't} = \left\{\begin{matrix}
(\gamma_R^{et} - \gamma_L^{et})\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_L^{et})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{R}^{e't}\mathcal L(e')), & \text{if } e < e'.
\end{matrix}\right.
\end{equation}

\begin{equation}\tag{$d^{t\mathcal P}_{RL}$}\label{eq:dRLPt}
d_{RL}^{ee't} = \left\{\begin{matrix}
(\gamma_{L}^{et+1}-\gamma_R^{et})\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_R^{et})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{L}^{e't+1}\mathcal L(e')), & \text{if } e < e'.
\end{matrix}\right.
\end{equation}

This distance requires a binary variable $z_{LR}^{ee't}$ that determines whether $d_{LR}^{ee'}$ is defined by the first or the second expression in the formula:
$$z_{LR}^{ee't} = 1 \text{ if } \mu_{L}^{et} = 1 \text{ and }\mu_{R}^{e't} = 1,$$

\noindent where $\mu_{L}^{et}$ and $\mu_{R}^{et}$ are indicator variables that attain the value one if the launch point (resp. retrieve point) is placed in the segment $e$ of $\mathcal P$ at the stage $t$.

Similarly, we define $z_{RL}^{ee't}$:
$$z_{RL}^{ee't} = 1 \text{ if } \mu_{R}^{et} = 1 \text{ and }\mu_{L}^{e't+1} = 1.$$

In addition, we need to define continuous variables $\lambda_R^t$ and $\lambda_L^t$ that model the absolute position of the point $x_L^t$ in the polygonal to ensure that the movement of the mothership goes always in the allowed direction of travel and never comes back when it traverses the polygonal chain. 

\begin{figure}[h!]
\begin{center}
 \includegraphics[width=1\linewidth]{TDRPG.png}
\end{center}
\caption{An example of a parameterization of a mothership route that goes from $A_1$ to $x_L^t$ to launch the drone, then moves to $x_R^t$ on the edge $\overline{A_1A_2}$ to retrieve it, then it goes to $x_L^t$ on $\overline{A_2A_3}$ to launch it again, and travels until $x_R^t$ on $\overline{A_3A_4}$ to retrieve the drone and returns to the starting point at $A_1$.\label{fig:ex1}}
\end{figure}

With all this, we can model the movement of the mothership on the polygonal. For each stage $t$, we have

\begin{align}
    x_L^t & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{L}^{et}\left[A^i + \gamma_L^{et}(A^{i+1} - A^i)\right]\label{param1}\\
    x_R^t & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{R}^{et}\left[ A^i + \gamma_R^{et}(A^{i+1} - A^i)\right]\label{param2}\\
    z_{LR}^{ee't} & = \mu_{L}^{et}\mu_{R}^{e't}\label{pol:prodLR}\\
    z_{RL}^{ee't} & = \mu_{R}^{et}\mu_{L}^{e't+1}\label{pol:prodRL}\\
    \sum_{e} \mu_{L}^{et} & = 1  \label{muL} \\
    \sum_{e} \mu_{R}^{et} & = 1 \label{muR}\\
    d_{LR}^t & = \sum_{e, e'} z_{LR}^{ee't} d_{LR}^{ee'} \label{pol:dLRt},\\
    d_{RL}^t & = \sum_{e, e'} z_{RL}^{ee't} d_{RL}^{ee't} \label{pol:dRLt},\\
    \lambda_L^t - i & \geq \mu_{L}^{et} - (p-1)(1-\mu_{L}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaLg}\\
    \lambda_L^t - i & \leq \mu_{L}^{et} - (p-1)(1-\mu_{L}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaLl}\\
    \lambda_R^t - i & \geq \mu_{R}^{et} - (p-1)(1-\mu_{R}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaRg}\\
    \lambda_R^t - i & \leq \mu_{R}^{et} + (p-1)(1-\mu_{R}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaRl}\\
    \lambda_R^t & \geq \lambda_L^t \label{lambdaRL}\\
    \lambda_L^{t+1} & \geq \lambda_R^t \label{lambdaLR}
\end{align}

\noindent where $d_{LR}^{ee'}$ and $d_{RL}^{ee't}$ are defined in \eqref{eq:dLRPt} and \eqref{eq:dRLPt}. Constraints \eqref{param1} and \eqref{param2} parameterize the launch and retrieve points on the polygonal chain. Constraints \eqref{pol:prodLR} and \eqref{pol:prodRL} model the product of binary variables. Constraints \eqref{muL} and \eqref{muR} state that, in each stage, the launch and retrieve points can be only in one segment, not necessarily the same. Constraints \eqref{pol:dLRt} and \eqref{pol:dRLt} compute the total distance between the launch and the retrieve point in each stage. Inequalities \eqref{lambdaLg}-\eqref{lambdaRl} link $\mu_{L}^{et}$ and $\lambda_L^t$ (resp. $\mu_{R}^{et}$ and $\lambda_R^t$). Finally, constraints \eqref{lambdaRL} and \eqref{lambdaLR} ensure that the mothership moves in the right direction on the polygonal. Note that, in this case, it is not required to account for the distance $d_{RL}^t$ because by the assumptions on the model the mothership will traverse all the polygonal chain (since we have imposed that the route starts and ends at the same point).


The goal of the (\PMD) is, once again, to find a feasible solution that minimizes the total distance covered by the mothership and the drone. Thus, gathering all the above constraints one gets the following valid formulation.
\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{}\tag{PMDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{param1}-\eqref{lambdaLR}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\eqref{eq:dLRPt}, \eqref{eq:dRLPt}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^t\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\hspace*{-1.5cm} \left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}), \,}{\forall g, t}{}\label{ACW}\tag{{\scriptsize DCW}}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}
\subsubsection{Alternative formulation for \PMD \  based on MTZ-constraints}

\JP{Analogously to the case of \AMD one can also model \PMD \ without any explicit reference to stages. Here, we will follow a very similar approach to that in Section \ref{sec:AMDMTZ} to describe the formulation for \PMD \ based on MTZ-constraints.}

Let $\mathcal P$ denote, as before,  the polygonal chain parametrized by its endpoints $A_1, \ldots, A_p$ ordered in the direction of travel. In addition, let also $\gamma_{L}^{eg}$ and $\gamma_{R}^{eg}$ be the parameter values that define the points $x_L^g$ and $x_R^g$ on the line segment $\overline{A_iA_{i+1}}$ in $\mathcal P$, respectively. \JP{Then, the distance traveled on the polygonal can be obtained by one of  the following expressions. The first one refers to distances covered by the mothership between the launching and retrieving points of a drone operation, whereas models the distance traveled by the mothership between the launching and retrieving points of two consecutive graphs targeted in its route.}
\begin{equation}\tag{$d_{LR}^{g\mathcal P}$}\label{eq:dLRPg}
d_{LR}^{ee'g} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg}|\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_{L}^{eg})\mathcal L(e) + \sum_{e'' =e+1}^{e'-1}\mathcal L(e'') + \gamma_{R}^{e'g}\mathcal L(e'), & \text{if } e < e', \\
\gamma_{L}^{eg}\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + (1-\gamma_{R}^{e'g})\mathcal L(e'), & \text{if } e > e'.
\end{matrix}\right.
\end{equation}

\begin{equation}\tag{$d_{RL}^{g\mathcal P}$}\label{eq:dRLPg}
d_{RL}^{ee'gg'} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg'}|\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_{R}^{eg})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{L}^{e'g'}\mathcal L(e'), & \text{if } e < e',\\
\gamma_{R}^{eg}\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + (1-\gamma_{L}^{e'g'})\mathcal L(e'), & \text{if } e > e'.
\end{matrix}\right.
\end{equation}

\JP{This distance requires binary variables $z_{LR}^{ee'g}$ and $z_{RL}^{ee'gg'}$ that determines which of the expressions in \eqref{eq:dLRPg} and  \eqref{eq:dRLPg} define $d_{LR}^{ee'g}$ and $d_{RL}^{ee'gg'}$,respectively.}
$$z_{LR}^{ee'g} = 1 \text{ iff } \mu_{L}^{eg} = 1 \text{ and }\mu_{R}^{e'g} = 1,\qquad
z_{RL}^{ee'gg'} = 1 \text{ iff } \mu_{L}^{eg} = 1 \text{ and }\mu_{R}^{e'g'} = 1,
$$
where $\mu_{L}^{eg}$ and $\mu_{R}^{eg}$ are indicator variables that attain the value one if the launch point (resp. retrieve point) associated to the graph $g$ is placed in the segment $\overline{A_iA_{i+1}}$ of the edge $e=(i, i+1) \in \mathcal P$ .

With all this, we can model the movement of the mothership inside the polygonal. 

\begin{align}
    x_L^g & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{L}^{eg}\left[A^i + \gamma_L^{eg}(A^{i+1} - A^i)\right]\label{param1g}\\
    x_R^g & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{R}^{eg}\left[ A^i + \gamma_R^{eg}(A^{i+1} - A^i)\right]\label{param2g}\\
    z_{LR}^{ee'g} & = \mu_{L}^{eg}\mu_{R}^{e'g}\label{prodLRg}\\
    z_{RL}^{ee'gg'} & = \mu_{R}^{eg}\mu_{L}^{e'g'}\label{prodRLg}\\
    \sum_{e} \mu_{L}^{eg} & = 1  \label{muLg} \\
    \sum_{e} \mu_{R}^{eg} & = 1 \label{muRg}\\
    d_{LR}^{g} & = \sum_{e, e'} z_{LR}^{ee'g} d_{LR}^{ee'g} \label{dLRg},\\
    d_{RL}^{gg'} & = \sum_{e, e'} z_{RL}^{ee'gg'} d_{RL}^{ee'gg'} \label{dRLgg},
\end{align}

\noindent where $d_{LR}^g$ and $d_{RL}^{gg'}$ are defined in \eqref{eq:dLRPg} and \eqref{eq:dRLPg}, respectively. Constraints \eqref{param1g} and \eqref{param2g} parameterize the launch and retrieve points on the polygonal chain. Constraints \eqref{prodLRg} and \eqref{prodRLg} model the product of binary variables. Constraints \eqref{muLg} and \eqref{muRg} state that, in each stage, the launch and retrieve points can be only in one segment, not necessarily the same. Constraints \eqref{dLRg} and \eqref{dRLgg} compute the total distance between the launch and the retrieve point for each pair of points. \JP{The reader may note that the above representation is similar to that given by \eqref{param1}-\eqref{pol:dRLt} with the exception that in \eqref{param1g}-\eqref{dRLgg} constraints are indexed in the set of graphs $g\in \mathcal{G}$ instead that on the stages. This fact allows a remarkable reduction on the number of distance variables and constraints as already discussed in Section \ref{ss:compare}.}

The goal of the (\PMD) is to find a feasible solution that minimizes the total distance covered by the drone and the mothership, i.e.,
\begin{mini*}|s|
 {}{\sum_{i_g} (u^{i_g}d_L^{i_g} + v^{i_g}d_R^{i_g}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_g d_{LR}^g + \sum_{g,g'}d_{RL}^{gg'}w^{gg'}}{}{}\label{PMDRPG-MTZ}\tag{PMDRPG-MTZ}
 \addConstraint{\eqref{DEnt2}-\eqref{DInv2}}{}{}
 \addConstraint{\eqref{TOrig}-\eqref{TEnt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{MTZ3} - \eqref{MTZ6} \text{ or } \eqref{SEC} }{}{}   
 \addConstraint{\eqref{param1g}-\eqref{dRLgg}}{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
  \addConstraint{\eqref{eq:dLRPg}, \eqref{eq:dRLPg}}{}{}
 \addConstraint{\|x_L^g- R^{i_g}\|}{\leq d_L^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g} d^{i_g} + \sum_{i_g}v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_{RL}^{g}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{The reader may note that the above formulation actually encloses two different ones depending whether it includes constraints \eqref{MTZ1} - \eqref{MTZ2}  or  \eqref{SEC}. However, for the sake of presentation we have preferred to present them in this compact form to reduce the length of the paper.}

\subsection{Network Mothership-Drone Routing Problem with Graphs (\NMD)}
\JP{This new model is a refinement of the last one in that now the mothership has to move on a general undirected network rather than on a polygonal chain. 
Even though the previous one, namely \PMD, can be seen as a particular case of \NMD, for the sake of presentation, we have preferred to include it first to ease the understanding of the more advanced \NMD \ model.

As before, we start with an approach that models the problems by stages. Later, we shall extend the analysis using the rationale of connectivity, as already done in the the previous models \AMD \ and \PMD.}

Let $\mathcal N=(V, E)$ be the network that model the space of movement for the mothership. For each stage $t\in \{1,\ldots,|\mathcal G|\}$, assume that the mothership starts and ends in the edge $e=(i,j)$ and $e'=(i',j')$, respectively. Then, it follows a route from the launching to the retrieving point and vice versa, determined by a sequence of intermediate vertices, similar to the following one:

$$
e=(i, j) \ni x_L^t \rightarrow V_i \vee V_j \rightarrow \ldots \rightarrow V_k \rightarrow \ldots \rightarrow V_{i'} \rightarrow x_R^t \in (i',j')=e'.
$$
\JP{**** \@ Carlos: La notacion de $V_i$ y $i$ es un lio. Esto hay que aclararlo. *****}
Therefore, the distance traveled by the mothership, between two consecutive launching and retrieving points in two edges, not necessarily distinct,  of the graph can be represented as:
\begin{equation}\tag{$d^{t\mathcal N}_{LR}$}\label{eq:dLRNt}
d_{LR}^{ee't} = \left\{\begin{matrix}
|\gamma_{L}^{et} - \gamma_{R}^{et}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{LR}^{it}\gamma_{L}^{et} + b_{LR}^{jt}(1 - \gamma_{L}^{et})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{LR}^{e''t}\mathcal L(e'') + \left[c_{LR}^{i't}\gamma_{R}^{e't} + c_{LR}^{j't}(1 - \gamma_{R}^{e't})\right]\mathcal{L}(e'), & \text{if } e \neq e',
\end{matrix}\right.
\end{equation}

\noindent 
where $b_{LR}^{it}$ (resp. $c_{LR}^{it}$) are binary variables that determine from which of the end-points of $e$ (respectively $e'$) one has to account for the distance and $q_{LR}^{et}$ is a binary variable that is one when the mothership fully traverses the edge $e$. \JP{Furthermore, we need to define another binary variable $z_{LR}^{ee't}$ that models the correct definition of the distance in \eqref{eq:dLRNt}. With the above definition one can account for  the movement of the mothership at each stage $t\in \{1, \ldots, |\mathcal G|\}$ from a launching to a retrieving  point:}

\begin{align}
    x_L^t & = \sum_{e=(i, j)\in E} \mu_{L}^{et}\left[V^i + \gamma_{L}^{et}(V^j - V^i)\right]\label{st:param1bis}\\
    x_R^t & = \sum_{e=(i, j)\in E} \mu_{R}^{et}\left[ V^i + \gamma_{R}^{et}(V^j - V^i)\right]\label{st:param2bis}\\
    z_{LR}^{ee't} & = \mu_{Le}^t\mu_{Re'}^t,\label{st:prodLRbis}\\
    b_{LR}^{it} & \leq \sum_{e\in\delta(i)}\mu_{L}^{et}, \label{st:bLt1}&\qquad\forall i\in V \\
    c_{LR}^{it} & \leq \sum_{e\in\delta(i)}\mu_{R}^{et}, \label{st:cLt1}&\qquad\forall i\in V\\
    b_{LR}^{it} + b_{LR}^{jt} & \geq \sum_{e'\neq e} z_{LR}^{ee't}, &\qquad \forall e=(i, j)\in E\label{st:bLt2}\\
    c_{LR}^{it} + c_{LR}^{jt} & \geq \sum_{e'\neq e} z_{LR}^{e'et}, &\qquad \forall e=(i, j)\in E\label{st:cLt2}\\
    b_{LR}^{it} + \sum_{\{j:(i, j)\in E\}} q_{LR}^{jit} & = \sum_{\{j:(i, j)\in E\}} q_{LR}^{ijt} +  c_{LR}^{it}, \label{st:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{et} & = 1,  \label{st:muLe} \\
    \sum_{e\in E} \mu_{R}^{et} & = 1, \label{st:muRe}\\
    d_{LR}^t & = \sum_{e, e'} z_{LR}^{ee't} d_{LR}^{ee't}, \label{st:dLRt}
\end{align}

Constraints \eqref{st:param1bis} and \eqref{st:param2bis} parameterize the launching and retrieving points in the network $\mathcal N$ at stage $t$. Constraints \eqref{st:prodLRbis} model the product of binary variables. Constraints \eqref{st:bLt1} and \eqref{st:cLt1} say that if the launching point (resp. retrieving point) is not in the edge $e$, the mothership cannot go (resp. exit) to the vertex that is incident to $e$. Constraints \eqref{st:bLt2} state that if the mothership leaves the edge $e$ to go to $e'$, it must exit from one of the incident vertices to $e$. In the same way, restrictions \eqref{st:cLt2} express that if the mothership leaves the edge $e'$ to go to $e$, it must enter to the edge $e$ from one of its incident vertices. Flow conservation constraints \eqref{st:flow} ensure that the number of incoming edges to each vertex $i$ is equal to the number of outgoing edges in the route followed by the mothership. Constraints \eqref{st:muLe} and \eqref{st:muRe} say that, in each stage, the selected points can be only in one edge. Finally, constraints \eqref{st:dLRt} defines the total distance between the launching and the retrieving points at  stage $t$.

\medskip

Similarly, the distance covered by the mothership along the path on the network from the retrieving point $x_R^t$ to the next launching point $x_L^{t+1}$ can be modeled using the following definition of distance:

\begin{equation}\tag{$d^{t\mathcal N}_{RL}$}\label{eq:dRLNt}
d_{RL}^{ee't} = \left\{\begin{matrix}
|\gamma_{R}^{et} - \gamma_{L}^{et+1}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{RL}^{it}\gamma_{R}^{et} + b_{RL}^{jt}(1 - \gamma_{R}^{et})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{RL}^{e''t}\mathcal L(e'') + \left[c_{RL}^{i't}\gamma_{L}^{e't+1} + c_{RL}^{j't}(1 - \gamma_{L}^{e't+1})\right]\mathcal{L}(e'), & \text{if } e \neq e'.
\end{matrix}\right.
\end{equation}

In this case, the binary variable $z_{ee'}^{RLt}$ links the retrieve point at $t$ with the launch point at $t+1$. Then, we can use a set of constraints similar to those used above and the distance from $x_R^t$ to $x_L^{t+1}$ is:

\begin{align}
    z_{RL}^{ee't} & = \mu_{R}^{et}\mu_{L}^{e't+1},\label{st1:prodRL}\\
    b_{RL}^{it} & \leq \sum_{e\in\delta(i)}\mu_{R}^{et}, \label{st1:bRt1}&\qquad \forall i\in V \\
    c_{RL}^{it} & \leq \sum_{e\in\delta(i)}\mu_{L}^{et}, \label{st1:cRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V\\
    b_{RL}^{it} + b_{RL}^{jt} & \geq \sum_{e'\neq e} z_{RL}^{ee't}, &\qquad \forall e=(i, j)\in E\label{st1:bRt2}\\
    c_{RL}^{it} + c_{RL}^{jt} & \geq \sum_{e'\neq e} z_{RL}^{e'et}, &\qquad \forall e=(i, j)\in E\label{st1:cRt2}\\
    b_{RL}^{it} + \sum_{\{j:(i, j)\in E\}} q_{RL}^{jit} & = \sum_{\{j:(i, j)\in E\}} q_{RL}^{ijt} +  c_{RL}^{it}, \label{st1:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{et} & = 1,  \label{st1:muLe} \\
    \sum_{e\in E} \mu_{R}^{et} & = 1, \label{st1:muRe}\\
    d_{RL}^t & = \sum_{e, e'} z_{RL}^{ee't} d_{RL}^{ee't}. \label{st1:dRLtN}
\end{align}

\JP{Constraints \eqref{st1:prodRL} model the product of binary variables. Constraints \eqref{st1:bRt1} and \eqref{st1:cRt1} say that if the retrieving point (resp. launching point) is not in the edge $e$, the mothership cannot go (resp. exit) to the end vertices of the edge $e$. Constraints \eqref{st1:bRt2} state that if the mothership leaves the edge $e$ to go to $e'$, it must exit via one of the end vertices of $e$. In the same way, restrictions \eqref{st1:cRt2} state that if the mothership leaves the edge $e'$ to go to $e$, it necessarily must enter to $e$ from one incident vertex of $e$. Flow conservation constraints \eqref{st1:flow} ensure that in the route followed by the mothership the number of used incoming edges to each vertex $i$ is equal to the number of used outgoing edges. Constraints \eqref{st1:muLe} and \eqref{st1:muRe} say that, in each stage, the selected points can be only in one edge. Constraints \eqref{st1:dRLtN} state the total distance between the retrieving and the launching points at stage $t$.}


Hence, once the distances inside the graph are set with the above two families of constraints, we can state the mathematical programming formulation of the problem as:

\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{}\tag{TDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{st:param1bis}-\eqref{st1:dRLtN}}{}{}
 \addConstraint{\eqref{eq:dLRNt}, \eqref{eq:dRLNt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d_g^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\hspace*{-2cm}\left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i, j}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_gt}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}),\ }{\forall g, t}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{A brief decription of this formulation must be included ...}

\subsubsection{MTZ formulation for the Network Mothership-Drone Routing Problem with Graphs}

\JP{Something missing to connect it to the previous section ... JUSTO: Por aqui 20/11/2020}

Therefore, the distance between launching and retrieving points in two edges, not necessarily distinct,  of the graph can be represented as:
\begin{equation}\tag{$d^{g\mathcal N}_{LR}$}\label{eq:dLRg}
d_{LR}^{ee'g} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{LR}^{ig}\gamma_{L}^{eg} + b_{LR}^{jg}(1 - \gamma_{L}^{eg})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{LR}^{e''g}\mathcal L(e'') + \left[c_{LR}^{i'g}\gamma_{R}^{e'g} + c_{LR}^{j'g}(1 - \gamma_{R}^{e'g})\right]\mathcal{L}(e'), & \text{if } e \neq e',
\end{matrix}\right.
\end{equation}

\noindent 
where $b_{LR}^{ig}$ (resp. $c_{LR}^{ig}$) are binary variables that determine from which of the end-points of $e$ (respectively $e'$) one has to account for the distance and $q_{LR}^{eg}$ is a binary variable that is one when the mothership fully traverses the edge $e$. Furthermore, we need to define binary variables $z_{LR}^{ee'g}$ that model the choice of the model for right definition (first or second formulas in \eqref{eq:dLRg}) of the distance in \eqref{eq:dLRg}. All the above give the necessary elements to account for the movement of the mothership in each graph $g\in \{1, \ldots, |\mathcal G|\}$:

\begin{align}
    x_L^g & = \sum_{e=(i, j)\in E} \mu_{L}^{eg}\left[V^i + \gamma_{L}^{eg}(V^j - V^i)\right]\label{g:param1bisg}\\
    x_R^g & = \sum_{e=(i, j)\in E} \mu_{R}^{eg}\left[ V^i + \gamma_{R}^{eg}(V^j - V^i)\right]\label{g:param2bisg}\\
    z_{LR}^{ee'g} & = \mu_{L}^{eg}\mu_{R}^{e'g},\label{g:prodLR}\\
    b_{LR}^{ig} & \leq \sum_{e\in\delta(i)} \mu_{L}^{eg}, \label{g:bLt1}&\qquad \forall i\in V \\
    c_{LR}^{ig} & \leq \sum_{e\in\delta(i)} \mu_{R}^{eg}, \label{g:cLt1}&\qquad \forall i\in V\\
    b_{LR}^{ig} + b_{LR}^{jg} & \geq \sum_{e'\neq e} z_{LR}^{ee'g}, &\qquad \forall e=(i, j)\in E\label{g:bLt2}\\
    c_{LR}^{ig} + c_{LR}^{jg} & \geq \sum_{e'\neq e} z_{LR}^{e'eg}, &\qquad \forall e=(i, j)\in E\label{g:cLt2}\\
    b_{LR}^{ig} + \sum_{\{j:(i, j)\in E\}} q_{LR}^{jig} & = \sum_{\{j:(i, j)\in E\}} q_{LR}^{ijg} +  c_{LR}^{ig}, \label{g:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{eg} & = 1,  \label{g:muLe} \\
    \sum_{e\in E} \mu_{R}^{eg} & = 1, \label{g:muRe}\\
    d_{LR}^g & = \sum_{e, e'} z_{LR}^{ee'g} d_{LR}^{ee'g}, \label{g:dLRgN}
\end{align}

\JP{Constraints \eqref{g:param1bisg} and \eqref{g:param2bisg} parameterize the launch and retrieve points in the network $\mathcal N$ induced by the visit to the graph  $g\in \mathcal{G}$. Constraints \eqref{g:prodLR} model the product of binary variables. Constraints \eqref{g:bLt1} and \eqref{g:cLt1} say that if the launch point (resp. retrieve point) is not in the edge $e$, the drone cannot go (resp. exit) to the vertices of the edge $e$. Constraints \eqref{g:bLt2} state that if the drone leaves the edge $e$ to go to $e'$, it must exit from one of the incident vertices to $e$. In the same way, restrictions \eqref{g:cLt2} express that if the drone leaves the edge $e'$ to go to $e$, it necessarily must enter to $e$ from one incident vertex of $e$. Flow conservation constraints \eqref{g:flow} ensure that the number of incoming edges to each vertex $i$ is equal to the number of outgoing edges. Constraints \eqref{g:muLe} and \eqref{g:muRe} say that, in visit to the graph  $g\in \mathcal{G}$, launching and retrieving points can be only in one edge. Constraints \eqref{g:dLRgN} returns the total distance traveled by the drone on the graph  $g\in \mathcal{G}$.}

\medskip

Similarly, the distance covered by the mothership along the path on the network from the retrieving point $x_R^g$ to the next launching point $x_L^{g'}$ can be modeled using the following definition of distance:

\begin{equation}\tag{$d^{g\mathcal N}_{RL}$}\label{eq:dRLg}
d_{RL}^{ee'gg'} = \left\{\begin{matrix}
|\gamma_{R}^{eg} - \gamma_{L}^{eg'}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{RL}^{ig}\gamma_{R}^{eg} + b_{RL}^{jg}(1 - \gamma_{R}^{eg})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{RL}^{e''gg'}\mathcal L(e'') + \left[c_{RL}^{i'g'}\gamma_{L}^{e'g'} + c_{RL}^{j'g'}(1 - \gamma_{L}^{e'g'})\right]\mathcal L(e'), & \text{if } e \neq e'.
\end{matrix}\right.
\end{equation}

In this case, the binary variable $z_{RL}^{ee'gg'}$ links the retrieve point at $g$ with the launch point at $g'$. Then, we can use a set of constraints similar to those used above and the distance from $x_R^g$ to $x_L^{g'}$ is:

\begin{align}
    z_{RL}^{ee'gg'} & = \mu_{R}^{eg}\mu_L^{e'g'},\label{prodRLggN}\\
    b_{RL}^{ig} & \leq \mu_{R}^{eg}, \label{bRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V \\
    c_{RL}^{ig} & \leq \mu_{L}^{eg}, \label{cRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V\\
    b_{RL}^{ig} + b_{RL}^{jg} & \geq \sum_{e'\neq e} z_{RL}^{ee'gg'}, &\qquad \forall e=(i, j)\in E\label{bRt2}\\
    c_{RL}^{ig'} + c_{RL}^{jg'} & \geq \sum_{e'\neq e} z_{RL}^{e'eg'g}, &\qquad \forall e=(i, j)\in E\label{cRt2}\\
    b_{RL}^{ig} + \sum_{\{j:(i, j)\in E} q_{RL}^{jigg'} & = \sum_{\{j:(i, j)\in E\}} q_{RL}^{ijgg'} +  c_{RL}^{ig}, \label{flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{eg} & = 1,  \label{muLe} \\
    \sum_{e\in E} \mu_{R}^{eg} & = 1, \label{muRe}\\
    d^{RLgg'} & = \sum_{e, e'} z_{RL}^{ee'gg'} d_{RL}^{ee'gg'}. \label{dRLt}
\end{align}

Hence, once the distances inside the graph are set with the above two families of constraints, we can state the mathematical programming formulation of the problem as:

\begin{mini*}|s|
 {}{\sum_{i, g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i,j,g}z^{i_gj_g}d^{i_gj_g}}{}{}\tag{TDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{g:param1bisg}-\eqref{dRLt}}{}{}
 \addConstraint{\eqref{eq:dLRg}, \eqref{eq:dRLg}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d_g^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i, j}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_g^{RL}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}
% $$
% e=(i, j) \ni x_R^t \rightarrow V_i \vee V_j \rightarrow \ldots \rightarrow V_k \rightarrow \ldots \rightarrow V_{i'} \rightarrow x_L^{t+1} \in (i',j')=e'
% $$

% The design of these paths obeys to define binary variables that decide which vertices are selected in each stage $t$:

==> Mothership Drone/heuristic.tex <==
\section{A Matheuristic for the Mothership-Drone Routing Problem with Graphs}\label{Math}
\noindent
This section is devoted to present our matheuristic approach to address the solution of the \AMD. Our motivation comes from the fact that the exact solution of the models presented in Section \ref{Form} is highly time demanding. Alternatively, the matheuristic provides good quality solution in limited computing times.\\
\noindent
%\JP{First, we focus on the synchronized case in which each drone that is used must be launched and retrieved in the same stage.}
The basic idea of the algorithm is to determine the route that a drone should perform for visiting each graph $g \in \mathcal{G}$, and thus the entry and exit points $L^{e_{g}}$ and $R^{e^{'}_{g}}$ for each graph.
Sequentially, a clustering procedure on the target graphs is applied in order to compute the route of the mothership via their reference points and the origin/destination points.
The clustering procedure is based on a random selection of the initial target graphs and for this reason it is repeated a number of times in order to consider different cluster structures. At each iteration the new clusters are evaluated by computing the cost of the route visiting their reference points and the origin/destination points. 
The route computed on the reference points of the best cluster generated by this iterative procedure, is used to set the values of the binary variables $u^{e_gtd}$ and $v^{e_gtd}$, that determine the order of visits to the graphs. Finally, these variables are provided as an initial partial solution to the \AMD\xspace model to produce a complete feasible solution.\\
In the following, we present the pseudo-code of this algorithm:



\begin{itemize} 
\item[STEP 1] (First entry and last exit points for each target graph)\\
Compute the route on each target graph $g \in \mathcal{G}$.
Let $L^{e_{g}}$ and $R^{e^{'}_{g}}$ be the pair of entry and exit points on $g$ closest to the origin and let  $\mathcal L(e_{g}, e^{'}_{g})$ be the associated length computed as the sum of the distances travelled by the drone to visit the graph $g$, excluding the distance between $L^{e_{g}}$ and $R^{e^{'}_{g}}$.
\item[STEP 2] (Clustering procedure)\\
Initialization: set $it=1$, define one cluster for each target graph and set $nit=1$. \\
Select randomly two clusters $K_i$ and $K_j$ (where $i<j$).\\
Check if the number of graphs belonging to the union of $K_i$ and $K_j$ is less than the number of available drones $n_D$.\\
If this condition is satisfied:\\
search for point $P$ satisfying the following capacity constraint:
$$
\frac{d(P, R^{e_g}) + \mathcal L(e_{g}, e^{'}_{g}) + d(L^{e^{'}_{g}}, P)}{v_D} \leq N^d, \quad \forall R^{e_g}, L^{e^{'}_{g}} \in K_i, \:\: K_j.
$$
If such a point exists, merge the two clusters and label the new one as $K_i$.\\
Set $nit=nit+1$.\\
Repeat the same procedure on the new cluster structure while $nit < maxit$.
\item[STEP 3] (Computation of Reference Points) 
%\JP{This step is not well-defined: The term centroid defines exactly the points we should use another term that allows to minimize something!!!} \\
% Compute the centroids of the clusters generated at STEP 2, by minimizing the distance between them and the origin always imposing that the capacity constraint is satisfied.
Compute a reference point for each cluster generated at STEP 2. This computation seeks for the minimization of the distance between each pair of reference points and the distance between them and the origin, always imposing that the \eqref{CAP} constraint is satisfied.



\item [STEP 4] (Setting the order of visits to the  graphs: route via the reference points and the origin/destination points) \\
Compute the TSP of the mothership among the reference points of the clusters and let $\mathcal L(TSP)$ be the associated length.\\
Set $it=it+1$.\\
if(it< maxseed) go to STEP 2\\
else go to STEP 5
\item [STEP 5] (Solution of the \AMD\space model fixing an initial partial solution)\\
Set the values of the binary variables $u^{e_{g}td}$ and $v^{e_{g}td}$ and solve the model \AMD\, to obtain a feasible solution.
\end{itemize}
\noindent
%}



\begin{figure}[h]
\centering
\includegraphics[width = 0.5\linewidth]{figures/example.png}
\caption{Illustrative example \label{fig:example1}}
\end{figure}

\noindent
Figure \ref{fig:example1} shows an illustrative example consisting of four target planar graphs ($g_1$, $g_2$, $g_3$ and $g_4$) to be visited. We assume that their visits must be performed by a fleet of two drones supported by a mothership which starts from the origin $(0,0)$ and ends on the destination point $(100,0)$.



\begin{figure}[h!]
    \centering
    \subfloat[\centering a]{{\includegraphics[width=5cm]{figures/example_tour_g1_Step1.png} }}%
    \qquad
    \subfloat[\centering b]{{\includegraphics[width=5cm]{figures/example_tour_g2_Step1.png} }}%
     \qquad
    \subfloat[\centering c]{{\includegraphics[width=5cm]{figures/example_tour_g3_Step1.png} }}%
    \qquad
    \subfloat[\centering d]{{\includegraphics[width=5cm]{figures/example_tour_g4_Step1.png} }}%
    \caption{STEP 1 for the illustrative example}%
    \label{fig:example2}%
\end{figure}

\noindent
Figure \ref{fig:example2} reports a zoom on each single target graph, showing the tour generated by STEP 1 of the heuristic procedure. A pair of points representing retrieving and launching points,  together with an arrow pointing the direction followed by the drone according with the order in which the edges are visited, are depicted on each edge.

\begin{figure}[h!]
    \centering
    \subfloat[\centering a]{{\includegraphics[width=5cm]{figures/example_step_2.png} }}%
    \qquad
    \subfloat[\centering b]{{\includegraphics[width=5cm]{figures/example_step_3.png} }}%
        \caption{[a] STEP 2, [b] STEP 3 for the illustrative example}%
    \label{fig:example3}%
\end{figure}

\noindent
By applying STEP 2 to this illustrative example, we obtain three clusters, as shown in Figure \ref{fig:example3}[a]. One cluster contains graphs $g_1$ and $g_3$ (in red), while graph $g_2$ and $g_4$ represent distinct clusters. The computation of the reference points of these clusters, according with STEP 3, produces the points $P_1$ and $P_2 = P_3$, as shown in Figure  \ref{fig:example3}[b]. Note that in this case the reference points for the two clusters containing respectively $g_2$ and $g_4$ coincide, and thus we have only two distinct reference points for the three clusters.

%\JP{*** With 3 clusters we should have three reference points, am I confused? ***}

\begin{figure}[h!]
    \centering
    \subfloat[\centering a]{{\includegraphics[width=5cm]{figures/example_step_4.png} }}%
    \qquad
    \subfloat[\centering b]{{\includegraphics[width=5cm]{figures/example_final.png} }}%
        \caption{[a] STEP 4, [b] STEP 5 for the illustrative example}%
    \label{fig:example4}%
\end{figure}

\noindent
STEP 4 of the heuristic procedure generates the tour of the mothership along the origin point, $P_1$, $P_2$ and the destination point, as shown in Figure \ref{fig:example4}[a]. This tour returns also the order in which the clusters are visited (and thus, also the order of visit to the target graphs) and this permits to set the values of the variables $u^{e_{g}td}$ and $v^{e_{g}td}$ of the \AMD\space model.\\
\noindent 
By providing the initial partial solution obtained by the values of the variables $u^{e_{g}td}$ and $v^{e_{g}td}$, STEP 5 solves the \AMD\space model and returns the final feasible solution shown in Figure \ref{fig:example4}[b]. From it we can observe that the sequence of visit of the target graphs does not change with respect to the one provided by STEP 4. The fleet of two drones first visits graphs $g_1$ and $g_3$ starting from the launching point $x^1_L$. Then, both drones are retrieved by the mothership at point $x^1_R$. The mothership moves to the point $x^2_L$  where one drone is launched for visiting graph $g_2$. Then the mothership reaches point $x^2_R$ to retrieve the drone and from the same point it launches the other drone for visiting graph $g_4$. Then, this drone is retrieved by the mothership at point $x^3_R$ before moving to the final destination point.


\begin{figure}[h!]
    \centering
    \subfloat[\centering a]{{\includegraphics[width=5cm]{figures/example_final-g1.png} }}%
    \qquad
    \subfloat[\centering b]{{\includegraphics[width=5cm]{figures/example_final-g3.png} }}%
     \qquad
    \subfloat[\centering c]{{\includegraphics[width=5cm]{figures/example_final-g2_g4.png} }}%
    \caption{Zoom on the tour on each target graph provided by STEP 5}%
    \label{fig:example5}%
\end{figure}

\noindent 
Focusing on each single target graph, Figure \ref{fig:example5} shows the zoom on the tours followed by the drones. For example, Figure \ref{fig:example5}[a] reports the one performed by the drone that visits graph $g_1$. The drone starts from the mothership at point $x^1_L$ and first visits the segment $\overline{R^1_1L^1_1}$. From point $L^1_1$ the drone moves to the second visited edge of graph $g_1$ visiting the segment $\overline{R^2_1L^2_1}$.
Finally, the drone leaves the graph from point $L^2_1$ and it is retrieved by the mothership at point $x^1_R$. Note that in this example the drones do not visit the full 100\% of each graph, but only a pre-specified percentage of each one of them.

\bigskip
\noindent
The reader may notice that the above algorithm can be also used to generate solutions for the model without synchronization  commented in Section \ref{amdasyn} since any solution of the synchronous model is also feasible for the asynchronous one. 

\begin{comment}
\JP{ \textbf{\noindent ***   NOT CLEAR THAT WE SHOULD INCLUDE THIS PART  (JUSTO: dixit) ***}
\bigskip

\noindent
As we already explained in Section \ref{amdasyn}, we also studied a variant of the \AMD\space model in which the mothership can launch and retrieve a drone in different stages. We designed a matheuristic also for this case with similar steps to the one previously presented.
The idea of this procedure is first solving the model with only one available drone (see \cite{art:Amorosi2021}) to determine the optimal launching/rendezvous points associated with each target graph and the corresponding minimum length of the mothership tour.
Then, a clustering procedure, like the one adopted in the matheuristic proposed for the synchronous case, is performed.
After that, the \AMD\space model without synchronization is solved on each cluster setting the launching point of the first cluster equal to the origin. Then the last retrieving point so determined is set as launching point of the next cluster and so on. From the solution obtained for each cluster the total length of the mothership tour is computed as the sum of the partial lengths of each tour associated with each cluster. The same procedure is repeated by starting the clustering procedure with different random seed.\\
In the following, we present the pseudo-code of this algorithm:

\begin{itemize} 
\item[STEP 1] (Launching/rendezvous points)
Solve the AMDRPG model and let $x_L^g$ and $x_R^g \forall g \in \mathcal{G}$ the associated optimal launching/rendezvous points and let $L$ be the associated minimum length of the mothership tour.  
\item[STEP 2] (Clustering procedure)
Initialization: define one cluster for each target graph and set $nit=1$ \\
Select randomly two clusters $C_i$ and $C_j$ (where $i<j$).\\
Check if the number of graphs belonging to the union of $C_i$ and $C_j$ is less than or equal to the number of available drones $n_D$.\\
If this condition is satisfied:\\
search for the point $C$ satisfying the following capacity constraint:
$$
\frac{[d(C, R^{e_g}) + C^{e_{g}e^{'}_{g}} + d(C,L^{e^{'}_{g}})]}{v_D} \leq cap \:\: \forall R^{e_g}, L^{e^{'}_{g}} \in C_i, \:\: C_j
$$
If such a point exists, merge the two clusters and assign to the resulting cluster so obtained the label $C_i$.\\

\item[STEP 3](Launch/rendezvous points exchanges)
Set $i=1$ and $x_L=orig$\\
For each cluster $C_i$ generated at STEP 2:\\
- solve the \AMD\space model with first launching point equal to $x_L$.\\
- let $x_R$ be the last rendezvous point associated with the cluster under analysis, set $x_L = x_R$.\\
Let $L'$ be the associated minimum length of the mothership tour computed as sum of the partial lengths of the tours associated with the clusters.\\
If $L' < L$ update the solution.\\
Set $nit=nit+1$.\\
Repeat STEP 2 and STEP 3 while $nit < maxit$
\end{itemize}
}
\end{comment}




==> Mothership Drone/introduction.tex <==
\section{Introduction}
In recent years the grow of the potential business opportunities related to the use of drone technology has motivated the appearance of an interesting body of methodological literature on optimizing of the use of such technology. 
We can find examples of that in many different sectors, like telecommunication where drones can be adopted in place of traditional infrastructures to provide connectivity (see for example \cite{art:Amorosi2018}, \cite{art:Chiaraviglio2018}, \cite{Jimenez2018}, \cite{art:Amorosi2019}, and \cite{art:Chiaraviglio2019a}), or to temporary deal with the damages caused by a disaster (\cite{art:Chiaraviglio2019}), deliveries (see for example \cite{art:Mathew2015} , \cite{art:Ferrandez2016}, \cite{art:Poikonen2020} and \cite{art:Amorosi2020}), also in emergency contexts (\cite{art:Wen2016}), inspection (\cite{art:Trotta2018}) and others.
The reader is referred to the recent surveys \cite{art:Otto2018} and \cite{art:Chung2020} for further details.\\
\noindent
Among the different aspects that can be considered we want to focus, for its relationship to the development in this paper, to the design, coordination and optimization of the combined routes of drones with a base vehicle. After the initial paper \cite{MURRAY201586} by Murray and Chu, where a combined model of truck and drone is considered, the work of Ulmer and Thomas \cite{Ulmer2018} also considers another model where trucks and drones are dispatched as order are placed and analyze the effect of different policies for either the truck or the drone. Other papers, as for instance, \cite{art:Campbell2017}, \cite{art:Carlsson2017} and \cite{art:Dayarian2017}, have also considered hybrid truck-and-drone models in order to mitigate the limited delivery range of drones. Poikonen and Golden, in \cite{Poikonen2019}, advance on the coordination problem considering the \textit{Mothership and drone routing problem} where these two vehicles are used to design a route that visits a number of points allowing the truck to launch and recover the drone in a continuous space. More recently in \cite{art:Poikonen2020} the authors consider the \textit{$k$-Multi-Visit drone routing problem} where a truck that acts as a mobile depot only allowed to stop in a predefined set of points, launches drones that can deliver more than one package to their designated destination points.
\noindent
Many of these papers make the assumptions that the set of allowable locations to launch/retrieve a drone are fixed and known a priori, the operations performed by the drone consist of delivering to a single point and the coordination is between a truck and a single drone. These assumptions may be appropriate in some frameworks but in other cases it may be better to relax them.\\
\noindent
In particular, only few papers in literature focus on drones operations consisting in traversing graphs rather than visiting single points. Campbell et al. 
\cite{art:Campbell2018} introduce the \textit{Drone Rural Postman Problem} (DRPP). The authors present a solution algorithm based on the approximation of curves in the plane by polygonal chains and that iteratively increases the number of points in the polygonal chain where the UAV can enter or leave. Thus, they solve the problem as a discrete optimization problem trying to better define the curve by increasing the number of points. The authors consider also the case in which the drone has limited capacity and thus it cannot serve all the lines. To deal with this latter case, they assume to have a fleet of drones and the problem consists in finding a set of routes, each of limited length.\\
In \cite{art:CAMPBELL202160}  this problem has been defined as the \textit{Length Constrained K-drones Rural Postman Problem}, a continuous optimization problem where a fleet of homogeneous drones have to jointly service (traverse) a set of (curved or straight) lines of a network. The authors design and implement a branch-and-cut algorithm for its solution and a matheuristic algorithm capable of providing good solutions for large scale instances of the problem.\\
Scanning the literature of arc routing problems involving hybrid systems consisting in one vehicle and one or multiple drones, the number of contributions is rather limited.\\
In \cite{art:Tokekar2016} the authors study the path planning problem of a system composed of a ground robot and one drone in precision agriculture and solve it by applying orienteering algorithms. Also the paper \cite{art:Garone2010} studies the problem of paths planning for systems consisting in a carrier vehicle and a carried one to visit a set of target points and assuming that the carrier vehicle moves in the continuous space.\\
To the best of our knowledge, only the paper \cite{art:Amorosi2021}, deals with the coordination of a mothership with one drone to visit targets represented by graphs. The authors made different assumptions on the route followed by the mothership: it can move on a continuous framework (the Euclidean plane), ii) on a connected piecewise linear polygonal chain or iii) on a general graph. In all cases, the authors develop exact formulations resorting to mixed integer second order cone programs and propose a matheuristic algorithm capable to obtain high quality solutions in short computing time.
\\
In this paper we deal with an extension of the problem studied in \cite{art:Amorosi2021} for which we propose a novel truck-and-multi-drones coordination model. We consider a system where a base vehicle (mothership) can stop anywhere in a continuous space and has to support the launch/retrieve of a number of drones that must visit graphs. The contribution on the existing literature is to extend the coordination beyond a single drone to the more cumbersome case of several drones and the operations to traversing graphs rather than visiting single points. In particular, we focus on a synchronous version in which every drone is launched and retrieved in the same stage. We present a mathematical programming formulation, valid inequalities to reinforce it and a matheuristic to deal with large instances of this problem. Moreover, we discuss and show how to extend further the former case to the  asynchronous situation where one assumes that the mothership can retrieve one drone in a different stage from the one in which it has been launched.\\
\noindent
The work is structured as follows: Section 2 provides a detailed description of the problem under consideration and develops a valid mixed integer non linear programming formulations for it. Section 3  provides some valid inequalities that strengthen the formulation and also derives upper and lower bounds on the big-M constants introduced in the proposed formulation. Section 4 presents details of the matheuristic algorithm designed to handle large instances. In Section 5 we report the results obtained testing the formulation and the matheuristic algorithm on different classes of planar graphs in order to assess its effectiveness. Finally, Section 6 concludes the paper.

==> Mothership Drone/literature.tex <==
\section{State of the art}
In this section we focus mainly on the previous works in literature related to systems where UAVs are assisted by a vehicle in order to serve a set of targets.
In these configurations the vehicle represents a launch and a recharging station for the UAVs and the main problem consists in coordinating the operations performed by one or multiple drones and the mothership.
Most of the previous works in literature on this subject are focused on node routing problems (NRPs), where the vehicle moves on a road network and the drone is used to visit target points outside the road network. 
Many of them are related to applications in the delivery sector where the set of targets to be visited is represented by a set of customers.
For example, \cite{art:Mathew2015} studies a delivery system consisting in one drone and one truck. The UAV visits one customer for each trip and the truck can wait at the launching node for the drone to come back or move to a different rendezvous node. In \cite{art:Carlsson2018} the authors study a continuous approximation on the Horse Fly Problem, where the truck is used as a mobile depot for the drone. In \cite{art:Campbell2017} the authors evaluate the economic impact of truck-and-drone hybrid models for deliveries by means of a continuous approximation model, considering different model parameters and customer densities. \cite{art:Ferrandez2016} focuses on a delivery system where one truck supports the operations of multiple drones. The authors first clusterize the customer demand by adopting a K-means algorithm to find truck stops that represent hubs for drone deliveries. Then, they determine a TSP of the truck among centroids of these clusters, by means of a genetic algorithm, assuming that drones are not constrained by flight range. In \cite{art:Moshref2017} the authors consider a similar delivery system where at each stop site the truck waits until all drones come back before moving to the next site. The goal is the minimization of the latency in a customer-oriented distribution system. Moreover, the authors compare the benefits of using drones for a single trip versus multiple trips. In \cite{art:Poikonen2020} the authors formalize the k-Multi-visit Drone Routing Problem (k-MVDRP) considering a tandem between a truck and a fleet of k drones. The authors assumed that each drone can deliver one or more packages to customers in a single mission. Each drone may return to the truck to swap/recharge batteries, pick up a new set of packages, and launch again to customer locations. Moreover, the authors decouple the set of launch locations from the set of customer locations. The article presents a mathematical formulation including a drone energy drain function that takes into account each package weight, but the problem is then solved by means of a heuristic algorithm.
\cite{art:Amorosi2020} presents a multi-objective mixed integer linear programming model for the management of a hybrid delivery system consisting in one base vehicle and a fleet of drones. As in \cite{art:Poikonen2020}, the set of launch locations is assumed to be different from the set of customer locations. The problem consists in determining the tour of the base vehicle and the assignments of the customers to the UAVs simultaneously optimizing the distance travelled by the vehicle, the one travelled by the drones and the maximum completion time. The model is solved on two realistic urban scenarios providing a partial exploration of the Pareto frontier of the problem by means of the weighted sum method.\\
Other examples of similar configurations in which a base vehicle supports the operations of one or multiple drones can be found also in other sectors. 
\cite{art:Trotta2018} studies, for example, the city-scale video monitoring of a set of points of interest performed by a fleet of UAVs whose operations are supported by buses and the problem is modeled as a mixed integer linear programming model based on a multi-period directed graph.
However, in all the works mentioned so far, the combined operations of vehicles and drones examine routing for a set of locations and these configurations exploit only part of the advantages of the adoption of drones. Indeed, UAVs can move between any two points in the space not following the road network. Thus, they can be adopted also for other kind of services in which the targets are represented by edges or part of them. This leads to another class of models, that is arc routing problems (ARPs).\\
With respected to NRPs, in the case of ARPs with drones there are relatively few papers. \cite{art:Oh2011} and \cite{art:Oh2014} study a coordinated road network search problem with multiple UAVs and they formulated it as a Multi-choice Multi-dimensional Knapsack Problem minimizing the flight time. This is a modified Chinese Postman Problem taking into account the UAVs energy capacity constraints. The authors solved the problem by means of a greedy insertion heuristic that models drone travel distance between the road components as a Dubins path.
\cite{art:Dille2013} faces the area coverage problem in sparse environments with multiple UAVs. Also in this case the UAVs motion is modeled using Dubins paths and it is assumed that they are equipped with a coverage sensor of a given radius.
The edge covering problem is solved by discretizing the network in orbits and then solving a TSP among this set of orbits. The authors compares the results obtained with the ones obtained with the method by \cite{art:Oh2014}, for simulated urban, suburban and rural scenarios, showing that for suburban densities their method outperforms both with one or multiple UAVs. 
In \cite{art:Chow2016} the authors deal with the problem of dynamically allocate a finite set of UAVs to links in a network that need monitoring, over multiple time periods. The need of drone monitoring is based on data related to traffic conditions. They formulated the first deterministic multi-period arc-inventory routing problem and then its stochastic dynamic version solved with an approximate dynamic programming algorithm. 
Another work related to multiple-period real-time monitoring of road traffic, adopting UAVs, is \cite{art:Li2018}. The authors proposed a mixed integer programming model combining the capacitated arc routing problem with the inventory routing problem and designed a local branching based method for dealing with large instances.\\
The ARPs with one UAV, have common characteristics with problems arising in path generation for laser cutting machines or drawing plotters. In particular, the authors of \cite{art:Campbell2018} studied the Drone Rural Postman Problem (DRPP) showing the relation with the Intermittent Cutting Problem (ICP). They presented a solution algorithm based on the approximation of curves in the plane by polygonal chains and that iteratively increases the number of points in the polygonal chain where the UAV can enter or leave. Thus, they solved the problem as a discrete optimization problem trying to better define the line by increasing the number of points. The authors considered also the case in which the drone has limited capacity and thus it cannot serve all the lines. To deal with this latter case, the authors assumed to have a fleet of drones and the problem consisted in finding a set of routes, each of limited length.\\
The literature related to Drone ARPs is limited with respect to the one related to Drone NRPs.
However, as regards arc routing problems involving a hybrid system consisting in one vehicle and one or multiple drones, the number of contributions in literature is further restricted and we can just mention \cite{art:Tokekar2016} and \cite{art:Garone2010}.\\
In \cite{art:Tokekar2016} the authors studied the path planning problem of a system composed of a ground robot and one drone in precision agriculture and solved it by applying orienteering algorithms. \cite{art:Garone2010} studied the problem of paths planning for systems consisting in a carrier vehicle and a carried one to visit a set of target points and assuming that the carrier vehicle moves in the continuous space. In particular, the authors formulated two different problems: the first one consisting in determining the takeoff/landings sequences of the carried vehicle to visit a set of points, assuming that in each mission of the carried vehicle only one target can be visited. The second one in which this constraint is removed permitting to the carried vehicle to visit more than one target in a single mission, before returning to the carrier vehicle. Heuristic approaches have been proposed to deal with both problems.\\
To the best of our knowledge none of the previous papers in literature deals with a drone arc routing problem combined with a node routing problem for a hybrid system consisting of one vehicle and one drone.
In this paper we present new Mixed Integer Non-Linear Programming (MINLP) formulations for the problem of coordinating a system composed of a mothership (the base vehicle) which supports the operations of one drone which has to visit a set of targets represented by graphs, with the goal of minimizing the total distance travelled by both vehicles.
Indeed, differently from the previous works in literature, we assume the drone can move freely on the continuous space. As regards the mothership, we studied both cases in which also the base vehicle can move freely on the continuous space or it is constrained to move on a road network, of different typologies, where launching and rendezvous points can be chosen.
The main contributions of this article can be summarized as follows:
\begin{itemize}
    \item New mathematical formalization of the coordinating problem of a base vehicle and one drone in the continuous space to visit a set of targets represented by graphs;
    \item Design of new alternative second order cone MINLP formulations;
    \item A new matheuristic algorithm to deal with large instances able to provide high quality solutions in short time;
    \item Extensive experimental analysis comparing the exact solution of the formulations and the matheuristic on a set of generated instances involving different typology of planar graphs.
\end{itemize}
 



==> description_old.tex <==
\section{Description of the Problem}
\JP{In the Mothership and Drone Routing Problem with Graphs (MDRPG), there is one mothership (the base vehicle) and one drone and the problem consists on the coordination between the drone and the base vehicle to minimize the total distance travelled by both vehicles. \JP{In this case, for the sake of simplicity, we assume that there exist no obstacles to prevent drone travel from moving in straight line segments. Nevertheless, that extension is interesting to be further considered although is beyond the scope of this paper.}

The mothership and the drone begin at a starting location, denoted $orig$. There exists a set $\mathcal G$ of target locations modeled by graphs that must be visited by the drone. The natural application for this situation comes from road or wired network inspection. For each stage $t \in \{1, \ldots, |\mathcal G|\}$, we require that the drone is launched from the current mothership location, that at stage $t$ is a decision variable denoted by $x_L^t$, flies to one of the graphs that has to be visited $g$, traverses the required portion of $g$ and then returns to the current position of the mothership, that most likely is different from the launching point $x_L^t$, and  that is another decision variable denoted by $x_R^t$. Once all targets graphs have been visited, the mothership and drone return to a final location (depot), denoted by $dest$.

Let $g = (V_G, E_G)$ be a graph in $\mathcal G$ whose total length is denoted by $\mathcal L(g)$ and $i_g$ that denotes the edge $e$ of this graph $g$. This edge is parametrized by its endpoints $B^{i_g}, C^{i_g}$ and its length $\|\overline{B^{i_g}C^{i_g}}\|$ is denoted by $\mathcal L(i_g)$. For each line segment, we assign a binary variable $\mu^{i_g}$ that indicates whether or not the drone visits the segment $i_g$ and define entry and exit points $(R^{i_g}, \rho^{i_g})$ and $(L^{i_g}, \lambda^{i_g})$, respectively, that determine the portion of the edge visited by the drone. }

We have considered two modes of visit to the targets graphs $g\in \mathcal{G}$:
\begin{itemize}
    \item Visiting a percentage $\alpha^{i_g}$ of each edge $i_g$ which can be modeled by using the following constraints:
    \begin{equation}\label{eq:alphaE}\tag{$\alpha$-E}
    |\lambda^{i_g} - \rho^{i_g}|\mu^{i_g}\geq \alpha^{i_g}, \quad \forall i_g, \forall g.
    \end{equation}
    \item Visiting a percentage $\alpha_g$ of the total length of the graph:
    \begin{equation}\label{eq:alphaG}\tag{$\alpha$-G}
    \sum_{i_g} \mu^{i_g}|\lambda^{i_g} - \rho^{i_g}|\mathcal L(i_g) \geq \alpha_g\mathcal L(g), \quad \forall g
    \end{equation}
    where $\mathcal L(g)$ denotes the total length of the graph.
\end{itemize}

\bigskip

In both cases, we need to introduce a binary variable that determines the traveling direction on the edge $i_g$ as well as the definition of the parameter values $\nu_\text{min}^{i_g}$ and $\nu_\text{max}^{i_g}$ of the access and exit points to that segment. Then, for each edge $i_g$, the absolute value constraint \eqref{eq:alphaE} can be represented by:

\begin{equation}\label{eq:alpha-E}\tag{$\alpha$-E}
 \mu^{i_g}|\rho^{i_g}-\lambda^{i_g}|\geq \alpha^{i_g} \Longleftrightarrow
 \left\{
 \begin{array}{ccl}
  \rho^{i_g} - \lambda^{i_g}                       & =    & \nu_\text{max}^{i_g} - \nu_\text{min}^{i_g}                                     \\
  \nu_\text{max}^{i_g}                         & \leq & 1-\text{entry}^{i_g}                                    \\
  \nu_\text{min}^{i_g}                      & \leq & \text{entry}^{i_g},                                        \\
  \mu^{i_g}(\nu_\text{max}^{i_g} + \nu_\text{min}^{i_g} ) & \geq & \alpha^{i_g}
  \\
 \end{array}
 \right.
\end{equation}

The linearization of \eqref{eq:alphaG} is similar to \eqref{eq:alphaE} by changing the last inequality in \eqref{eq:alpha-E} for

\begin{equation}\label{eq:alpha-G}\tag{$\alpha$-G}
\sum_{i_g} \mu^{i_g}(\nu_\text{max}^{i_g} + \nu_\text{min}^{i_g})\mathcal L(i_g)\geq \alpha_g\mathcal L(g).
\end{equation}

\JP{In our model wlog, we assume  that the mothership and drone do not need to arrive at a rendezvous location at the same time: the
faster arriving vehicle may wait for the other at the rendezvous location. In addition, we also assume that vehicles move at constant speeds, although this hypothesis could be relaxed. The mothership travels at $v_M$ speed whereas the drone has a speed of $v_D$ > $v_M$. The mothership and the drone must travel together from $orig$ to the first launch location. Similarly, after the drone visits the last target location, the mothership and the drone must meet at the final rendezvous location before traveling together back to $dest$. The first launch location and final rendezvous location are allowed to be $orig$ and $dest$, respectively, but it is not mandatory. For the ease of presentation, in this paper we will assume that $orig$ and $dest$ are the same location. However, all results extend easily to the case that $orig$ and $dest$ are different locations.

The goal is to find a minimum time path that begins at $orig$, ends at $dest$, and where
every $g \in \mathcal G$ is visited by the drone.

Depending on the assumptions made on the movements of the mothership vehicle this problem gives rise to two different versions: a) the mothership vehicle can move freely on the continuous space (all terrain ground vehicle, boat on the water or flying vehicle); and b) the mothership vehicle must move on a travel network (that is, it is a normal truck or van). In the former case, that we will call All terrain Mothership-Drone Routing Problem with Graphs (\AMD), each launch and rendezvous location may be chosen from a continuous space (the Euclidean 2-or-3 dimension space). In the latter case, that we will call Network Mothership-Drone Routing Problem with Graphs (\NMD) from now on, each launch and rendezvouz location must be chosen on a given graph embedded in the considered space. For the sake of presentation and length  of the paper, we will focus in this paper, mainly, on the first model \AMD. The second model, namely \NMD, is addressed using similar techniques but providing slightly less details.}




==> formulations_old.tex <==
\section{Mixed Integer Non Linear Programming Formulations}
In this section we present alternative MINLP formulations for the (\MDR) depending on the nature of  the mothership  that will be compared computationally in later sections. We start analyzing first the situation where the mothership moves in a continuous space, namely the (\AMD). 
%We shall address later the second model (\NMD). As it will clear later, we will elaborate from the previous model modifying some intrinsic conditions that characterize each problem.

A first attempt to model this problem uses stages identified with the order in which the different elements in the problem are visited. We identify each visit to one of the target graphs with a stage of the process. Then, by using the notation below, in each stage $t\in \{1,\ldots,|\mathcal G|\}$, the drone follows the following path starting from the mothership, visiting the required edges of $G$ and returning to the mothership:

$$
x_L^t\rightarrow R^{i_g}\rightarrow L^{i_g}\rightarrow\ldots\rightarrow R^{j_g}\rightarrow L^{j_g}\rightarrow \ldots \rightarrow R^{u(g)} \rightarrow x_R^t\rightarrow x_L^{t+1}.
$$

This path calls in a natural way for the definition of binary variables that choose:
\begin{itemize}
    \item The optimal order to visit each graph $g\in\mathcal G$. In other words, defining the sequence of the stages.
    \item The optimal order to visit the edges of each graph in its corresponding stage.
\end{itemize}

Thus, to this end one can define the following binary variables:
\begin{itemize}
    \item $u^{i_gt} = 1$ if the drone enters by the segment $i_g$ at the stage $t$.
    \item $z^{i_gj_g} = 1$ if the drone goes from the segment $i_g$ to the segment $j_g$.
    \item $v^{i_gt} = 1$ if the drone exits the graph by the segment $i_g$ at the stage $t$.
\end{itemize}

By using these binary variables, we can model the route that follows the drone:
\begin{align}
    \sum_{i_g} u^{i_gt} & = 1, &\quad\forall t \label{st:DEnt}\\%\tag{DEn}\\
    \sum_{i_g} v^{i_gt} & = 1, &\quad\forall t \label{st:DExt}\\%\tag{DEx}\\
    \sum_{i_g, t} u^{i_gt} & = 1, &\quad\forall g \label{st:DEng}\\%\tag{D
    \sum_{i_g, t} v^{i_gt} & = 1, &\quad\forall g \label{st:DExg}\\%\tag{D
    \sum_{i_g} u^{i_gt} & = \sum_{i_g} v^{i_gt}, &\quad\forall g, t \label{st:Duv}\\%\tag{D
    \sum_{j_g} z_g^{j_gi_g} + \sum_{t} u^{i_gt} & = \mu^{i_g}, &\quad\forall i_g \label{st:DInu}\\
    \sum_{j_g} z_g^{i_gj_g} + \sum_{t} v^{i_gt} & = \mu^{i_g}, &\quad\forall i_g \label{st:DInv}
\end{align}

Equations \eqref{st:DEnt} and \eqref{st:DExt} state that in each stage the drone visits (enter and exit, respectively) only one graph. Constraints \eqref{st:DEng} and \eqref{st:DExg} assure that each graph is visited at some stage. Constraints \eqref{st:DInu} (resp. \eqref{st:DInv}) say that the number of exterior edges plus the number of interior edges that enter (resp. exit) to the edge $i_g$ is given by $\mu^{i_g}$.

\subsubsection*{Elimination of subtours}
To prevent the existence of subtours within each graph $g\in \mathcal G$ that the drone must visit, one can include, among others, either the compact formulation that uses the Miller-Tucker-Zemlin constraints or the subtour elimination  constraints (SEC).

For the MTZ formulation, we define the continuous variables $s^{i_g}$ that indicate the order to visit the edge $i_g$ and establish the following constraints for each $g\in\mathcal G$:

\begin{align}
    s^{i_g} - s^{j_g} + |E_g|z^{i_gj_g} & \leq |E_g| - 1  , &\quad\forall i_g\neq j_g \tag{MTZ$_1$} \label{MTZ1}\\
    0 & \leq s^{i_g} \leq |E_g| - 1 &\quad\forall i_g\tag{MTZ$_2$}\label{MTZ2}
\end{align}

Alternatively, we can also use the family of subtour elimination constraints:
\begin{equation}\tag{SEC}\label{SEC}
    \sum_{i_g, j_g \in S} z_g^{i_gj_g} \leq |S| - 1, \quad \forall g \in \mathcal G,\quad \forall S\subset E_g
\end{equation}

%(Copiado del XPPN)
Since there is an exponential number of SEC constraints, when we implement this formulation we need to perform a row generation procedure including constraints whenever they are required by a separation oracle. To find SEC inequalities, as usual, we search for disconnected components in the current solution. Among them, we choose the shortest subtour found in the solution to be added as a lazy constraint to the model.

 \subsection{All terrain Mothership-Drone Routing Problem with Graphs}
In this problem, we assume that the mothership  is allowed to move freely in a continuous space: $\mathbb R^2$ or $\mathbb R^3$. The goal of the \AMD is to find a feasible solution that minimizes the total distance traveled  by the drone and  the mothership. Hence, assuming that lengths are given by the Euclidean distance, $\|\cdot\|_2$, between their endpoints, to account for the different distances among the decision variables of the model we need to define the following instrumental variables:
\begin{itemize}
    \item $d_L^{i_gt} = \|x_L^t - R^{i_g}\|$. Distance traveled by the drone from the launch point at the stage $t$ to the first visiting point in the segment $i_g$.
    \item $d^{i_gj_g} = \|R^{i_g} - L^{j_g}\|$. Distance traveled by the drone from the launch point in $i_g$ to the rendezvous point in $j_g$.
    \item $d^{i_g} = \|R^{i_g} - L^{i_g}\|$. Distance traveled by the drone from the retrieve point  to the next launch point in $i_g$.
\end{itemize}

\subsubsection{A first formulation for \AMD \ based on stages}
\JP{A natural approach to model this problem is to consider stages which are identified with the targets that the drone has to visit. This way the problem needs to considers $|\mathcal{G}|$ stages that are indexed by $t=1,\ldots, |\mathcal{G}|$. To provide a valid formulation for the model under this approach, we introduce the following variables:
\begin{itemize}
    \item $d_R^{i_gt} = \|L^{i_g} - x_R^t\|$. Distance traveled by the drone from the launch point in the segment $i_g$ to the retrieve point on the mothership at the stage $t$.
    \item $d_{LR}^t = \|x_L^t - x_R^t\|$. Distance traveled by the mothership from the launch point to the retrieve point at the stage $t$.
    \item $d_{RL}^t = \|x_R^t - x_L^{t+1}\|$. Distance traveled by the mothership from the retrieve point at the stage $t$ to the launch point at the stage $t+1$.
\end{itemize}

Therefore, the following formulation minimizes the overall distance traveled by the mothership and drone coordinating their movements and ensuring the required coverage of the targets.}
\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{} \label{AMDRPG-ST} \tag{AMDRPG-ST}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^t\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|x_R^t- x_L^{t+1}\|}{\leq d_{RL}^t,\quad}{\forall i_g,t}{}
 \addConstraint{\|x_L^t- x_R^t\|}{\leq d_{LR}^t,\quad}{\forall i_g,t}{}
 \addConstraint{\left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}), \quad}{\forall g, t}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{The objective function has four terms: the first and fourth ones compute the distances to go to and return from the mothership to the target graph $g$ visited at the stage $t$, the second one accounts for the distance traveled by the drone on the edges of the target graph $g$ between two consecutive \textit{jumps} between edges, and the third one computes the distances traveled by the drone while it \textit{jumps} between two consecutive edges on the target graph $g$. Constraints \eqref{st:DEnt}-\eqref{st:DInv} models the route followed by the drone, \eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G} ensure that the displacement of the drone in each visit to a target graph is a Hamiltonian route, \eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G} defines what is required in each visit to a target graph. Then, the next six constraints models Euclidean distances needed in the model.}
Constraints \eqref{ACW} ensure that the time spent by the drone to visit the graph $g$ at the stage $t$ is less than or equal to the time that the mothership needs to move from the launch point to the retrieve point at the stage $t$. If we want to penalized the waiting time of the drone, we can add a slack variable in the restriction that has to be included in the objective function. %

Observe that we are assuming constant velocities for the mothership $v_M$ and the drone $v_D$.
%(Meto restricción de capacidad? para hacer experimentos puede complicarse)

To deal with the bilinear terms of the objective function, we use McCormick's envelopes to linearize these terms by adding variables $p\geq 0$ that represent these products and introduce these constraints:
\begin{align*}
    p & \geq  m z, \\
    p & \leq d - M(1 - z),
\end{align*}
where $m$ and $M$ are, respectively, the lower and upper bounds of the distance variable $d$. These bounds will be adjusted for each bilinear term in Section \ref{bounds}.

 \subsubsection{Alternative formulations for \AMD  based on enforcing connectivity: MTZ-constraints and subtour elimination-constraints (SEC)\label{sec:AMDMTZ}}
 
\JP{In this family of formulations we replace the variables $u^{\cdot t},\; v^{\cdot t}$ and constraints that model the tour using stages, namely (\ref{st:DEnt})-(\ref{st:DInv}), by constraints that ensure connectivity. We will distinguish two different approaches. The first one is based on the rationale of Miller-Tucker-Zemlin (MTZ) whereas the second one uses an extended formulation based on SEC.} 

We start presenting the formulation based on MTZ. It requires the definition of two families of binary variables that choose:
\begin{itemize}
    \item The optimal order to visit the  graphs $g\in\mathcal G$ in the tour of the mothership.
    \item The optimal order to visit the edges of each graph.
\end{itemize}

The above concepts can be modeled with the following binary variables:
\begin{itemize}
    \item $u^{i_g} = 1$ if the drone accesses the segment $i_g$.
    \item $z^{i_gj_g} = 1$ if the drone goes from the segment $i_g$ to the segment $j_g$.
    \item $v^{i_g} = 1$ if the drone exits the graph  $g$ by the segment $i_g$.
    \item $w^{gg'} = 1$ if the mothership goes from $x_L^g$ to $x_R^{g'}$.
\end{itemize}

By using these binary variables, we can model the route that follows the drone in each particular graph $g\in \mathcal G$:
\begin{align}
    \sum_{i_g} u^{i_g} & = 1, \label{DEnt2}\\%\tag{DEn}\\
    \sum_{i_g} v^{i_g} & = 1, \label{DExt}\\%\tag{DEx}\\
    \sum_{j_g} z^{j_gi_g} + u^{i_g} & = \mu^{i_g}, &\quad\forall i_g \label{DInu}\\
    \sum_{j_g} z^{i_gj_g} + v^{i_g} & = \mu^{i_g}, &\quad\forall i_g \label{DInv2}
\end{align}

On the other hand, to model the tour followed by the mothership, we have to include the following new constraints:
\begin{align}
    \sum_{g\in\mathcal G} w^{g0} & = 0, \label{TOrig}\\
    \sum_{g'\in\mathcal G} w^{(n_G+1) g'} & = 0, \label{TDest}\\
    \sum_{g'\in\mathcal G'\setminus\{g\}} w^{gg'} & = 1, \label{TExt} &\quad\forall g\in \mathcal G\\
    \sum_{g\in\mathcal G'\setminus\{g'\}} w^{gg'} & = 1, &\quad\forall g'\in \mathcal G\label{TEnt}\\
    s_g - s_{g'} + |\mathcal G'|w^{gg'} & \leq |\mathcal G'| - 1  , &\quad\forall g \neq g' \tag{MTZ$_3$} \label{MTZ3}\\
    0 & \leq s_g \leq |\mathcal G'| - 1 &\quad\forall g\in \mathcal G\tag{MTZ$_4$}\label{MTZ4}\\
    s_0 & = 0, \tag{MTZ$_5$}\label{MTZ5}\\
    s_{n_G+1}&=n_G+1, \tag{MTZ$_6$}\label{MTZ6}
\end{align}

\JP{The reader may note that constraints (\ref{TExt}), (\ref{TEnt}) and (\ref{MTZ3})-(\ref{MTZ6}) are of the type MTZ for the complete graph $\hat G=(\hat N,\hat E)$ induced by the graphs $g\in \mathcal G$ to be visited, where a node $\hat e_g \in \hat N$ if $g\in \mathcal G$. Thus, we enforce that the mothership route follows a Hamiltonian tour on the graphs to be visited by the drone.  Next, we have to connect the visits of the drone to the graphs with the tour followed by the mothership. To this end, we require to introduce variables defining the launching and recovery points to account for the distances traveled and to defined the inner tour of the mothership. }


In this problem, we assume that the mothership is allowed to move freely in $\mathbb R^2$. Hence, assuming that lengths are given by the Euclidean distance, $\|\cdot\|_2$, between their endpoints, we need to define the following continuous variables that account for the distances among distinguished points:
\begin{itemize}
    \item $d_L^{i_g} = \|x_L^g - R^{i_g}\|$. Distance traveled by the drone from the launching point to the first visiting point in the segment $i_g$.
    \item $d^{i_gj_g} = \|R^{i_g} - L^{j_g}\|$. Distance traveled by the drone from the launching point in $i_g$ to the next rendezvous point $j_g$.
    \item $d^{i_g} = \|R^{i_g} - L^{i_g}\|$. Distance traveled by the drone from the retrieve point  to the next launch point in $i_g$.
    \item $d_R^{i_g} = \|L^{i_g} - x_R^g\|$. Distance traveled by the drone from the launch point in the segment $i_g$ to the retrieve point on the mothership.
    \item $d_{LR}^g = \|x_L^g - x_R^g\|$. Distance traveled by the mothership from the launch point to the retrieve point while the drone is visiting $g$.
    \item $d_{RL}^{gg'} = \|x_R^g - x_L^{g'}\|$. Distance traveled by the mothership from the retrieve point for the graph $g$ to the launch point associated to the graph $g'$.
\end{itemize}

\begin{figure}[h]
\centering
\includegraphics[height=9cm,width=\textwidth]{AMDRPG2.png}
\caption{Example illustrating the meaning of the launching  (L) and retrieving (R)  points. \label{fig:illustrative}}
\end{figure}

\JP{Figure \ref{fig:illustrative} shows an example of a configuration with two target graphs with four  nodes and four edges.%: one with six nodes and 7 edges and the other one with four nodes and edges%. 
The mothership begins at its starting point $x_L^0$. Then, it moves to $x_L^1$ where the drone is launched to visit the graph 2. There, the drone follows a route that ensures the coverage of $0.66 \%$ of the entire graph and returns to the point $x_R^2$ from where it is launched again to visit the second graph. Once, this graph is visited the drone returns to the mothership at the rendezvous point $x_R^2$ and so on ... }


\JP{In this formulation of \AMD the goal of is again to find a feasible solution that minimizes the total distance traveled  by the drone and  the mothership but without using stages. Instead the model ensures the Hamiltonian nature of the routes using the rationale of connectivity by the MTZ or SEC family of constraints. Therefore, modifying the previous formulation \sf{AMDRPG-ST}, replacing constraints based on stages, one obtains the following alternative valid formulation.}
\begin{mini*}|s|
 {}{\sum_{i_g} (u^{i_g}d_L^{i_g} + v^{i_g}d_R^{i_g}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_g d_{LR}^g + \sum_{g,g'}d_{RL}^{gg'}w^{gg'}}{}{}\label{AMDRPG-MTZ}\tag{AMDRPG-MTZ}
 \addConstraint{\eqref{DEnt2}-\eqref{DInv2}}{}{}
 \addConstraint{\eqref{TOrig}-\eqref{TEnt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
%\addConstraint{\eqref{MTZ3} - \eqref{MTZ6} \text{ or } \eqref{SEC} }{}{}   
 \addConstraint{\eqref{MTZ3} - \eqref{MTZ6}}{}{}   
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^g- R^{i_g}\|}{\leq d_L^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^g\|}{\leq d_R^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|x_R^g- x_L^{g'}\|}{\leq d^{gg'}_{RL},\quad}{\forall g,g'}{}
 \addConstraint{\|x_L^g- x_R^g\|}{\leq d^g_{LR},\quad}{\forall g}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g} d^{i_g} + \sum_{i_g}v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_{RL}^{g}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}


\JP{The formulation above \eqref{AMDRPG-MTZ} can be slightly modified replacing constraints $\eqref{MTZ3} - \eqref{MTZ6}$ by 
\begin{equation}\label{SEC-graph}
\sum_{g,g'\in \mathcal G} w^{gg'} \le |S|-1, \quad \forall S\subseteq \{1,\ldots, |\mathcal G|\}.
\end{equation}
This way we obtain another formulation for \AMD using SEC rather than MTZ constraints to represent the mothership tour. We will call this formulation (AMDRPG-SEC). Later, we will compare their performance in the computational results section.


\subsubsection{Comparing the formulations\label{ss:compare}}
A straightforward analysis of the two types of formulations, namely by stages and based on connectivity, shows that \ref{AMDRPG-MTZ} has much less variables and constraints than \ref{AMDRPG-ST}. Indeed, the latter requires definition of distance variables for each $i_g$ and $t$ which is a quadratic number rather than a linear one as used by the former. In addition, to enforce coordination \ref{AMDRPG-ST} needs constraints (DCW) for each $g\in \mathcal{G},\ t=1,\ldots,T$ whereas \ref{AMDRPG-MTZ} only uses (DCW) constraints for $g\in \mathcal{G}$. This is an important decrease in the dimension of the problems to be solved. This observation is confirmed in efficiency in problem solving in the section of computational experiments.} 


\subsection{Network Mothership-Drone Routing Problem on a Polygonal with Graphs (\PMD)}
The most significant difference between \AMD and  \PMD \ is that, in the latter, the mothership cannot move freely in $\mathbb R^2$ but it has to move on a network that models a road system where the mothership (truck) is restricted to move. \JP{An intermediate situation between moving freely and moving on a general road network is to assume that the mothership moves on a closed polygonal, namely a piecewise linear, chain. Modeling this situation is a transition step to achieve the more general case of the mothership moving on general networks. We will present the results for the \PMD \  following a scheme similar to that of \AMD. First, we present a model by stages and then another one based on connectivity constraints.}

Let $\mathcal P$ denote a polygonal chain parametrized by its breakpoints $A_1, \ldots, A_p$ ordered in the direction of travel. Observe that we are assuming that there exists a pre-specified orientation that determines the direction of the mothership's displacement. Let also $\gamma_L^{et}$ and $\gamma_R^{et}$ be the parameter values that define the points $x_L^t$ and $x_R^t$ on the edge $e$ on $\mathcal P$, respectively. \JP{Figure \ref{fig:ex1} illustrates the meaning of the parameters $\gamma_L^{et}$ and $\gamma_R^{et}$ on a polygonal chain with 4 pieces.} Then, the distance measured on the polygonal can be obtained by the following expressions:
\begin{equation}\tag{$d^{t\mathcal P}_{LR}$}\label{eq:dLRPt}
d_{LR}^{ee't} = \left\{\begin{matrix}
(\gamma_R^{et} - \gamma_L^{et})\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_L^{et})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{R}^{e't}\mathcal L(e')), & \text{if } e < e'.
\end{matrix}\right.
\end{equation}

\begin{equation}\tag{$d^{t\mathcal P}_{RL}$}\label{eq:dRLPt}
d_{RL}^{ee't} = \left\{\begin{matrix}
(\gamma_{L}^{et+1}-\gamma_R^{et})\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_R^{et})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{L}^{e't+1}\mathcal L(e')), & \text{if } e < e'.
\end{matrix}\right.
\end{equation}

This distance requires a binary variable $z_{LR}^{ee't}$ that determines whether $d_{LR}^{ee'}$ is defined by the first or the second expression in the formula:
$$z_{LR}^{ee't} = 1 \text{ if } \mu_{L}^{et} = 1 \text{ and }\mu_{R}^{e't} = 1,$$

\noindent where $\mu_{L}^{et}$ and $\mu_{R}^{et}$ are indicator variables that attain the value one if the launch point (resp. retrieve point) is placed in the segment $e$ of $\mathcal P$ at the stage $t$.

Similarly, we define $z_{RL}^{ee't}$:
$$z_{RL}^{ee't} = 1 \text{ if } \mu_{R}^{et} = 1 \text{ and }\mu_{L}^{e't+1} = 1.$$

In addition, we need to define continuous variables $\lambda_R^t$ and $\lambda_L^t$ that model the absolute position of the point $x_L^t$ in the polygonal to ensure that the movement of the mothership goes always in the allowed direction of travel and never comes back when it traverses the polygonal chain. 

\begin{figure}[h!]
\begin{center}
 \includegraphics[width=1\linewidth]{TDRPG.png}
\end{center}
\caption{An example of a parameterization of a mothership route that goes from $A_1$ to $x_L^t$ to launch the drone, then moves to $x_R^t$ on the edge $\overline{A_1A_2}$ to retrieve it, then it goes to $x_L^t$ on $\overline{A_2A_3}$ to launch it again, and travels until $x_R^t$ on $\overline{A_3A_4}$ to retrieve the drone and returns to the starting point at $A_1$.\label{fig:ex1}}
\end{figure}

With all this, we can model the movement of the mothership on the polygonal. For each stage $t$, we have

\begin{align}
    x_L^t & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{L}^{et}\left[A^i + \gamma_L^{et}(A^{i+1} - A^i)\right]\label{param1}\\
    x_R^t & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{R}^{et}\left[ A^i + \gamma_R^{et}(A^{i+1} - A^i)\right]\label{param2}\\
    z_{LR}^{ee't} & = \mu_{L}^{et}\mu_{R}^{e't}\label{pol:prodLR}\\
    z_{RL}^{ee't} & = \mu_{R}^{et}\mu_{L}^{e't+1}\label{pol:prodRL}\\
    \sum_{e} \mu_{L}^{et} & = 1  \label{muL} \\
    \sum_{e} \mu_{R}^{et} & = 1 \label{muR}\\
    d_{LR}^t & = \sum_{e, e'} z_{LR}^{ee't} d_{LR}^{ee'} \label{pol:dLRt},\\
    d_{RL}^t & = \sum_{e, e'} z_{RL}^{ee't} d_{RL}^{ee't} \label{pol:dRLt},\\
    \lambda_L^t - i & \geq \mu_{L}^{et} - (p-1)(1-\mu_{L}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaLg}\\
    \lambda_L^t - i & \leq \mu_{L}^{et} - (p-1)(1-\mu_{L}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaLl}\\
    \lambda_R^t - i & \geq \mu_{R}^{et} - (p-1)(1-\mu_{R}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaRg}\\
    \lambda_R^t - i & \leq \mu_{R}^{et} + (p-1)(1-\mu_{R}^{et}), \quad \forall e=(i, i+1)\in\mathcal P \label{lambdaRl}\\
    \lambda_R^t & \geq \lambda_L^t \label{lambdaRL}\\
    \lambda_L^{t+1} & \geq \lambda_R^t \label{lambdaLR}
\end{align}

\noindent where $d_{LR}^{ee'}$ and $d_{RL}^{ee't}$ are defined in \eqref{eq:dLRPt} and \eqref{eq:dRLPt}. Constraints \eqref{param1} and \eqref{param2} parameterize the launch and retrieve points on the polygonal chain. Constraints \eqref{pol:prodLR} and \eqref{pol:prodRL} model the product of binary variables. Constraints \eqref{muL} and \eqref{muR} state that, in each stage, the launch and retrieve points can be only in one segment, not necessarily the same. Constraints \eqref{pol:dLRt} and \eqref{pol:dRLt} compute the total distance between the launch and the retrieve point in each stage. Inequalities \eqref{lambdaLg}-\eqref{lambdaRl} link $\mu_{L}^{et}$ and $\lambda_L^t$ (resp. $\mu_{R}^{et}$ and $\lambda_R^t$). Finally, constraints \eqref{lambdaRL} and \eqref{lambdaLR} ensure that the mothership moves in the right direction on the polygonal. Note that, in this case, it is not required to account for the distance $d_{RL}^t$ because by the assumptions on the model the mothership will traverse all the polygonal chain (since we have imposed that the route starts and ends at the same point).


The goal of the (\PMD) is, once again, to find a feasible solution that minimizes the total distance covered by the mothership and the drone. Thus, gathering all the above constraints one gets the following valid formulation.
\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{}\tag{PMDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{param1}-\eqref{lambdaLR}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\eqref{eq:dLRPt}, \eqref{eq:dRLPt}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j_g}{}
 \addConstraint{\|L^{i_g}- x_R^t\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\hspace*{-1.5cm} \left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}), \,}{\forall g, t}{}\label{ACW}\tag{{\scriptsize DCW}}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}
\subsubsection{Alternative formulation for \PMD \  based on MTZ-constraints}

\JP{Analogously to the case of \AMD one can also model \PMD \ without any explicit reference to stages. Here, we will follow a very similar approach to that in Section \ref{sec:AMDMTZ} to describe the formulation for \PMD \ based on MTZ-constraints.}

Let $\mathcal P$ denote, as before,  the polygonal chain parametrized by its endpoints $A_1, \ldots, A_p$ ordered in the direction of travel. In addition, let also $\gamma_{L}^{eg}$ and $\gamma_{R}^{eg}$ be the parameter values that define the points $x_L^g$ and $x_R^g$ on the line segment $\overline{A_iA_{i+1}}$ in $\mathcal P$, respectively. \JP{Then, the distance traveled on the polygonal can be obtained by one of  the following expressions. The first one refers to distances covered by the mothership between the launching and retrieving points of a drone operation, whereas models the distance traveled by the mothership between the launching and retrieving points of two consecutive graphs targeted in its route.}
\begin{equation}\tag{$d_{LR}^{g\mathcal P}$}\label{eq:dLRPg}
d_{LR}^{ee'g} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg}|\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_{L}^{eg})\mathcal L(e) + \sum_{e'' =e+1}^{e'-1}\mathcal L(e'') + \gamma_{R}^{e'g}\mathcal L(e'), & \text{if } e < e', \\
\gamma_{L}^{eg}\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + (1-\gamma_{R}^{e'g})\mathcal L(e'), & \text{if } e > e'.
\end{matrix}\right.
\end{equation}

\begin{equation}\tag{$d_{RL}^{g\mathcal P}$}\label{eq:dRLPg}
d_{RL}^{ee'gg'} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg'}|\mathcal L(e), & \text{if } e = e',\\ 
(1 - \gamma_{R}^{eg})\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + \gamma_{L}^{e'g'}\mathcal L(e'), & \text{if } e < e',\\
\gamma_{R}^{eg}\mathcal L(e) + \sum_{e'' = e+1}^{e'-1}\mathcal L(e'') + (1-\gamma_{L}^{e'g'})\mathcal L(e'), & \text{if } e > e'.
\end{matrix}\right.
\end{equation}

\JP{This distance requires binary variables $z_{LR}^{ee'g}$ and $z_{RL}^{ee'gg'}$ that determines which of the expressions in \eqref{eq:dLRPg} and  \eqref{eq:dRLPg} define $d_{LR}^{ee'g}$ and $d_{RL}^{ee'gg'}$,respectively.}
$$z_{LR}^{ee'g} = 1 \text{ iff } \mu_{L}^{eg} = 1 \text{ and }\mu_{R}^{e'g} = 1,\qquad
z_{RL}^{ee'gg'} = 1 \text{ iff } \mu_{L}^{eg} = 1 \text{ and }\mu_{R}^{e'g'} = 1,
$$
where $\mu_{L}^{eg}$ and $\mu_{R}^{eg}$ are indicator variables that attain the value one if the launch point (resp. retrieve point) associated to the graph $g$ is placed in the segment $\overline{A_iA_{i+1}}$ of the edge $e=(i, i+1) \in \mathcal P$ .

With all this, we can model the movement of the mothership inside the polygonal. 

\begin{align}
    x_L^g & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{L}^{eg}\left[A^i + \gamma_L^{eg}(A^{i+1} - A^i)\right]\label{param1g}\\
    x_R^g & = \sum_{e=(i, i+1)\in\mathcal P} \mu_{R}^{eg}\left[ A^i + \gamma_R^{eg}(A^{i+1} - A^i)\right]\label{param2g}\\
    z_{LR}^{ee'g} & = \mu_{L}^{eg}\mu_{R}^{e'g}\label{prodLRg}\\
    z_{RL}^{ee'gg'} & = \mu_{R}^{eg}\mu_{L}^{e'g'}\label{prodRLg}\\
    \sum_{e} \mu_{L}^{eg} & = 1  \label{muLg} \\
    \sum_{e} \mu_{R}^{eg} & = 1 \label{muRg}\\
    d_{LR}^{g} & = \sum_{e, e'} z_{LR}^{ee'g} d_{LR}^{ee'g} \label{dLRg},\\
    d_{RL}^{gg'} & = \sum_{e, e'} z_{RL}^{ee'gg'} d_{RL}^{ee'gg'} \label{dRLgg},
\end{align}

\noindent where $d_{LR}^g$ and $d_{RL}^{gg'}$ are defined in \eqref{eq:dLRPg} and \eqref{eq:dRLPg}, respectively. Constraints \eqref{param1g} and \eqref{param2g} parameterize the launch and retrieve points on the polygonal chain. Constraints \eqref{prodLRg} and \eqref{prodRLg} model the product of binary variables. Constraints \eqref{muLg} and \eqref{muRg} state that, in each stage, the launch and retrieve points can be only in one segment, not necessarily the same. Constraints \eqref{dLRg} and \eqref{dRLgg} compute the total distance between the launch and the retrieve point for each pair of points. \JP{The reader may note that the above representation is similar to that given by \eqref{param1}-\eqref{pol:dRLt} with the exception that in \eqref{param1g}-\eqref{dRLgg} constraints are indexed in the set of graphs $g\in \mathcal{G}$ instead that on the stages. This fact allows a remarkable reduction on the number of distance variables and constraints as already discussed in Section \ref{ss:compare}.}

The goal of the (\PMD) is to find a feasible solution that minimizes the total distance covered by the drone and the mothership, i.e.,
\begin{mini*}|s|
 {}{\sum_{i_g} (u^{i_g}d_L^{i_g} + v^{i_g}d_R^{i_g}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_g d_{LR}^g + \sum_{g,g'}d_{RL}^{gg'}w^{gg'}}{}{}\label{PMDRPG-MTZ}\tag{PMDRPG-MTZ}
 \addConstraint{\eqref{DEnt2}-\eqref{DInv2}}{}{}
 \addConstraint{\eqref{TOrig}-\eqref{TEnt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{MTZ3} - \eqref{MTZ6} \text{ or } \eqref{SEC} }{}{}   
 \addConstraint{\eqref{param1g}-\eqref{dRLgg}}{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
  \addConstraint{\eqref{eq:dLRPg}, \eqref{eq:dRLPg}}{}{}
 \addConstraint{\|x_L^g- R^{i_g}\|}{\leq d_L^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_g},\quad}{\forall i_g}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i_g, j_g}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g} d^{i_g} + \sum_{i_g}v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_{RL}^{g}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{The reader may note that the above formulation actually encloses two different ones depending whether it includes constraints \eqref{MTZ1} - \eqref{MTZ2}  or  \eqref{SEC}. However, for the sake of presentation we have preferred to present them in this compact form to reduce the length of the paper.}

\subsection{Network Mothership-Drone Routing Problem with Graphs (\NMD)}
\JP{This new model is a refinement of the last one in that now the mothership has to move on a general undirected network rather than on a polygonal chain. 
Even though the previous one, namely \PMD, can be seen as a particular case of \NMD, for the sake of presentation, we have preferred to include it first to ease the understanding of the more advanced \NMD \ model.

As before, we start with an approach that models the problems by stages. Later, we shall extend the analysis using the rationale of connectivity, as already done in the the previous models \AMD \ and \PMD.}

Let $\mathcal N=(V, E)$ be the network that model the space of movement for the mothership. For each stage $t\in \{1,\ldots,|\mathcal G|\}$, assume that the mothership starts and ends in the edge $e=(i,j)$ and $e'=(i',j')$, respectively. Then, it follows a route from the launching to the retrieving point and vice versa, determined by a sequence of intermediate vertices, similar to the following one:

$$
e=(i, j) \ni x_L^t \rightarrow V_i \vee V_j \rightarrow \ldots \rightarrow V_k \rightarrow \ldots \rightarrow V_{i'} \rightarrow x_R^t \in (i',j')=e'.
$$
\JP{**** \@ Carlos: La notacion de $V_i$ y $i$ es un lio. Esto hay que aclararlo. *****}
Therefore, the distance traveled by the mothership, between two consecutive launching and retrieving points in two edges, not necessarily distinct,  of the graph can be represented as:
\begin{equation}\tag{$d^{t\mathcal N}_{LR}$}\label{eq:dLRNt}
d_{LR}^{ee't} = \left\{\begin{matrix}
|\gamma_{L}^{et} - \gamma_{R}^{et}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{LR}^{it}\gamma_{L}^{et} + b_{LR}^{jt}(1 - \gamma_{L}^{et})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{LR}^{e''t}\mathcal L(e'') + \left[c_{LR}^{i't}\gamma_{R}^{e't} + c_{LR}^{j't}(1 - \gamma_{R}^{e't})\right]\mathcal{L}(e'), & \text{if } e \neq e',
\end{matrix}\right.
\end{equation}

\noindent 
where $b_{LR}^{it}$ (resp. $c_{LR}^{it}$) are binary variables that determine from which of the end-points of $e$ (respectively $e'$) one has to account for the distance and $q_{LR}^{et}$ is a binary variable that is one when the mothership fully traverses the edge $e$. \JP{Furthermore, we need to define another binary variable $z_{LR}^{ee't}$ that models the correct definition of the distance in \eqref{eq:dLRNt}. With the above definition one can account for  the movement of the mothership at each stage $t\in \{1, \ldots, |\mathcal G|\}$ from a launching to a retrieving  point:}

\begin{align}
    x_L^t & = \sum_{e=(i, j)\in E} \mu_{L}^{et}\left[V^i + \gamma_{L}^{et}(V^j - V^i)\right]\label{st:param1bis}\\
    x_R^t & = \sum_{e=(i, j)\in E} \mu_{R}^{et}\left[ V^i + \gamma_{R}^{et}(V^j - V^i)\right]\label{st:param2bis}\\
    z_{LR}^{ee't} & = \mu_{Le}^t\mu_{Re'}^t,\label{st:prodLRbis}\\
    b_{LR}^{it} & \leq \sum_{e\in\delta(i)}\mu_{L}^{et}, \label{st:bLt1}&\qquad\forall i\in V \\
    c_{LR}^{it} & \leq \sum_{e\in\delta(i)}\mu_{R}^{et}, \label{st:cLt1}&\qquad\forall i\in V\\
    b_{LR}^{it} + b_{LR}^{jt} & \geq \sum_{e'\neq e} z_{LR}^{ee't}, &\qquad \forall e=(i, j)\in E\label{st:bLt2}\\
    c_{LR}^{it} + c_{LR}^{jt} & \geq \sum_{e'\neq e} z_{LR}^{e'et}, &\qquad \forall e=(i, j)\in E\label{st:cLt2}\\
    b_{LR}^{it} + \sum_{\{j:(i, j)\in E\}} q_{LR}^{jit} & = \sum_{\{j:(i, j)\in E\}} q_{LR}^{ijt} +  c_{LR}^{it}, \label{st:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{et} & = 1,  \label{st:muLe} \\
    \sum_{e\in E} \mu_{R}^{et} & = 1, \label{st:muRe}\\
    d_{LR}^t & = \sum_{e, e'} z_{LR}^{ee't} d_{LR}^{ee't}, \label{st:dLRt}
\end{align}

Constraints \eqref{st:param1bis} and \eqref{st:param2bis} parameterize the launching and retrieving points in the network $\mathcal N$ at stage $t$. Constraints \eqref{st:prodLRbis} model the product of binary variables. Constraints \eqref{st:bLt1} and \eqref{st:cLt1} say that if the launching point (resp. retrieving point) is not in the edge $e$, the mothership cannot go (resp. exit) to the vertex that is incident to $e$. Constraints \eqref{st:bLt2} state that if the mothership leaves the edge $e$ to go to $e'$, it must exit from one of the incident vertices to $e$. In the same way, restrictions \eqref{st:cLt2} express that if the mothership leaves the edge $e'$ to go to $e$, it must enter to the edge $e$ from one of its incident vertices. Flow conservation constraints \eqref{st:flow} ensure that the number of incoming edges to each vertex $i$ is equal to the number of outgoing edges in the route followed by the mothership. Constraints \eqref{st:muLe} and \eqref{st:muRe} say that, in each stage, the selected points can be only in one edge. Finally, constraints \eqref{st:dLRt} defines the total distance between the launching and the retrieving points at  stage $t$.

\medskip

Similarly, the distance covered by the mothership along the path on the network from the retrieving point $x_R^t$ to the next launching point $x_L^{t+1}$ can be modeled using the following definition of distance:

\begin{equation}\tag{$d^{t\mathcal N}_{RL}$}\label{eq:dRLNt}
d_{RL}^{ee't} = \left\{\begin{matrix}
|\gamma_{R}^{et} - \gamma_{L}^{et+1}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{RL}^{it}\gamma_{R}^{et} + b_{RL}^{jt}(1 - \gamma_{R}^{et})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{RL}^{e''t}\mathcal L(e'') + \left[c_{RL}^{i't}\gamma_{L}^{e't+1} + c_{RL}^{j't}(1 - \gamma_{L}^{e't+1})\right]\mathcal{L}(e'), & \text{if } e \neq e'.
\end{matrix}\right.
\end{equation}

In this case, the binary variable $z_{ee'}^{RLt}$ links the retrieve point at $t$ with the launch point at $t+1$. Then, we can use a set of constraints similar to those used above and the distance from $x_R^t$ to $x_L^{t+1}$ is:

\begin{align}
    z_{RL}^{ee't} & = \mu_{R}^{et}\mu_{L}^{e't+1},\label{st1:prodRL}\\
    b_{RL}^{it} & \leq \sum_{e\in\delta(i)}\mu_{R}^{et}, \label{st1:bRt1}&\qquad \forall i\in V \\
    c_{RL}^{it} & \leq \sum_{e\in\delta(i)}\mu_{L}^{et}, \label{st1:cRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V\\
    b_{RL}^{it} + b_{RL}^{jt} & \geq \sum_{e'\neq e} z_{RL}^{ee't}, &\qquad \forall e=(i, j)\in E\label{st1:bRt2}\\
    c_{RL}^{it} + c_{RL}^{jt} & \geq \sum_{e'\neq e} z_{RL}^{e'et}, &\qquad \forall e=(i, j)\in E\label{st1:cRt2}\\
    b_{RL}^{it} + \sum_{\{j:(i, j)\in E\}} q_{RL}^{jit} & = \sum_{\{j:(i, j)\in E\}} q_{RL}^{ijt} +  c_{RL}^{it}, \label{st1:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{et} & = 1,  \label{st1:muLe} \\
    \sum_{e\in E} \mu_{R}^{et} & = 1, \label{st1:muRe}\\
    d_{RL}^t & = \sum_{e, e'} z_{RL}^{ee't} d_{RL}^{ee't}. \label{st1:dRLtN}
\end{align}

\JP{Constraints \eqref{st1:prodRL} model the product of binary variables. Constraints \eqref{st1:bRt1} and \eqref{st1:cRt1} say that if the retrieving point (resp. launching point) is not in the edge $e$, the mothership cannot go (resp. exit) to the end vertices of the edge $e$. Constraints \eqref{st1:bRt2} state that if the mothership leaves the edge $e$ to go to $e'$, it must exit via one of the end vertices of $e$. In the same way, restrictions \eqref{st1:cRt2} state that if the mothership leaves the edge $e'$ to go to $e$, it necessarily must enter to $e$ from one incident vertex of $e$. Flow conservation constraints \eqref{st1:flow} ensure that in the route followed by the mothership the number of used incoming edges to each vertex $i$ is equal to the number of used outgoing edges. Constraints \eqref{st1:muLe} and \eqref{st1:muRe} say that, in each stage, the selected points can be only in one edge. Constraints \eqref{st1:dRLtN} state the total distance between the retrieving and the launching points at stage $t$.}


Hence, once the distances inside the graph are set with the above two families of constraints, we can state the mathematical programming formulation of the problem as:

\begin{mini*}|s|
 {}{\sum_{i_g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i_g,j_g}z^{i_gj_g}d^{i_gj_g} + \sum_t (d_{RL}^t + d_{LR}^t)}{}{}\tag{TDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{st:param1bis}-\eqref{st1:dRLtN}}{}{}
 \addConstraint{\eqref{eq:dLRNt}, \eqref{eq:dRLNt}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d_g^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\hspace*{-2cm}\left(\sum_{i_g} u^{i_gt}d_L^{i_gt} + \sum_{i, j}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_gt}d^{i_g} + \sum_{i_g} v^{i_gt}d_R^{i_gt}\right)/v_D}{\leq d_{RL}^t/v_M + M(1 - \sum_{i_g} u^{i_gt}),\ }{\forall g, t}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}

\JP{A brief decription of this formulation must be included ...}

\subsubsection{MTZ formulation for the Network Mothership-Drone Routing Problem with Graphs}

\JP{Something missing to connect it to the previous section ... JUSTO: Por aqui 20/11/2020}

Therefore, the distance between launching and retrieving points in two edges, not necessarily distinct,  of the graph can be represented as:
\begin{equation}\tag{$d^{g\mathcal N}_{LR}$}\label{eq:dLRg}
d_{LR}^{ee'g} = \left\{\begin{matrix}
|\gamma_{L}^{eg} - \gamma_{R}^{eg}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{LR}^{ig}\gamma_{L}^{eg} + b_{LR}^{jg}(1 - \gamma_{L}^{eg})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{LR}^{e''g}\mathcal L(e'') + \left[c_{LR}^{i'g}\gamma_{R}^{e'g} + c_{LR}^{j'g}(1 - \gamma_{R}^{e'g})\right]\mathcal{L}(e'), & \text{if } e \neq e',
\end{matrix}\right.
\end{equation}

\noindent 
where $b_{LR}^{ig}$ (resp. $c_{LR}^{ig}$) are binary variables that determine from which of the end-points of $e$ (respectively $e'$) one has to account for the distance and $q_{LR}^{eg}$ is a binary variable that is one when the mothership fully traverses the edge $e$. Furthermore, we need to define binary variables $z_{LR}^{ee'g}$ that model the choice of the model for right definition (first or second formulas in \eqref{eq:dLRg}) of the distance in \eqref{eq:dLRg}. All the above give the necessary elements to account for the movement of the mothership in each graph $g\in \{1, \ldots, |\mathcal G|\}$:

\begin{align}
    x_L^g & = \sum_{e=(i, j)\in E} \mu_{L}^{eg}\left[V^i + \gamma_{L}^{eg}(V^j - V^i)\right]\label{g:param1bisg}\\
    x_R^g & = \sum_{e=(i, j)\in E} \mu_{R}^{eg}\left[ V^i + \gamma_{R}^{eg}(V^j - V^i)\right]\label{g:param2bisg}\\
    z_{LR}^{ee'g} & = \mu_{L}^{eg}\mu_{R}^{e'g},\label{g:prodLR}\\
    b_{LR}^{ig} & \leq \sum_{e\in\delta(i)} \mu_{L}^{eg}, \label{g:bLt1}&\qquad \forall i\in V \\
    c_{LR}^{ig} & \leq \sum_{e\in\delta(i)} \mu_{R}^{eg}, \label{g:cLt1}&\qquad \forall i\in V\\
    b_{LR}^{ig} + b_{LR}^{jg} & \geq \sum_{e'\neq e} z_{LR}^{ee'g}, &\qquad \forall e=(i, j)\in E\label{g:bLt2}\\
    c_{LR}^{ig} + c_{LR}^{jg} & \geq \sum_{e'\neq e} z_{LR}^{e'eg}, &\qquad \forall e=(i, j)\in E\label{g:cLt2}\\
    b_{LR}^{ig} + \sum_{\{j:(i, j)\in E\}} q_{LR}^{jig} & = \sum_{\{j:(i, j)\in E\}} q_{LR}^{ijg} +  c_{LR}^{ig}, \label{g:flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{eg} & = 1,  \label{g:muLe} \\
    \sum_{e\in E} \mu_{R}^{eg} & = 1, \label{g:muRe}\\
    d_{LR}^g & = \sum_{e, e'} z_{LR}^{ee'g} d_{LR}^{ee'g}, \label{g:dLRgN}
\end{align}

\JP{Constraints \eqref{g:param1bisg} and \eqref{g:param2bisg} parameterize the launch and retrieve points in the network $\mathcal N$ induced by the visit to the graph  $g\in \mathcal{G}$. Constraints \eqref{g:prodLR} model the product of binary variables. Constraints \eqref{g:bLt1} and \eqref{g:cLt1} say that if the launch point (resp. retrieve point) is not in the edge $e$, the drone cannot go (resp. exit) to the vertices of the edge $e$. Constraints \eqref{g:bLt2} state that if the drone leaves the edge $e$ to go to $e'$, it must exit from one of the incident vertices to $e$. In the same way, restrictions \eqref{g:cLt2} express that if the drone leaves the edge $e'$ to go to $e$, it necessarily must enter to $e$ from one incident vertex of $e$. Flow conservation constraints \eqref{g:flow} ensure that the number of incoming edges to each vertex $i$ is equal to the number of outgoing edges. Constraints \eqref{g:muLe} and \eqref{g:muRe} say that, in visit to the graph  $g\in \mathcal{G}$, launching and retrieving points can be only in one edge. Constraints \eqref{g:dLRgN} returns the total distance traveled by the drone on the graph  $g\in \mathcal{G}$.}

\medskip

Similarly, the distance covered by the mothership along the path on the network from the retrieving point $x_R^g$ to the next launching point $x_L^{g'}$ can be modeled using the following definition of distance:

\begin{equation}\tag{$d^{g\mathcal N}_{RL}$}\label{eq:dRLg}
d_{RL}^{ee'gg'} = \left\{\begin{matrix}
|\gamma_{R}^{eg} - \gamma_{L}^{eg'}|\mathcal L(e), & \text{if } e = e',\\ 
\left[b_{RL}^{ig}\gamma_{R}^{eg} + b_{RL}^{jg}(1 - \gamma_{R}^{eg})\right]\mathcal L(e) + \displaystyle \sum_{e''\in \mathcal N}q_{RL}^{e''gg'}\mathcal L(e'') + \left[c_{RL}^{i'g'}\gamma_{L}^{e'g'} + c_{RL}^{j'g'}(1 - \gamma_{L}^{e'g'})\right]\mathcal L(e'), & \text{if } e \neq e'.
\end{matrix}\right.
\end{equation}

In this case, the binary variable $z_{RL}^{ee'gg'}$ links the retrieve point at $g$ with the launch point at $g'$. Then, we can use a set of constraints similar to those used above and the distance from $x_R^g$ to $x_L^{g'}$ is:

\begin{align}
    z_{RL}^{ee'gg'} & = \mu_{R}^{eg}\mu_L^{e'g'},\label{prodRLggN}\\
    b_{RL}^{ig} & \leq \mu_{R}^{eg}, \label{bRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V \\
    c_{RL}^{ig} & \leq \mu_{L}^{eg}, \label{cRt1}&\qquad \forall e\in\delta(i),\,\forall i\in V\\
    b_{RL}^{ig} + b_{RL}^{jg} & \geq \sum_{e'\neq e} z_{RL}^{ee'gg'}, &\qquad \forall e=(i, j)\in E\label{bRt2}\\
    c_{RL}^{ig'} + c_{RL}^{jg'} & \geq \sum_{e'\neq e} z_{RL}^{e'eg'g}, &\qquad \forall e=(i, j)\in E\label{cRt2}\\
    b_{RL}^{ig} + \sum_{\{j:(i, j)\in E} q_{RL}^{jigg'} & = \sum_{\{j:(i, j)\in E\}} q_{RL}^{ijgg'} +  c_{RL}^{ig}, \label{flow}&\qquad \forall i \in V\\
    \sum_{e\in E} \mu_{L}^{eg} & = 1,  \label{muLe} \\
    \sum_{e\in E} \mu_{R}^{eg} & = 1, \label{muRe}\\
    d^{RLgg'} & = \sum_{e, e'} z_{RL}^{ee'gg'} d_{RL}^{ee'gg'}. \label{dRLt}
\end{align}

Hence, once the distances inside the graph are set with the above two families of constraints, we can state the mathematical programming formulation of the problem as:

\begin{mini*}|s|
 {}{\sum_{i, g, t} (u^{i_gt}d_L^{i_gt} + v^{i_gt}d_R^{i_gt}) + \sum_{i_g} d^{i_g} + \sum_{i,j,g}z^{i_gj_g}d^{i_gj_g}}{}{}\tag{TDRPG}
 \addConstraint{\eqref{st:DEnt}-\eqref{st:DInv}}{}{}
 \addConstraint{\eqref{g:param1bisg}-\eqref{dRLt}}{}{}
 \addConstraint{\eqref{eq:dLRg}, \eqref{eq:dRLg}}{}{}
 \addConstraint{\eqref{MTZ1} - \eqref{MTZ2} \text{ or } \eqref{SEC} }{}{}
 \addConstraint{\eqref{eq:alpha-E} \text{ or } \eqref{eq:alpha-G}}{}{}
 \addConstraint{\|x_L^t- R^{i_g}\|}{\leq d_L^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{i_g}\|}{\leq d_g^{i_g},\quad}{\forall i_g,t}{}
 \addConstraint{\|R^{i_g}- L^{j_g}\|}{\leq d^{i_gj_g},\quad}{\forall i_g,j}{}
 \addConstraint{\|L^{i_g}- x_R^i\|}{\leq d_R^{i_gt},\quad}{\forall i_g,t}{}
 \addConstraint{\left(\sum_{i_g} u^{i_g}d_L^{i_g} + \sum_{i, j}z^{i_gj_g}d^{i_gj_g} + \sum_{i_g} \mu^{i_g}d^{i_g} + \sum_{i_g} v^{i_g}d_R^{i_g}\right)/v_D}{\leq d_g^{RL}/v_M, \quad}{\forall g}{}\label{ACW}\tag{DCW}
 \addConstraint{x_L^0}{= orig}{}
 \addConstraint{x_R^0}{= orig}{}
 \addConstraint{x_L^{|\mathcal G|+1}}{= dest}{}
 \addConstraint{x_R^{|\mathcal G|+1}}{= dest.}{}
\end{mini*}
% $$
% e=(i, j) \ni x_R^t \rightarrow V_i \vee V_j \rightarrow \ldots \rightarrow V_k \rightarrow \ldots \rightarrow V_{i'} \rightarrow x_L^{t+1} \in (i',j')=e'
% $$

% The design of these paths obeys to define binary variables that decide which vertices are selected in each stage $t$:

==> literature.tex <==
\section{State of the art}
In this section we focus mainly on the previous works in literature related to systems where UAVs are assisted by a vehicle in order to serve a set of targets.
In these configurations the vehicle represents a launch and a recharging station for the UAVs and the main problem consists in coordinating the operations performed by one or multiple drones and the mothership.
Most of the previous works in literature on this subject are focused on node routing problems (NRPs), where the vehicle moves on a road network and the drone is used to visit target points outside the road network. 
Many of them are related to applications in the delivery sector where the set of targets to be visited is represented by a set of customers.
For example, \cite{art:Mathew2015} studies a delivery system consisting in one drone and one truck. The UAV visits one customer for each trip and the truck can wait at the launching node for the drone to come back or move to a different rendezvous node. In \cite{art:Carlsson2018} the authors study a continuous approximation on the Horse Fly Problem, where the truck is used as a mobile depot for the drone. In \cite{art:Campbell2017} the authors evaluate the economic impact of truck-and-drone hybrid models for deliveries by means of a continuous approximation model, considering different model parameters and customer densities. \cite{art:Ferrandez2016} focuses on a delivery system where one truck supports the operations of multiple drones. The authors first clusterize the customer demand by adopting a K-means algorithm to find truck stops that represent hubs for drone deliveries. Then, they determine a TSP of the truck among centroids of these clusters, by means of a genetic algorithm, assuming that drones are not constrained by flight range. In \cite{art:Moshref2017} the authors consider a similar delivery system where at each stop site the truck waits until all drones come back before moving to the next site. The goal is the minimization of the latency in a customer-oriented distribution system. Moreover, the authors compare the benefits of using drones for a single trip versus multiple trips. In \cite{art:Poikonen2020} the authors formalize the k-Multi-visit Drone Routing Problem (k-MVDRP) considering a tandem between a truck and a fleet of k drones. The authors assumed that each drone can deliver one or more packages to customers in a single mission. Each drone may return to the truck to swap/recharge batteries, pick up a new set of packages, and launch again to customer locations. Moreover, the authors decouple the set of launch locations from the set of customer locations. The article presents a mathematical formulation including a drone energy drain function that takes into account each package weight, but the problem is then solved by means of a heuristic algorithm.
\cite{art:Amorosi2020} presents a multi-objective mixed integer linear programming model for the management of a hybrid delivery system consisting in one base vehicle and a fleet of drones. As in \cite{art:Poikonen2020}, the set of launch locations is assumed to be different from the set of customer locations. The problem consists in determining the tour of the base vehicle and the assignments of the customers to the UAVs simultaneously optimizing the distance travelled by the vehicle, the one travelled by the drones and the maximum completion time. The model is solved on two realistic urban scenarios providing a partial exploration of the Pareto frontier of the problem by means of the weighted sum method.\\
Other examples of similar configurations in which a base vehicle supports the operations of one or multiple drones can be found also in other sectors. 
\cite{art:Trotta2018} studies, for example, the city-scale video monitoring of a set of points of interest performed by a fleet of UAVs whose operations are supported by buses and the problem is modeled as a mixed integer linear programming model based on a multi-period directed graph.
However, in all the works mentioned so far, the combined operations of vehicles and drones examine routing for a set of locations and these configurations exploit only part of the advantages of the adoption of drones. Indeed, UAVs can move between any two points in the space not following the road network. Thus, they can be adopted also for other kind of services in which the targets are represented by edges or part of them. This leads to another class of models, that is arc routing problems (ARPs).\\
With respected to NRPs, in the case of ARPs with drones there are relatively few papers. \cite{art:Oh2011} and \cite{art:Oh2014} study a coordinated road network search problem with multiple UAVs and they formulated it as a Multi-choice Multi-dimensional Knapsack Problem minimizing the flight time. This is a modified Chinese Postman Problem taking into account the UAVs energy capacity constraints. The authors solved the problem by means of a greedy insertion heuristic that models drone travel distance between the road components as a Dubins path.
\cite{art:Dille2013} faces the area coverage problem in sparse environments with multiple UAVs. Also in this case the UAVs motion is modeled using Dubins paths and it is assumed that they are equipped with a coverage sensor of a given radius.
The edge covering problem is solved by discretizing the network in orbits and then solving a TSP among this set of orbits. The authors compares the results obtained with the ones obtained with the method by \cite{art:Oh2014}, for simulated urban, suburban and rural scenarios, showing that for suburban densities their method outperforms both with one or multiple UAVs. 
In \cite{art:Chow2016} the authors deal with the problem of dynamically allocate a finite set of UAVs to links in a network that need monitoring, over multiple time periods. The need of drone monitoring is based on data related to traffic conditions. They formulated the first deterministic multi-period arc-inventory routing problem and then its stochastic dynamic version solved with an approximate dynamic programming algorithm. 
Another work related to multiple-period real-time monitoring of road traffic, adopting UAVs, is \cite{art:Li2018}. The authors proposed a mixed integer programming model combining the capacitated arc routing problem with the inventory routing problem and designed a local branching based method for dealing with large instances.\\
The ARPs with one UAV, have common characteristics with problems arising in path generation for laser cutting machines or drawing plotters. In particular, the authors of \cite{art:Campbell2018} studied the Drone Rural Postman Problem (DRPP) showing the relation with the Intermittent Cutting Problem (ICP). They presented a solution algorithm based on the approximation of curves in the plane by polygonal chains and that iteratively increases the number of points in the polygonal chain where the UAV can enter or leave. Thus, they solved the problem as a discrete optimization problem trying to better define the line by increasing the number of points. The authors considered also the case in which the drone has limited capacity and thus it cannot serve all the lines. To deal with this latter case, the authors assumed to have a fleet of drones and the problem consisted in finding a set of routes, each of limited length.\\
The literature related to Drone ARPs is limited with respect to the one related to Drone NRPs.
However, as regards arc routing problems involving a hybrid system consisting in one vehicle and one or multiple drones, the number of contributions in literature is further restricted and we can just mention \cite{art:Tokekar2016} and \cite{art:Garone2010}.\\
In \cite{art:Tokekar2016} the authors studied the path planning problem of a system composed of a ground robot and one drone in precision agriculture and solved it by applying orienteering algorithms. \cite{art:Garone2010} studied the problem of paths planning for systems consisting in a carrier vehicle and a carried one to visit a set of target points and assuming that the carrier vehicle moves in the continuous space. In particular, the authors formulated two different problems: the first one consisting in determining the takeoff/landings sequences of the carried vehicle to visit a set of points, assuming that in each mission of the carried vehicle only one target can be visited. The second one in which this constraint is removed permitting to the carried vehicle to visit more than one target in a single mission, before returning to the carrier vehicle. Heuristic approaches have been proposed to deal with both problems.\\
To the best of our knowledge none of the previous papers in literature deals with a drone arc routing problem combined with a node routing problem for a hybrid system consisting of one vehicle and one drone.
In this paper we present new Mixed Integer Non-Linear Programming (MINLP) formulations for the problem of coordinating a system composed of a mothership (the base vehicle) which supports the operations of one drone which has to visit a set of targets represented by graphs, with the goal of minimizing the total distance travelled by both vehicles.
Indeed, differently from the previous works in literature, we assume the drone can move freely on the continuous space. As regards the mothership, we studied both cases in which also the base vehicle can move freely on the continuous space or it is constrained to move on a road network, of different typologies, where launching and rendezvous points can be chosen.
The main contributions of this article can be summarized as follows:
\begin{itemize}
    \item New mathematical formalization of the coordinating problem of a base vehicle and one drone in the continuous space to visit a set of targets represented by graphs;
    \item Design of new alternative second order cone MINLP formulations;
    \item A new matheuristic algorithm to deal with large instances able to provide high quality solutions in short time;
    \item Extensive experimental analysis comparing the exact solution of the formulations and the matheuristic on a set of generated instances involving different typology of planar graphs.
\end{itemize}
 


